Entailment vs. Verification for Partial-assignment Satisfiability and Enumeration

Many procedures for SAT-related problems, in particular for those requiring the complete enumeration of satisfying truth assignments, rely their efficiency and effectiveness on the detection of (possibly small) partial assignments satisfying an input formula. Surprisingly, there seems to be no unique universally-agreed definition of formula satisfaction by a partial assignment in the literature. In this paper we analyze in deep the issue of satisfaction by partial assignments, raising a flag about some ambiguities and subtleties of this concept, and investigating their practical consequences. We identify two alternative notions that are implicitly used in the literature, namely verification and entailment, which coincide if applied to CNF formulas but differ and present complementary properties if applied to non-CNF or to existentially-quantified formulas. We show that, although the former is easier to check and as such is implicitly used by most current search procedures, the latter has better theoretical properties, and can improve the efficiency and effectiveness of enumeration procedures.

==> abstract.tex.1 <==
Many procedures for SAT and 
SAT-related problems --in particular those requiring the complete
enumeration of satisfying truth assignments--
rely their efficiency
on the detection of {\em partial} assignments satisfying an input
formula.
%
In this paper we analyze in deep the notion of partial-assignment
satisfiability. 
%
We start by raising a flag on the fact that by %ambiguity of the sentence 
``{\em a partial truth assignment $\mu$ satisfies a formula $\vi$}'',
we may  mean  either that $\mu$ {\em entails} $\vi$
(i.e. that all total assignments extending $\mu$
satisfy $\vi$) or that $\mu$ {\em validates} $\vi$ 
 (i.e. that applying $\mu$ to $\vi$ makes $\vi$ true).
%
% We start by raising a flag on the ambiguity of the sentence 
% ``{\em a partial truth assignment $\mu$ satisfies a formula $\vi$}'',
% which may  mean  either that $\mu$ {\em entails} $\vi$
% (i.e. ``all total assignments extending $\mu$
% satisfy $\vi$'') or that $\mu$ {\em validates} $\vi$ 
%  (i.e. ``applying $\mu$ to $\vi$ makes $\vi$ true'');
% %
We notice that, whereas for (tautology-free) CNF formulas entailment 
and validation are equivalent, for non-CNF formulas --and for
existentially-quantified formulas, even CNF ones--
{\em validation is strictly stronger than entailment}, and they have
complementary properties. 

\ignore{
Also, (Tseitin-style) CNF-ization does not solve this
issue, because 
%with Tseitin CNF-ization 
it may lose 
information regarding partial-assignment entailment or validation.
} 
The distinction between entailment and validation
%is not just an issue of terminology, rather it 
has important consequences at algorithmic level:
distinct algorithms implicitly use one or the other as 
satisfiablity criterium; checking entailment is much harder than
checking validation, but it allows for producing smaller partial
assignments, and hence possibly drastically reducing their number. 
This
 may drive the
development of more effective assignment-enumeration algorithms.
%


==> arxiv-version/abstract.tex <==
Many procedures for 
SAT-related problems, in particular for those requiring the complete
enumeration of satisfying truth assignments,
rely their efficiency and effectiveness
on the detection of (possibly small) {\em partial} assignments satisfying an input
formula. 
Surprisingly,
{there seems to be no unique universally-agreed definition of formula satisfaction by
a partial assignment in the literature}.

In this paper we analyze in deep the issue of satisfaction by partial assignments,
%highlighting
raising a flag about
some ambiguities and subtleties of this concept, and investigating their
practical consequences.
%
We identify two alternative notions that are implicitly used in the literature,
namely {\em verification} and {\em entailment},
which coincide if applied to CNF formulas but differ and
present complementary properties if
applied to non-CNF or to existentially-quantified formulas. 
%
We show that, although the former is easier to check and as such is implicitly used
by most current search procedures, the latter has better theoretical
properties, and
can improve the efficiency and effectiveness of enumeration
procedures. 





==> arxiv-version/abstract.tex.1 <==
Many procedures for SAT and 
SAT-related problems --in particular those requiring the complete
enumeration of satisfying truth assignments--
rely their efficiency
on the detection of {\em partial} assignments satisfying an input
formula.
%
In this paper we analyze in deep the notion of partial-assignment
satisfiability. 
%
We start by raising a flag on the fact that by %ambiguity of the sentence 
``{\em a partial truth assignment $\mu$ satisfies a formula $\vi$}'',
we may  mean  either that $\mu$ {\em entails} $\vi$
(i.e. that all total assignments extending $\mu$
satisfy $\vi$) or that $\mu$ {\em validates} $\vi$ 
 (i.e. that applying $\mu$ to $\vi$ makes $\vi$ true).
%
% We start by raising a flag on the ambiguity of the sentence 
% ``{\em a partial truth assignment $\mu$ satisfies a formula $\vi$}'',
% which may  mean  either that $\mu$ {\em entails} $\vi$
% (i.e. ``all total assignments extending $\mu$
% satisfy $\vi$'') or that $\mu$ {\em validates} $\vi$ 
%  (i.e. ``applying $\mu$ to $\vi$ makes $\vi$ true'');
% %
We notice that, whereas for (tautology-free) CNF formulas entailment 
and validation are equivalent, for non-CNF formulas --and for
existentially-quantified formulas, even CNF ones--
{\em validation is strictly stronger than entailment}, and they have
complementary properties. 

\ignore{
Also, (Tseitin-style) CNF-ization does not solve this
issue, because 
%with Tseitin CNF-ization 
it may lose 
information regarding partial-assignment entailment or validation.
} 
The distinction between entailment and validation
%is not just an issue of terminology, rather it 
has important consequences at algorithmic level:
distinct algorithms implicitly use one or the other as 
satisfiablity criterium; checking entailment is much harder than
checking validation, but it allows for producing smaller partial
assignments, and hence possibly drastically reducing their number. 
This
 may drive the
development of more effective assignment-enumeration algorithms.
%


==> arxiv-version/background.tex <==


In this section we introduce the 
notation and terminology adopted in this paper, and 
%Moreover,
% in order to avoid any ambiguity
% (although at the risk of being a little pedantic),
we recall the standard
syntax, semantics and basic facts of propositional logics.

% In order to avoid any ambiguity ---although at the risk of being %a little
% pedantic--- 
% I introduce some
% notation and terminology, and recall the standard
% syntax and semantics of propositional logics, plus some basic facts. 
%

%%% Notation.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Notation.}
In what follows
%the symbols
$\tval$, $\fval$, $\uval$ denote the
truth values ``true'', ``false'' and ``unknown'' respectively;
%the symbols
$\top$, $\bot$ denote the logic constants
``true'' and ``false'' respectively; 
%
%the letters
$A$, $B$ denote propositional atoms;
%
% the Greek symbols
$\varphi,\phi,\psi$ denote propositional formulas;
%
%the Greek symbols
$\mu,\eta,\gamma$ denote truth value assignments.
%  (All above symbols may possibly
% have subscripts.)
%  
The symbols $\alla\defas\set{A_1,...,A_N}$ and
$\allb\defas\set{B_1,...,B_K}$ 
denote disjoint sets of propositional atoms. 
%
More precisely, $\vi$, $\phi$ and $\psi$ denote generic propositional formulas
built on $\alla$, $\allb$ and $\alla\cup\allb$ respectively;
 $\eta$ and $\mu$ denote total and a partial
assignments on $\alla$ respectively;
$\delta$ denote total assignments on $\allb$. (All above symbols may possibly
have subscripts.)  


%%% Syntax.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Syntax.}
A \new{propositional formula} is defined inductively as follows: 
the constants $\top$ and $\bot$ (denoting the truth values true and false)
are formulas; 
   a {propositional atom} 
   $A_1,A_2,A_3,...$ is a formula;
   if $\varphi_1$ and $\varphi_2$ are formulas, then 
\ignore{ $\neg\varphi_1$ and 
  $\varphi_1\bowtie\varphi_2$ are formulas, s.t. $\bowtie\ \in\set{\wedge,\vee,\imp,\limp,\iff}$.
}
%\ignore{
  $\neg\varphi_1$ and 
  $\varphi_1\wedge\varphi_2$
    % $\varphi_1\vee\varphi_2$, 
    % $\varphi_1\imp\varphi_2$, 
    % $\varphi_1\limp\varphi_2$, 
    % $\varphi_1\iff\varphi_2$
%
  are formulas.
We use the standard Boolean abbreviations:  
``$\varphi_1\vee\varphi_2$'' for  
``$\neg(\neg\varphi_1\wedge\neg\varphi_2)$'', 
``$\varphi_1\imp\varphi_2$'' for ``$\neg(\varphi_1\wedge\neg\varphi_2)$'', 
%``$\varphi_1\limp\varphi_2$'' for ``$\neg(\neg\varphi_1\wedge\varphi_2)$'', 
``$\varphi_1\iff\varphi_2$'' for 
``$\neg(\varphi_1\wedge\neg\varphi_2) \wedge
\neg(\varphi_2\wedge\neg\varphi_1)$''.
%}
%
A \new{literal} is either an atom (a \new{positive
 literal}) or its negation (a \new{negative
 literal}).
(If $l$ is a negative literal $\neg A_i$,
then by ``$\neg l$'' we conventionally mean $A_i$ rather than
$\neg\neg A_i$.)
%
A \new{clause} is a disjunction of literals $\bigvee_j l_j$.
% 
A \new{cube} is a conjunction of literals $\bigwedge_j l_j$.
%  
$\varphi$ is in \new{Conjunctive Normal Form (CNF)} iff it is
   a conjunction of clauses:
$
\bigwedge_{i=1}^{L}\bigvee_{j_i=1}^{K_i} l_{j_i}
$.


%%% Semantics.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Semantics.}
Given $\alla\defas\set{A_1,...,A_N}$,
a map  $\eta:\alla\longmapsto\set{\trueval,\falseval}^N$ is a
\new{total truth assignment} for $\alla$. 
%
{We assume $\eta(\top)\defas \trueval$ and $\eta(\bot)\defas \falseval$.}
%
We  represent $\eta$ as a \new{set of literals}
$\eta\defas \set{A_i\ |\ \eta(A_i)=\trueval}\cup\set{\neg A_i\ |\
  \eta(A_i)=\falseval}$. We sometimes represent $\eta$ also as a
\new{cube} 
$%\andeta\defas 
\bigwedge_{\eta(A_i)=\tiny{\trueval}} A_i \wedge 
\bigwedge_{\eta(A_i)=\tiny{\falseval}}\neg A_i
$ which we denote as ``$\andeta$'' so that to distinguish the set and the cube
representations. We denote by $|\eta|$ the number of literals in $\eta$.


Given a {\em total} truth assignment $\eta$ on \alla{} and some formulas
$\vi,\vi_1,\vi_2$ on \alla, the sentence ``$\eta$ {\em satisfies} $\varphi$'', written
``$\eta\models\varphi$'', 
is defined recursively on the structure of $\varphi$ as follows:
%\RSTODO{extend to other connectives?}
$\eta\models \top$, 
$\eta\not\models \bot$, 
$\eta\models A_i$ if and only if $\eta(A_i)=\trueval$,
$\eta\models\neg\vione$ if and only if $\eta\not\models\vione$,
$\eta\models\vione\wedge\vitwo$ if and only if
$\eta\models\vione$ and $\eta\models\vitwo$.
{(The definition of $\eta\models\vi_1\bowtie\vi_2$ for the other
  connectives  follows straightforwardly from their definition in terms
  of $\neg,\wedge$.)}
% $$
% \begin{array}{lcl}
% eta\models A_i &\ \mbox{iff}\ & \eta(A_i)=\trueval\\
% \eta\models \top  & & \\ 
% \eta\not\models \bot  & & \\ 
% \eta\models\neg\phi  &\ \mbox{iff}\ & \eta\not\models\phi\\ 
% \eta\models\phi_1\wedge\phi_2  &\ \mbox{iff}\ & \eta\models\phi_1
%                                                 \mbox{ and}
%                                                 \eta\models\phi_2.\\ 
% \end{array}
% $$
%
$\varphi$ is \new{satisfiable} iff $\eta\models\varphi$ for some total truth
assignment $\eta$ on $\alla$.
%
$\varphi$ is \new{valid} (written ``$\models \vi$'') iff $\eta\models\varphi$ for every total truth
assignment $\eta$ on $\alla$. 
%
\new{$\varphi_1$ entails $\varphi_2$} (written \new{``$\varphi_1\entails
     \varphi_2$''}) iff,  for every total assignment $\eta$ on
   $\alla$, if
 $\eta\models\varphi_1$
then $\eta\models\varphi_2$.
%
$\varphi_1$ and $\varphi_2$ are \new{ equivalent} (written \new{``$\varphi_1\equiv \varphi_2$''}) iff 
$\varphi_1\entails  \varphi_2$ and $\varphi_2\entails  \varphi_1$.
%
Consequently: $\varphi$ is unsatisfiable iff $\neg\varphi$ is valid;
$\vione\models\vitwo$ iff $\vione\imp\vitwo$ is valid;
a clause $\bigvee_i l_i$ is valid (aka is a \new{tautology}) iff both $A_i$ and $\neg A_i$
occur in it for some $A_i$; a CNF formula \vi is valid iff either it
is $\top$ or all its clauses are tautologies. 
We say that a CNF formula is \new{tautology-free} iff none of its clauses
is a tautology.
%

%%%%% PARTIAL ASSIGNMENTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
\input{fig_threevalues}

\paragraph{Partial assignments.}
A map  $\mu:\alla'\longmapsto\set{\trueval,\falseval}^{N'}$
s.t. $\alla'\subseteq\alla$ and $N'\defas|\alla'|$ is a
\new{partial truth assignment} for $\alla$. 
%
% A {\em partial} assignment $\mu$ on $\alla$ is a subset of some total
% assignment $\mu$ for $\alla$, that is, it is a map 
% $\mu:\alla'\longmapsto\set{\trueval,\falseval}^{N'}$ s.t. 
% $\alla'\subseteq A$ and $N'\defas|\alla'|$.
%
As with total assignments, we can represent $\mu$ as a set of literals or as
a cube, denoted with ``$\andmu$''. 
%
Using a three-value logic we extend $\mu$ to \alla{} as
$\mu:\alla\longmapsto\set{\trueval,\falseval,\unknown}^{N}$
by assigning to \unknown{} (unknown) the unassigned atoms in $\alla\setminus \alla'$.
Then we extend the semantics of $\mu$ to any formula $\vi$ on \alla as
described in Figure~\ref{fig:threeval}.
%\ignore{%%% LO DICI DOPO
  We say that $\mu$
{\em \verbverifies{} \resp{\verbfalsifies{}}} $\vi$ if
$\muof{\vi}=\tval$ \resp{$\muof{\vi}=\fval$}.
%}

By ``{\em apply a partial assignment $\mu$ to $\varphi$}'' we mean 
``substitute all instances of each assigned
$A_i$ in $\varphi$ with the truth constants in $\set{\top,\bot}$
corresponding to the truth value assigned by
$\mu$, and then apply recursively the standard
propagation of truth constants through the Boolean connectives
described in Figure~\ref{fig:boolprop}.
%
% , i.e., $\neg\top \thus \bot$, 
% $\neg\bot \thus \top$,
% $\phi\wedge\top \thus \phi$, 
% $\phi\wedge\bot \thus \bot$, and the corresponding ones for $\vee$,
% $\imp$, $\limp$, $\iff$.''
% %
% \RSTODO{Scrivi tutte le rewrtiting rules in figura}
We denote by ``$\applymuvi$'' (``{\em residual of $\vi$ under $\mu$''}) the formula resulting from applying
$\mu$ to $\vi$.
%The following facts follow straightforwardly. % from the above definitions.% we have the following.

%%% general property
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The following facts follow straightforwardly and are of interest for our discussion.

\begin{property}
\label{prop:total-properties}
Let $\eta$ be a total truth assignment on \alla{} and
$\vi,\vione,\vitwo$ be formulas on \alla. 
\begin{renumerate}
\item 
$\eta\models\varphi$ iff $\andeta\entails\varphi$.
\item 
If $\vione$ and $\vitwo$ are  equivalent, then 
$\eta\models\vione$ iff $\eta\models\vitwo$.
\item
$\eta\models\varphi$ iff \applyetavi{} is $\top$ (also, by
property~\ref{prop:eval-simplifies}, iff $\etaof{\vi}= \tval$). 
\item 
Checking
 $\eta\models\vi$
requires at most a polynomial amount of steps.  
\end{renumerate}  
\end{property}
\noindent
Notice that property~\ref{prop:total-properties}(i) justifies the
  usage of ``$\models$'' 
for both satisfiability and entailment.




\begin{property}
  \label{prop:eval-simplifies}
  % Notice that
% Let $\vi$ and $\mu$ be as above.
% Then
Let $\mu$ be a partial assignment on \alla{} and
$\vi$ be a formula on \alla. \\Then
$\applymuvi$ is $\top$ iff $\muof{\vi}=\tval$ and
$\applymuvi$ is $\bot$ iff $\muof{\vi}=\fval$.
\end{property}
\begin{IGNORE}%
  \begin{property}%
  $\andmu\wedge\applymuvi\ \equiv\ \andmu\wedge\vi$.
\end{property}  
\end{IGNORE}

\noindent
Notice that total assignments are a subcase of partial ones, so that
the definition of residual and property~\ref{prop:eval-simplifies} 
% above definitions and facts
apply also to total assignments $\eta$.





\paragraph{Existentially-quantified formulas.}
% In the following $\psi$ denote generic formulas on
% $\alla\cup\allb$, and $\delta$ denote total truth assignments on \allb
% (all symbols possibly with subscripts).
%
A total truth assignment $\eta$ satisfies $\exists \allb. \psi$,
written ``$\eta\models\exists \allb. \psi$'',
iff exists a total truth assignment $\delta$ on \allb s.t.
$\eta\cup\delta\models\psi$.
We call the {\em Shannon expansion} \shannonpsib of the existentially-quantified
formula $\exists \allb. \psi$ the propositional formula on \alla
defined as 
\begin{eqnarray}
\label{eq:shannon}
%$
\shannonpsib\defas 
\textstyle
\bigvee_{\delta_i\in \set{{\scriptsize \tval,\fval}}^{|\allb|}}
\apply{\psi}{\delta_i}
%$
\end{eqnarray}
where $\set{{\tval,\fval}}^{|\allb|}$ is the set of all total
assignments on \allb.
{Notice that some $\apply{\psi}{\delta_i}$ may be inconsistent or $\bot$.}
The following property derives directly from the above definitions.

\begin{property}
\label{prop:total-shannon}
Let   $\psi$ be a formula on
$\alla\cup\allb$ and $\eta$ be a total truth assignment on \alla.
% and $\delta_i$ be total truth assignments on \allb. 
\\Then
% \begin{renumerate}
% \item
$\eta\models\exists \allb. \psi$\ iff\ $\eta\models\shannonpsib$,
that is, $\exists \allb. \psi\equiv \shannonpsib $.
%\end{renumerate}
\end{property}

%%% CNF-ization
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{CNF-ization.}
Every generic formula $\vi$ on \alla can be encoded into a CNF formula $\psi$
on $\alla\cup\allb$ for some \allb by applying (variants of) Tseitin
CNF-ization \TseitinCNF(\vi) \cite{tseitin1}, consisting in applying recursively bottom-up 
the rewriting rule:
%\RSTODO{Introduce also Pl\&Gr CNF-ization?}
\begin{eqnarray}
\label{eq:tseitin}
\vi &\Rightarrow&
\vi[(l_{j1} \bowtie l_{j2})\mapsto B_j]\wedge \DeMorganCNF(B_j \iff (l_{j1} \bowtie l_{j2}))  
\end{eqnarray}
until the resulting formula $\psi$ is in CNF, where $l_{j1},l_{j2}$ are
literals, $\bowtie\ \in\ \set{\wedge,\vee,\imp,\limp,\iff}$ and 
$\DeMorganCNF()$ is the validity-preserving CNF conversion based on DeMorgan
rules (e.g., 
$\DeMorganCNF(B \iff (l_1 \wedge l_2)) \defas 
(\neg B \vee l_1) \wedge 
(\neg B \vee l_2) \wedge 
(B \vee \neg l_1 \vee \neg l_2)$).
%
The size of $\psi$ is linear wrt. that of $\vi$.  
%
With Plaisted\&Greenbaum CNF-ization \PlaistedCNF(\vi)
\cite{plaistedStructurepreservingClauseForm1986}
the term $B_j \iff (l_{j1} \bowtie l_{j2})$ in \eqref{eq:tseitin} is
substituted with $B_j \imp (l_{j1} \bowtie l_{j2})$ \resp{$B_j \limp
  (l_{j1} \bowtie l_{j2})$} if $(l_{j1} \bowtie l_{j2})$ occurs only
positively \resp{negatively} in $\vi$.


\begin{property}{}
\label{prop:cnfequiv}
If $\psi\defas\TseitinCNF(\vi)$ or $\psi\defas\PlaistedCNF(\vi)$, then
%$\psi$ is s.t.
$\eta\models\vi$ iff exists a total assignment $\delta$ on
\allb s.t. $\eta\cup\delta\models\psi$, that is,
$\vi\equiv\exists\allb.\psi$.
\end{property}

%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> arxiv-version/cnf.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Dealing with CNF-ized formulas.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newpage
\subsection{\Verbverification{} and entailment of CNF-ized non-CNF formulas.}
%\subsection{Dealing with CNF-ized formulas.}
\label{sec:partialsat-cnf}

One might argue that in SAT-related problems the distinction between verification and
entailment in \sref{sec:partialsat-plain} is not relevant in practice, because we could
CNF-ize upfront the input non-CNF formulas and then remove tautological clauses,
exploiting property~\ref{prop:cnfequiv} and the fact that the above
distinction does not hold for (tautology-free) CNF
formulas.

Unfortunately, the following result shows this is not the case.
% we show that this is not the case.
% , because with CNF-ization we may loose
% relevant information regarding entailment or \verbverification{}.
%

\begin{theorem}
\label{prop:cnf-stronger}
Let $\vi$ be a non-cnf formula on $\alla$ and $\psi\defas
\TseitinCNF(\vi)$ or $\psi\defas
\PlaistedCNF(\vi)$,
% the formula on $\alla\cup\allb$ resulting from applying Tseitin
% CNF-ization to $\vi$,
and let $\mu$ be a partial truth
assignment over $\alla$.
Then
$\mu\entails\exists\allb.\psi$ if $\mu\verifies\exists\allb.\psi$, but
the converse does not hold. %, even if $\psi$ is tautology-free CNF.
\end{theorem}

\begin{proof}
As an instantiation of \cref{prop:stronger-exists} we have 
$\mu\entails\exists\allb.\psi$ if $\mu\verifies\exists\allb.\psi$.
  %
  \\The fact that the converse does not hold is shown in
  \cref{ex:exists-cnf-stronger}.
  \hfill $\qed$
\end{proof}

\begin{example}
\label{ex:exists-cnf-stronger}
Consider $\vi\defas (A_1\wedge A_2) \vee (A_1\wedge \neg A_2)$ and
$\mu\defas\set{A_1}$.
Then $\psi\defas\TseitinCNF(\vi)$ 
is the formula in \cref{ex:exists-stronger}.
Then $\mu\entails\exists\allb.\TseitinCNF(\vi)$ but
$\mu\not\verifies\exists\allb.\TseitinCNF(\vi)$.\\
Let $\psi\defas\PlaistedCNF(\vi)$ instead. Since $\psi$ is \TseitinCNF(\vi) minus
its two ternary clauses, we also have that
$  \shannonpsib= 
  \xcancel{(A_1\wedge A_2\wedge\neg A_2)}\vee (A_1\wedge A_2)\vee (A_1\wedge\neg A_2) 
\vee \xcancel{\bot}.$\\
Thus $\mu\entails\exists\allb.\PlaistedCNF(\vi)$ but
$\mu\not\verifies\exists\allb.\PlaistedCNF(\vi)$.
\hfill $\diamond$
\end{example}

Intuitively, the whole point is that both \TseitinCNF(\vi) and \PlaistedCNF(\vi)
introduce fresh variables \allb{}, which must be implicitly existentially
quantified away in order to preserve equivalence and thus produce the set
of original satisfying assignments (property~\ref{prop:cnfequiv}).
Although these variable do not affect entailment, they may affect
\verbverification{}. In fact, since $\vi$ and $\exists\allb.\TseitinCNF(\vi)$
\resp{$\exists\allb.\PlaistedCNF(\vi)$} are equivalent, they are
entailed by the same partial assignments, but they are not
\verbverified{} by the same partial assignments.

To this extent, in \cite{masinaCNFConversionDisjoint2023} we addressed
a different though related problem: we proved 
that ---unlike with $\psi\defas\TseitinCNF(\vi)$ or with
$\psi\defas\PlaistedCNF(\vi)$--- if $\psi\defas\PlaistedCNF(\NNF{\vi})$ and 
$\mu\verifies\vi$, then $\mu\verifies\exists\allb.\psi$.
Notice, however, that this fact does not apply to our problem, 
% even using $\psi\defas\PlaistedCNF(\NNF{\vi})$ instead of
% $\psi\defas\TseitinCNF(\vi)$ or $\defas\PlaistedCNF(\vi)$ does not fix our problem,
because \cref{prop:cnf-stronger} holds also for $\psi\defas\PlaistedCNF(\NNF{\vi})$.

\begin{example}
  Consider $\vi$ and $\mu$ as in \cref{ex:exists-cnf-stronger}.
  Since $\vi$ is already in NNF, then we have that
  $\psi\defas\PlaistedCNF(\NNF{\vi}) = \PlaistedCNF(\vi)$.
  Therefore $\mu\entails\exists\allb.\PlaistedCNF(\NNF{\vi})$ but
$\mu\not\verifies\exists\allb.\PlaistedCNF(\NNF{\vi})$.
\hfill $\diamond$

\end{example}

%\TODO{Commentare. Confrontare con paper con gabriele. \\Altro? ?}




\ignore{%%% TAGLIATA %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In fact, if
$\psi$ on $\alla\cup\allb$ is the result of Tseitin CNF-izing $\vi$, 
then:
\begin{itemize}
% \item 
% If $\mu\cup\gamma\verifies\phi$ for some total truth assignment
%   $\gamma$, then $\mu\verifies\vi$.
% \item 
% If $\mu\cup\gamma\entails\phi$ for some total truth assignment
%   $\gamma$, then $\mu\entails\vi$.
\item 
$\mu\verifies\vi$ \emph{does not imply} that there exists a total assignment
  $\delta$ on \allb s.t. $\mu\cup\delta\verifies\psi$;
\item 
$\mu\entails\vi$ \emph{does not imply} that there exists a total assignment
  $\delta$ on \allb s.t. $\mu\cup\delta\entails\psi$.
\end{itemize}

\begin{example}
Consider $\vi\defas A_1 \vee (A_2\wedge A_3)$ 
and its Tseitin CNF-ized version:\\
$
\begin{array}{lll}
\psi\defas & (A_1\vee  B_1)\ \wedge \\
& (\neg B_1 \vee  A_2) \wedge
(\neg B_1 \vee  A_3) \wedge 
(B_1\vee \neg A_2 \vee \neg A_3) & \ \ \ //\ B_1 \iff (A_2\wedge A_3). \\
\end{array}
$\\
On the one hand, $\mu\defas \set{A_1}$ is such that $\mu\verifies\vi$. 
On the other hand, there is no total truth assignment $\delta$ on
\set{B_1} s.t. $\mu\cup\delta\verifies\psi$. In fact, neither 
$\set{A_1,B_1}\verifies\psi$ nor $\set{A_1,\neg B_1}\verifies\psi$.

Consider $\vi\defas
(A_1\wedge \pos A_2)\vee (A_1\wedge\neg A_2) 
$ 
and its Tseitin CNF-ized version:\\
$
\begin{array}{lll}
\psi\defas  
& (B_1\vee B_2)\ \wedge & \\
& (\neg B_1 \vee \pos A_1) \wedge
(\neg B_1 \vee \pos A_2) \wedge
(B_1\vee \neg A_1 \vee \neg A_2)\ \wedge\ & \ \ \ //\ B_1 \iff (A_1\wedge \pos A_2) \\
& (\neg B_2 \vee \pos A_1) \wedge
(\neg B_2 \vee \neg A_2) \wedge
(B_2\vee \neg A_1 \vee \pos A_2).\ & \ \ \ //\ B_2 \iff (A_1\wedge \neg A_2) 
\end{array}
%
% \psi\defas
% (B_1\vee B_2) \wedge
% (\neg B_1 \vee A_1) \wedge
% (\neg B_1 \vee A_2) \wedge
% (B_1\vee \neg A_1 \vee \neg A_2) \wedge
% (\neg B_2 \vee \neg A_1) \wedge
% (\neg B_2 \vee \neg A_2) \wedge
% (B_2\vee \neg A_1 \vee A_2)   
$\\
Although $\mu\defas \set{A_1}$ is such that $\mu\entails\vi$,
%On the other hand,
\RSTODO{WRONG: riscrivere}
 there is no total truth assignment $\delta$ on
\set{B_1,B_2} s.t. $\mu\cup\delta\entails\psi$:
$\set{A_1,B_1,\neg B_2}\not\entails \psi$ since
$\set{A_1,\neg A_2,B_1,\neg B_2}\not\entails \psi$;
$\set{A_1,\neg B_1,B_2}\not\entails \psi$
since $\set{A_1,A_2,\neg B_1,B_2}\not\entails \psi$;
$\set{A_1,B_1,B_2}$ and $\set{A_1,\neg B_1,\neg B_2}$ are both inconsistent
with $\psi$.
\hfill $\diamond$
\end{example}


\begin{theorem}
 \RSTODO{PROVA e scrivi controesempi. Scrivi in background l'equivalente controparte per $\eta \models\vi$\\}
Let $\vi$ be a generic (non-CNF)
formula on \alla and let $\psi$ on $\alla\cup\allb$ be the result of
CNF-izing \vi by applying standard Tseitin CNF-ization 
\cite{tseitin1} and removing valid clauses from $\psi$ if any, \allb
being the set of fresh propositions introduced in the process. Then:
\begin{itemize}
\item 
If $\mu\cup\gamma\verifies\psi$ for some total truth assignment
  $\gamma$, then $\mu\verifies\vi$.
\item 
If $\mu\cup\gamma\entails\psi$ for some total truth assignment
  $\gamma$, then $\mu\entails\vi$.
\item 
$\mu\verifies\vi$ \emph{does not imply} that there exists a total assignment
  $\delta$ on \allb s.t. $\mu\cup\delta\verifies\vi$
\item 
$\mu\entails\vi$ \emph{does not imply} that there exists a total assignment
  $\delta$ on \allb s.t. $\mu\cup\delta\entails\vi$
\end{itemize}

%Then $\mu\verifies\vi$, but
%$\mu\entails\vi$
\end{theorem}
} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> arxiv-version/concl.tex <==
In this paper we have analyzed in deep the issue of formula satisfaction by
partial assignments.
%
We have identified two alternative notions that are implicitly used in the literature,
namely {verification} and {entailment}, and we have showed that, 
%
although the former is easier to check and as such is implicitly used
by most current search procedures, the latter has better theoretical
properties, and
can improve the efficiency and effectiveness of enumeration
procedures.

From a theoretical viewpoint, we champion the idea that
partial-assignment satisfaction should universally be defined as
entailment, % by the AR and SAT communities,
considering  \verbverification{} only an easy-to-check sufficient condition for it.
%
From a practical viewpoint, we suggest that entailment should be
adopted as partial-assignment satisfaction check inside
enumeration-based procedures in place of \verbverification. 

\smallskip
The analysis presented in this paper opens several research
avenues. 
%
First, we wish to investigate and evaluate empirically novel entailment-based
techniques for both (projected) enumeration and (projected) model counting.
In particular we wish to enhance our (projected) AllSAT procedure
in \cite{spallittaDisjointPartialEnumeration2024} with entailment
tests.
%
Second, we wish to implement entailment-based enumeration techniques
to enhance our AllSMT procedures in \mathsat{} \cite{mathsat5_tacas13} and evaluate them empirically. In particular,
we wish to embed and evaluate such entailment-based AllSMT procedure inside our WMI tools
\cite{morettin_aij19,spallittaEnhancingSMTbasedWeighted2024a}. 
%
Third, we wish to embed novel entailment-based AllSMT procedures
inside our SMT compilers for \T-OBDDs and \T-SDDs
\cite{MicheluttiEcai24}, extending it also to general \T-d-DNNFs. 





==> arxiv-version/fig_threevalues.tex <==
\begin{figure}[t!]
  % \footnotesize
  \small
  %\centering
  \begin{tabular}{ccc}
  \begin{minipage}[t]{0.45\textwidth}
  %\centering
    $
      \begin{array}{||c||l|l|l|l|l|l|l|l|l||}
  \hline    
  \muof{\vi_1}            & \tval & \tval & \tval & \uval & \uval & \uval &\fval & \fval & \fval\\
  \muof{\vi_2}            & \tval & \uval & \fval & \tval & \uval & \fval &\tval & \uval & \fval\\
     \hline
  \muof{\neg\vi_1}        & \fval & \fval & \fval & \uval & \uval & \uval &\tval & \tval & \tval\\
  \muof{\vi_1\wedge\vi_2} & \tval & \uval & \fval & \uval & \uval & \fval &\fval & \fval & \fval\\
  \muof{\vi_1\vee\vi_2}   & \tval & \tval & \tval & \tval & \uval & \uval &\tval & \uval & \fval\\
  \muof{\vi_1\imp\vi_2}   & \tval & \uval & \fval & \tval & \uval & \uval &\tval & \tval & \tval\\
  \muof{\vi_1\iff\vi_2}   & \tval & \uval & \fval & \uval & \uval & \uval &\fval & \uval & \tval\\
     \hline
      \end{array}
      $
\caption{\label{fig:threeval}
Three-value-semantics of $\muof{\vi}$ in terms of \set{\tval,\fval,\uval}%
%(``true'', ``false'', ``unknown'')%
.\newline
\ignoreinlong{The definition of
$\muof{\vi_1\bowtie\vi_2}$ s.t. $\bowtie\ \in\set{\vee,\imp,\limp,\iff}$
follows straighforwardly.}
}
  \end{minipage}
      & \hspace{.025\textwidth} &
  \begin{minipage}[t]{0.4\textwidth}
  %\centering
    $
    \begin{array}{|cl|cl|}
  \hline    
      \neg\top & \Rightarrow \bot & \neg \bot & \Rightarrow \top \\
      \top\wedge\vi, \vi\wedge\top  & \Rightarrow \vi & \bot\wedge\vi,  \vi\wedge\bot& \Rightarrow \bot \\
      \top\vee\vi, \vi\vee\top& \Rightarrow \top & \bot\vee\vi, \vi\vee\bot& \Rightarrow \vi \\
      \top\imp\vi & \Rightarrow \vi & \bot\imp\vi & \Rightarrow \top \\
      \vi\imp\top & \Rightarrow \top & \vi\imp\bot & \Rightarrow \neg\vi \\
      \top\iff\vi, \vi\iff\top& \Rightarrow \vi & \bot\iff\vi, \vi\iff\bot& \Rightarrow \neg\vi \\
 %     & & &  \\
  \hline         
    \end{array}
    $\\ 
    \caption{\label{fig:boolprop}
    Propagation of truth values 
through the Boolean connectives.  }
\end{minipage}%
\end{tabular}
\end{figure}


==> arxiv-version/figure.tex <==
\newcommand{\mainwff}{\ensuremath{(A_1\wedge  A_2)\vee(A_1\wedge \neg A_2)}}
\newcommand{\wffl}{\ensuremath{(A_1\wedge  A_2)}}
\newcommand{\wffr}{\ensuremath{(A_1\wedge \neg A_2)}}
\newcommand{\Aone}{\ensuremath{A_1}}
\newcommand{\nAone}{\ensuremath{\neg A_1}}
\newcommand{\Atwo}{\ensuremath{A_2}}
\newcommand{\nAtwo}{\ensuremath{\neg A_2}}  
\newcommand{\singlemu}{\set{A_1}}
\newcommand{\allmus}{\set{\set{A_1,A_2},\set{A_1,\neg A_2}}}
% 
\begin{figure}[t]  
  \centering   
\scalebox{.8}{\input{comparison.pdf_t}} 
\caption{Left: OBDD for $\vi\defas\mainwff{}$. \newline
Center and right: Assignment enumeration for  $\vi$ via Analytic
Tableaux and (non-CNF) DPLL.
\label{fig:comparison}} 
\end{figure} 


==> arxiv-version/figure_long.tex <==
\newcommand{\mainwffone}{\ensuremath{(A_1\wedge  A_2)\vee(A_1\wedge \neg A_2)}}
\newcommand{\mainwfftwo}{\ensuremath{(\neg A_3\wedge  A_4)\vee(\neg A_3\wedge \neg A_4)}}
\newcommand{\mainwff}{\ensuremath{(\mainwffone)\wedge(\mainwfftwo)}}
\newcommand{\mainwffstacked}{\ensuremath{
    \begin{array}{c}
      \mainwffone \\
      \mainwfftwo
    \end{array}}}
\newcommand{\wffl}{\ensuremath{(A_1\wedge  A_2)}}
\newcommand{\wffr}{\ensuremath{(A_1\wedge \neg A_2)}}
\newcommand{\wffltwo}{\ensuremath{(\neg A_3\wedge  A_4)}}
\newcommand{\wffrtwo}{\ensuremath{(\neg A_3\wedge \neg A_4)}} 
\newcommand{\Aone}{\ensuremath{A_1}}
\newcommand{\nAone}{\ensuremath{\neg A_1}}
\newcommand{\Atwo}{\ensuremath{A_2}}
\newcommand{\nAtwo}{\ensuremath{\neg A_2}}  
\newcommand{\Athree}{\ensuremath{A_3}}
\newcommand{\nAthree}{\ensuremath{\neg A_3}}
\newcommand{\Afour}{\ensuremath{A_4}}
\newcommand{\nAfour}{\ensuremath{\neg A_4}} 
\newcommand{\singlemu}{\set{A_1,\neg A_3}}
\newcommand{\allmus}{
  \set{
    \set{A_1,A_2,\neg A_3,A_4},
    \set{A_1,A_2,\neg A_3,\neg A_4},
    \set{A_1,\neg A_2,\neg A_3,A_4},
    \set{A_1,\neg A_2,\neg A_3,\neg A_4}}}
%  
\begin{figure}[t]  
  \centering 
\scalebox{.8}{\input{comparison_long.pdf_t}} 
\caption{$\vi\defas\mainwff{}$.
%\TODO{Split into two figures}  
  \TODO{Add example of d-DNNFs and SDDs}
  \TODO{add example with dualiza/HALL}
\TODO{Add example of enumeration of CNF-ized formula}
Left and center: Assignment enumeration for $\vi$  via Analytic
Tableaux and (non-CNF) DPLL. 
Right: OBDD for $\vi$.
\label{fig:comparison}} 
\end{figure} 


==> arxiv-version/intro.tex <==
% \TODO{\bf Note for PC members: in compliance with the chairs' indications,
%   this paper was submitted in draft form by February 26 AoE
%   only to allow for
%   its bidding, and the final version will be submitted by March 1 AoE.}
\emph{Motivations.}
Many search procedures for SAT-related problems (e.g.  Analytic
Tableaux \cite{smullyan1}, DPLL \cite{davis7}, circuit AllSAT~\cite{friedAllSATCombinationalCircuits2023}) and many formula compilers
(e.g., d-DNNFs
\cite{darwicheCompilerDeterministicDecomposable2002,darwicheKnowledgeCompilationMap2002},
OBDDs \cite{bryant2} and SDDs \cite{darwicheSDDNewCanonical2011})
rely their efficiency and effectiveness on the detection of {\em partial} truth
assignments $\mu$ satisfying an input propositional formula $\vi$,
which allows to state that not only 
$\vi$ is satisfiable, but also
all total
assignments extending $\mu$ satisfy \vi.
In particular,
when it comes to SAT-based problems requiring
the {\em complete enumeration} of satisfying assignments (e.g. \#SAT
\cite{GomesSS21}, Lazy SMT \cite{sebastiani07,BarrettSST21}, OMT \cite{sebastiani15_optimathsat}, AllSAT and AllSMT
\cite{lahiriSMTTechniquesFast2006,cavada_fmcad07_predabs,friedAllSATCombinationalCircuits2023},
\#SMT \cite{PhanM15,chisticov15}, Projected \#SAT
\cite{azizExistsSATProjected2015}, Projected AllSAT/AllSMT
\cite{lahiriSMTTechniquesFast2006,gebserSolutionEnumerationProjected2009,spallittaDisjointPartialEnumeration2024},
knowledge compilation into d-DNNF{} \cite{darwicheCompilerDeterministicDecomposable2002,lagniezLeveragingDecisionDNNFCompilation2024},
satisfiability in modal and description logics
\cite{SebastianiT21}, Weighted Model Integration
\cite{morettin_aij19,spallittaEnhancingSMTbasedWeighted2024a}),
%
the ability of enumerating satisfying {partial} assignments which are
as small as possible is essential, because
each of them avoids the enumeration of the whole subtree of total
assignments extending it, whose size is exponential in the number of
unassigned atoms.

We start by raising %This raised
a
%fundamental
very-basic
question: \emph{What should we mean by ``a partial
assignment $\mu$ satisfies a formula $\vi$''?} 
%
We notice that, quite surprisingly and despite its
widespread implicit usage in algorithms, 
%\emph%
{there is no unique and universally-agreed definition for
%the sentence ``\emph{a partial assignment $\mu$ satisfies a formula $\vi$}''  
formula satisfaction by partial assignments
in the literature}:
% {\em there seems to be no general and universally-agreed notion of
% formula satisfaction by a partial assignment in the literature}:
%\begin{itemize}
%\item
most authors do not define it 
  explicitly;
% \footnote{An  exception is our own work (e.g., 
%   \cite{gs-infocomp2000,sebastiani07,SebastianiT21}), where we defined it as entailment, see below.}
%\item
a few others define it only when dealing with
%(tautology-free)
CNF formulas (e.g.  \cite{BuningK21});
%\item
the very few who define it, 
  adopt one of the following distinct 
  definitions: %, either
\begin{itemize}
\item %[{\em \Verbverification{}:}]
%\\%(a)
[``\emph{applying $\mu$ to $\vi$ makes $\vi$ true}''] (e.g.,
  \cite{DarwicheDNNF-ACM01,friedAllSATCombinationalCircuits2023}).
We say that \emph{$\mu$ \verbverifies{} $\vi$};~\footnote{%
The etymology of ``to verify'' derives from Latin ``{\em verum facere}'', meaning ``to make true''.} 
%\\
%, or
%\item[{\em Entailment{}:}]  %(a)
%(b)
\item
   [``\emph{all total assignments extending $\mu$ satisfy $\vi$}'']
   (e.g., \cite{gs-infocomp2000,sebastiani07}).
   We say that \emph{$\mu$ entails $\vi$}.
%For the former we say that \emph{$\mu$ \verbverifies{} $\vi$};
%for the latter we say that \emph{$\mu$ entails $\vi$}.
  % (E.g. we defined it as entailment in
  % \cite{gs-infocomp2000,sebastiani07,SebastianiT21}, whereas 
  % \cite{friedAllSATCombinationalCircuits2023} defined it as
  % verification, see below.)~%
\end{itemize}
%For (a) we say that \emph{$\mu$ \verbverifies{} $\vi$}
%\end{itemize}
%
%\footnote{%
Notice that this is not simply an issue of
%\RSTODO{Tagliare questo paragrafo?}
the meaning of the word ``satisfy'': regardless which verb we
may  use for it (e.g. ``satisfy'', ``entail'',  ``verify'',
``imply'',...), it should be desirable to have a unique and universally-agreed criterion
to establish it.
% , if a partial truth-assignment {\sf verb}s a formula
% $\vi$, then $\vi$ is satisfiable and all total truth
%  assignments extending it satisfy $\vi$.
% %}

\paragraph{Contributions.}
In this paper we 
%\RSTODO{Espandi o modifica}
analyze in deep
the notion of {\em partial-assignment
satisfiability}, in particular when dealing with  non-CNF and
existentially-quantified formulas,
raising  a flag about the ambiguities and subtleties
of this concept, and
investigating their consequences.
Our contributions are both theoretical and practical.

\paragraph{Theoretical analysis.}
%From a theoretical perspective,
We show, %we notice,
analyze and discuss
the following theoretical facts.

% \TODO{Distinguere aspetti teorici da quelli pratici.\\
% From a theoretical viewpoint ...\\
% From a practical viewpoint ...}
% \marg{no agreed notion of pa-sat}

\begin{aenumerate}
\item Whereas for (tautology-free\footnote{A CNF formula is
tautology-free if it contains no tautological clause in the form
$(l\vee \neg l\vee ...)$. Since tautological clause can be easily
removed upfront by simple preprocessing, hereafter we often assume
w.l.o.g. that CNF formulas are tautology-free.})
CNF formulas
partial-assignment satisfiability can be indifferently be interpreted
either as \verbverification{} or as entailment
% the sentence \marg{$\entails$
% or $\verifies$} ``{a partial truth assignment $\mu$ satisfies a
% formula $\vi$}'' may be indifferently be interpreted either as ``$\mu$
% {\em \verbverifies{}} $\vi$'' or as ``$\mu$ {\em entails} $\vi$''
because in this case the two concepts coincide,
%\marg{$\verifies$  stronger $\entails$ }
{\em for non-CNF formulas \verbverification{} is
strictly stronger than entailment}, and they have complementary
properties.
 %

\item
Whereas two equivalent %though syntactically-different
  formulas are always entailed by the
same partial assignments,
{\em they are not always
  \verbverified{} by the same partial assignments}.

\item \Verbverification{} checks that the residual of a
  formula under a partial assignment is the true formula, whereas
  entailment checks it is a valid formula. Thus
  \verbverification{} can be computationally much cheaper to check than
  entailment. % , although less informative.

\item
$(a)$-$(c)$ apply also to
existentially-quantified formulas, \emph{even those in CNF}.


\item
$(a)$-$(c)$ apply also to
existentially-quantified formulas resulting from CNF-ization.


\ignore{  
CNF-izing upfront the formulas %with the standard techniques
\cite{tseitin1,plaistedStructurepreservingClauseForm1986} does not
fix %solve %the above
issues $(a)$-$(c)$, since fresh atoms are introduced, and
\emph{a partial assignment over the original atoms
% variables of the
%  \RSTODO{inverti con punto (e)?}
%  original %non-CNF
%  formula
  may
  entail the existentially-quantified 
  CNF-ized formula without   \verbverifying{} it.}
} 
%with Tseitin CNF-ization 
% the introduction of fresh atoms may affect
% \verbverification{}.



\end{aenumerate}
%
We stress the fact that $(b)$ (and $(d)$ and $(e)$ consequently) would be an embarrassing fact
if we adopted \verbverification{} as the definition of  partial-assignment
satisfiability. As such, we champion the idea
that the latter should be defined as
entailment \cite{gs-infocomp2000,sebastiani07,SebastianiT21},
and that \verbverification{} should be considered an easy-to-check sufficient %but unnecessary
condition for it. 

% Theoretical condiderations suggest to interpretate the sentence
% ``{\em a partial truth assignment $\mu$ satisfies a formula $\vi$}'' as
% ``$\mu$ {\em entails} $\vi$''
% (i.e. ``all total assignments extending $\mu$
% satisfy $\vi$''). \RSTODO{Dire quali: preserve equivalence.}
% %
% Practical condiderations suggest instead to interpretate \RSTODO{completare}

%\marg{algos diff notions}

%\newpage
%\smallskip
\paragraph{Practical consequences.}
% From the practical perspective, we show the following important
% consequences. 
% We show %that the above facts have
% the following practical consequences of the above facts.
The above facts have
the following practical consequences.


\begin{enumerate}
% \item In plain satisfiability is not worth adopting entailment 
%   because is more expensive and produces no benefits
%   wrt. \verbverification{}, since we need
%   finding only one total assignment $\eta$ extending $\mu$.
%   Also, due to $(a)$, when the input problem is natively in CNF the above
%   distinction is not relevant as well, because these two concepts
%   concide.
\item In plain satisfiability we need
  finding only one total assignment $\eta$ extending $\mu$, so that
  entailment produces no benefits
  wrt. \verbverification{} and is more expensive $(c)$. 
  % is not worth adopting entailment 
  % because is more expensive $(c)$ and produces no benefits
  % wrt. \verbverification{}.
  Also, due to $(a)$, when the input problem is natively in CNF the 
  distinction between \verbverification{} and entailment is not relevant, because these two concepts
  coincide.~%
\ignore{\footnote{We conjecture that this is the main reason why the distinction between
\verbverification{} and entailment has been long overlooked in the literature.}}


  
% \item For plain satisfiability the distinction between
%   \verbverification{} and entailment is not  relevant, because we need
%   finding only one total assignment $\eta$ extending $\mu$.
%    Also, due to $(a)$, when the input problem is natively in CNF the above
%    distinction is not relevant as well, because these two concepts concide.
\end{enumerate}


\noindent
Consequently, both the algorithms for satisfiability and these for enumeration with CNF
formulas typically use \verbverification{} as satisfiability criterion for
the current partial assignments, because it
is much cheaper and easier to implement than entailment.~%
\ignore{\footnote{For satisfiability of CNF formulas, CDCL SAT solvers produce
  {\em total} truth
assignments.}}
This is the case, e.g., of classical procedures like  Analytic
Tableaux \cite{smullyan1} and DPLL \cite{davis7,armando5}, 
or more-recent
enumeration, counting or knowledge compilation procedures, e.g. 
\cite{darwicheCompilerDeterministicDecomposable2002,lahiriSMTTechniquesFast2006,gebserSolutionEnumerationProjected2009,azizExistsSATProjected2015,friedAllSATCombinationalCircuits2023,lagniezLeveragingDecisionDNNFCompilation2024}.
A few notable exceptions are the {\sf Dualiza} procedure
\cite{mohleDualizingProjectedModel2018} and the procedures we
described in 
\cite{moehle20,moehle21,friedEntailingGeneralizationBoosts2024};
also OBDDs \cite{bryant2} and SDDs \cite{darwicheSDDNewCanonical2011}
formula compilers implicitly use entailment to prune branches so that
to guarantee canonicity (see below and 
\sref{sec:practical}).

%Nevertheless,
The scenario changes when we deal with
enumeration-based algorithms applied to non-CNF formulas, or to
existentially-quantified formulas, or to CNF-ized formulas.
\begin{enumerate}
  \setcounter{enumi}{1}
\item Due to $(a)$, a partial assignment may entail a formula without
  \verbverifying{} it. Thus adopting entailment as partial-assignment satisfiability
  criterion during the search allows for detecting satisfiability earlier than with
  verification, %in the search,
  and thus for producing smaller partial truth assignments.
\end{enumerate}
\noindent
Although this fact is not very interesting for plain satisfiability,
it may become fundamental for enumeration, because the detection of a
satisfying partial assignment avoids the enumeration of the whole subtree of total assignments
extending it, whose size is exponential in the number of unassigned
atoms: \emph{the earlier satisfiability is detected, the (up to
exponentially) less assignments are enumerated}.

%Also existentially-quantified formulas are affected by this  distinction:

\begin{enumerate}
  \setcounter{enumi}{2}
\item Due to $(d)$, a partial assignment may entail an
  existentially-quantified formula, even a CNF one, without
  \verbverifying{} it. Thus, as with non-CNF formulas $(b)$, adopting entailment as partial-assignment satisfiability
  criterion during the search allows for detecting satisfiability earlier than with
  verification.
\end{enumerate}

\noindent
This is important because in many application domains
%\marg{relevance of existentially- quantified}
fundamental operations ---like {\em  
  pre-image computation} in symbolic model checking
(see e.g. \cite{burch1}) or {\em predicate abstraction} in SW verification
(see e.g. \cite{graf_predabs97,lahiriSMTTechniquesFast2006}) or {\em projected
  enumeration} (see e.g. \cite{lahiriSMTTechniquesFast2006,gebserSolutionEnumerationProjected2009,spallittaDisjointPartialEnumeration2024})
or {\em projected model counting} (see e.g. \cite{azizExistsSATProjected2015}) ---
require dealing with existentially-quantified formulas and with
the enumeration of partial assignments satisfying them.



\begin{enumerate}
  \setcounter{enumi}{3}
\item Due to $(e)$, CNF-izing upfront the non-CNF formula with the standard
  techniques \cite{tseitin1,plaistedStructurepreservingClauseForm1986}
  does not fix issues $(a)$-$(c)$, since fresh atoms are
  introduced, and \emph{a partial assignment over the original
    atoms may entail the existentially-quantified CNF-ized
    formula without \verbverifying{} it.}
\end{enumerate}

\noindent
This is important because it shows that,
although verification and entailment coincide for CNF formulas, 
fact
2. above cannot be fixed by simply CNF-izing a formula
upfront and running a CNF enumeration procedure based on partial-assignment
verification, projecting out the fresh variables introduced by the CNF-ization.



\begin{enumerate}
  \setcounter{enumi}{4}
\item Due to $(c)$, checking \verbverification{}
is polynomial, whereas checking
entailment is co-NP-complete, since it consists in checking the validity of
the residual formula. 
\end{enumerate}

\noindent
This is the main argument in favour of \verbverification{}
vs. entailment. 
%
We notice, however, that if $\mu$ entails $\vi$, then the residual of
$\vi$ under $\mu$ 
is typically much smaller than \vi with a much
smaller search space, since its
atoms are only (a subset of) those which are not assigned
by $\mu$. Notice also that, when this happens, entailment prevents
from enumerating a number of assignments which is exponential in the
number of the atoms in the residual. Therefore, unlike with
plain satisfiability, for enumeration the tradeoff may be favourable
to entailment checks.


% \newpage
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \NOTE{RISCRITTO FIN QUI}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Theoretical condiderations suggest to interpretate the sentence
% ``{\em a partial truth assignment $\mu$ satisfies a formula $\vi$}'' as
% ``$\mu$ {\em entails} $\vi$''
% (i.e. ``all total assignments extending $\mu$
% satisfy $\vi$''). \RSTODO{Dire quali: preserve equivalence.}
% %
% Practical condiderations suggest instead to interpretate \RSTODO{completare}



Based on the considerations above, not only we suggest to adopt
entailment 
 rather than \verbverification{} as unique definition of partial-assignment
 satisfiability, but also we champion its usage inside
 enumeration-based search
 procedures. %(See related work below and \sref{sec:practical}.)
 %
 \ignore{
To this extent, in the last years we have proposed techniques for efficiently implementing
 entailment within enumeration
 procedures~\cite{moehle20,moehle21,friedEntailingGeneralizationBoosts2024},
 which are mostly based on \cite{mohleDualizingProjectedModel2018};
 in particular, in \cite{friedEntailingGeneralizationBoosts2024} we
 have enhanced the enumeration tool for circuits from
 \cite{friedAllSATCombinationalCircuits2023} by substituting
 \verbverification{} checks with entailment checks, obtaining drastic
 improvements in terms of both time efficiency and size of 
 partial-assignment sets .
}
\input{related}
 
\paragraph{Content.} The rest of the paper is organized as follows.
\sref{sec:background} provides the necessary notation, terminology
and concepts used in the paper.
\sref{sec:partialsat} presents our theoretical analysis:
\sref{sec:partialsat-plain}
introduces \verbverification{} and entailment
 for generic propositional formulas and discusses their
 relative properties;
 \sref{sec:partialsat-others} analyzes other candidate forms of partial-assignment satisfaction;
\sref{sec:partialsat-exist} lifts the discussion to
existentially-quantified formulas;
\sref{sec:partialsat-cnf} discusses the role of CNF-ization in this
context.
\sref{sec:practical} discusses the practical consequences
of entailment vs. \verbverification{}.
\sref{sec:concl} provides some conclusions and suggestions for future research.


\ignore{
 . Although entailment  is more expensive, it does not
 suffer for the ''embarrassing'' theoretical weakness mentioned above.
Overall, the theoretical considerations above suggest to adopt entailment
 rather \verbverification{} as general definition of partial-assignment satisfiability, although
  \verbverification{} is a cheaper though less-effective criterion which can 
  (most) often be adopted in
  actual implementations. 
%
  Moreover, since partial assignments entailing $\vi$ are in general
  subsets of those \verbverifying{} $\vi$, using entailment rather
  than \verbverification{} as satisfiability criterion allows for
  producing smaller partial assignments, and hence possibly
  drastically reducing their number, in particular in the presence of
  existentially-quantified formulas.  This suggests the development
  of more effective assignment-enumeration algorithms.
}
  % 
% When it comes to enumerating, in order to maximizing efficiency
% we would like to produce  partial assignments
% entailing the input formula, although most 
% algorithms give us only partial assignments
% \verbverifying{} it.



%\TODO{Aggiungi riferimento a poll.\\}
\ignore{
\paragraph{A poll.}
In order to support the analysis, I've set up an email
poll among some current or past SAT PC and some SMT PC members, asking
for the truth/falsehood of five statements on the
notion of partial-assignment satisfiability.
The result are available at \cite{poll} %
%\footnote{\url{http://disi.unitn.it/rseba/partialsat_poll_2019.03.11.pdf}}
 and as an appendix submitted with this paper. 
Although only 20 out of 65 people replied, 
the result 
reveals the lack of general agreement among the repliers on the notion of
partial-assignment satisfiability and on its consequences: e.g.,
% since 
the repliers split evenly into supporters 
of entailment, of \verbverification{}, and people considering them equivalent.
}

%\TODO{Aggiungere related work paragraph? Menzionare papers \cite{moehle20,moehle21}}

\ignore{
  \paragraph{Motivation.} The analysis presented in this paper was
\RSTODO{Tagliare questo paragrafo}
triggered
by the effort of conceiving more efficient procedures for predicate
abstraction in SMT for improving Weighted Model Integration
\cite{morettin_aij19,spallittaEnhancingSMTbasedWeighted2024a},
which forced me to elaborate on the distinction between 
\verbverification{} and entailment. Before then, I have
always used to see 
partial-assignment satisfiability as {entailment}
 (see \cite{gs-infocomp2000,sebastiani07,SebastianiT21}) without paying attention to this distinction.
}


\ignore{
Schema

* need for partial assignment
* in this paper we analyze
From a theoretical viewpoint:
* no agreed definition of pa-s
  - most do not define it
  - some defini for cnf only
  - onfly a few do, leadind to different: verify and entail
* we notice two possible definitions from the literature:
verification and entailment (cita)
  - for CNF they are the same
  - for non-CNF different
  
}


==> arxiv-version/intro.tex.1 <==
% Although  CDCL 
% \cite{MSLM09HBSAT} 
% and SLS \cite{Maj09HBSAT} SAT solvers return  {\em total} truth assignments
% satisfying the input formula, other SAT procedures 
Many procedures for for SAT and SAT-related problems
(e.g. OBDDs
\cite{bryant2}, Analytic Tableaux \cite{smullyan1}, DPLL
\cite{davis7}) rely their efficiency
on the detection of {\em partial} assignments satisfying an input
formula.
In particular,
when it comes to SAT-based problems requiring
the complete enumeration of satisfying assignments (e.g. \#SAT
\cite{GSS09HBSAT}, Lazy SMT \cite{BSST09HBSAT}, AllSAT and AllSMT
\cite{allsmt}, satisfiability of modal and description logics
\cite{ST09HBSAT}), the capability of enumerating  {\em
partial}  satisfying assignments which are as small as possible is often essential, because 
detecting that a partial assignment satisfies the input formula 
may avoid the enumeration of the whole subtree
of total assignments extending it, whose size is exponential in the
number of unassigned propositions.

% a satisfying partial
% assignment can be generated instead of the whole subtree
% of total assignments extending it, whose size is exponential in the
% number of unassigned propositions.

% When we deal with (tautology-free) CNF formulas, the notion of
% partial-assignment satisfiablity is clear SPIEGA E CITA. BOTH PROPERTIES

In this paper we analyze in deep the notion of partial-assignment
satisfiability. 
First we raise a flag on the fact that by
``{\em a partial truth assignment $\mu$ satisfies a formula $\vi$}'',
we may mean either that $\mu$ {\em entails} $\vi$
(i.e. that all total assignments extending $\mu$
satisfy $\vi$) or that $\mu$ {\em validates} $\vi$
 (i.e. that applying $\mu$ to $\vi$ makes $\vi$ true).
%
Typically most authors in the SAT community
leave this definition
implicit, or provide a definition only for (tautology-free) CNF
formulas (e.g. \cite{KBK09HBSAT}).
% where we notice that
% entailment and validation concide. 
%
We notice that, whereas for (tautology-free) CNF formulas entailment 
and validation are equivalent, for non-CNF formulas --and for
existentially-quantified formulas, even CNF ones--
{\em validation is strictly stronger than entailment}, and they have
complementary properties. 

We also notice that 
 (Tseitin-style) CNF-ization does not solve this
issue, because 
%with Tseitin CNF-ization 
it may lose 
information regarding partial-assignment entailment or validation.
%\ignoreinshort{\RSTODO{Mention Kripke \& C e Stefano Tonetta?}}
%We stress the fact that the 

We stress the fact that the distinction between entailment and validation
is not just an issue of terminology; rather, it 
has important consequences at
algorithmic level. 
%
We notice, e.g., that
OBDDs \cite{bryant2} implicitly enumerate partial assignment {\em entailing}
the input formulas, whereas Analytic Tableaux \cite{smullyan1} and
(non-CNF) DPLL \cite{davis7} implicitly enumerate partial assignment
{\em validating} it. 
%
Also, e.g., techniques like {\em pure-literal
filtering} 
%and {\em ghost-literal filtering} 
\cite{sebastiani07,BSST09HBSAT} in lazy
SMT 
implicitly aim at reducing a
total assignment to a partial one {\em validating} the input formula. 
%
On the one hand, checking entailment is computationally
much harder than checking
validation. On the other hand, since partial assignments entailing
$\vi$ are in general subsets of those validating $\vi$, being able
to produce  partial assignments
{\em entailing} the input formula rather than {\em validating} it
 allows for producing smaller partial assignments,
and hence possibly drastically reducing their number. 
This may drive the development of more effective assignment-enumeration algorithms.
%
% When it comes to enumerating, in order to maximizing efficiency
% we would like to produce  partial assignments
% entailing the input formula, although most 
% algorithms give us only partial assignments
% validating it.

%\RSTODO{Aggiungi riferimento a poll.\\}
\ignore{
\paragraph{A poll.}
In order to support the analysis, I've set up an email
poll among some current or past SAT PC and some SMT PC members, asking
for the truth/falsehood of five statements on the
notion of partial-assignment satisfiability.
The result are available at \cite{poll} %
%\footnote{\url{http://disi.unitn.it/rseba/partialsat_poll_2019.03.11.pdf}}
 and as an appendix submitted with this paper. 
Although only 20 out of 65 people replied, 
the result 
reveals the lack of general agreement among the repliers on the notion of
partial-assignment satisfiability and on its consequences: e.g.,
% since 
the repliers split evenly into supporters 
of entailment, of validation, and people considering them equivalent.
}


\paragraph{Personal note.} The analysis presented in this paper was
triggered
by the effort of conceiving more efficient procedures for predicate
abstraction in SMT for improving Weighted Model Integration
\cite{MorPasSeb17,morettin_aij19},
which forced me to elaborate on the distinction between entailment
and validation. Before then, I personally used to see
partial-assignment satisfiability as {entailment}
 (see \cite{gs-infocomp2000}) without paying attention to the distinction.

{\paragraph{Content.} The rest of the paper is organized as follows.
\sref{sec:background} provides the necessary notation, terminology
and concepts used in the paper.
\sref{sec:partialsat} introduces entailment and
validation for generic propositional formulas and discusses their
relative properties and use.
\sref{sec:partialsat-exist} lifts the discussion to
existentially-quantified formulas.
\sref{sec:concl} provides some conclusions and future-work suggestions.
}



==> arxiv-version/intro_v1.tex <==
% Although  CDCL 
% \cite{MSLM09HBSAT} 
% and SLS \cite{Maj09HBSAT} SAT solvers return  {\em total} truth assignments
% satisfying the input formula, other SAT procedures 
Many procedures for for SAT and SAT-related problems
(e.g. OBDDs
\cite{bryant2}, Analytic Tableaux \cite{smullyan1}, DPLL
\cite{davis7}) rely their efficiency
on the detection of {\em partial} assignments satisfying an input
formula.
In particular,
when it comes to SAT-based problems requiring
the complete enumeration of satisfying assignments (e.g. \#SAT
\cite{GomesSS21}, Lazy SMT \cite{BarrettSST21}, AllSAT and AllSMT
\cite{allsmt}, satisfiability of modal and description logics
\cite{SebastianiT21}), the capability of enumerating  {\em
partial}  satisfying assignments which are as small as possible is often essential, because 
detecting that a partial assignment satisfies the input formula 
may avoid the enumeration of the whole subtree
of total assignments extending it, whose size is exponential in the
number of unassigned propositions.

% a satisfying partial
% assignment can be generated instead of the whole subtree
% of total assignments extending it, whose size is exponential in the
% number of unassigned propositions.

% When we deal with (tautology-free) CNF formulas, the notion of
% partial-assignment satisfiablity is clear SPIEGA E CITA. BOTH PROPERTIES

In this paper we analyze in deep the notion of partial-assignment
satisfiability. 
First we raise a flag on the fact that by
``{\em a partial truth assignment $\mu$ satisfies a formula $\vi$}'',
we may mean either that $\mu$ {\em entails} $\vi$
(i.e. that all total assignments extending $\mu$
satisfy $\vi$) or that $\mu$ {\em verifies} $\vi$
 (i.e. that applying $\mu$ to $\vi$ makes $\vi$ true).
%
Typically most authors in the SAT community
leave this definition
implicit, or provide a definition only for (tautology-free) CNF
formulas (e.g. \cite{BuningK21}).
% where we notice that
% entailment and verification concide. 
%
We notice that, whereas for (tautology-free) CNF formulas entailment 
and verification are equivalent, for non-CNF formulas --and for
existentially-quantified formulas, even CNF ones--
{\em verification is strictly stronger than entailment}, and they have
complementary properties. 

We also notice that 
 (Tseitin-style) CNF-ization does not solve this
issue, because 
%with Tseitin CNF-ization 
it may lose 
information regarding partial-assignment entailment or verification.
%\ignoreinshort{\RSTODO{Mention Kripke \& C e Stefano Tonetta?}}
%We stress the fact that the 

We stress the fact that the distinction between entailment and verification
is not just an issue of terminology; rather, it 
has important consequences at
algorithmic level. 
%
We notice, e.g., that
OBDDs \cite{bryant2} implicitly enumerate partial assignment {\em entailing}
the input formulas, whereas Analytic Tableaux \cite{smullyan1} and
(non-CNF) DPLL \cite{davis7} implicitly enumerate partial assignment
{\em verifying} it. 
%
Also, e.g., techniques like {\em pure-literal
filtering} 
%and {\em ghost-literal filtering} 
\cite{sebastiani07,BarrettSST21} in lazy
SMT 
implicitly aim at reducing a
total assignment to a partial one {\em verifying} the input formula. 
%
On the one hand, checking entailment is computationally
much harder than checking
verification. On the other hand, since partial assignments entailing
$\vi$ are in general subsets of those verifying $\vi$, being able
to produce  partial assignments
{\em entailing} the input formula rather than {\em verifying} it
 allows for producing smaller partial assignments,
and hence possibly drastically reducing their number. 
This may drive the development of more effective assignment-enumeration algorithms.
%
% When it comes to enumerating, in order to maximizing efficiency
% we would like to produce  partial assignments
% entailing the input formula, although most 
% algorithms give us only partial assignments
% verifying it.

%\RSTODO{Aggiungi riferimento a poll.\\}
\ignore{
\paragraph{A poll.}
In order to support the analysis, I've set up an email
poll among some current or past SAT PC and some SMT PC members, asking
for the truth/falsehood of five statements on the
notion of partial-assignment satisfiability.
The result are available at \cite{poll} %
%\footnote{\url{http://disi.unitn.it/rseba/partialsat_poll_2019.03.11.pdf}}
 and as an appendix submitted with this paper. 
Although only 20 out of 65 people replied, 
the result 
reveals the lack of general agreement among the repliers on the notion of
partial-assignment satisfiability and on its consequences: e.g.,
% since 
the repliers split evenly into supporters 
of entailment, of verification, and people considering them equivalent.
}


\paragraph{Personal note.} The analysis presented in this paper was
triggered
by the effort of conceiving more efficient procedures for predicate
abstraction in SMT for improving Weighted Model Integration
\cite{MorPasSeb17,morettin_aij19},
which forced me to elaborate on the distinction between entailment
and verification. Before then, I personally used to see
partial-assignment satisfiability as {entailment}
 (see \cite{gs-infocomp2000}) without paying attention to the distinction.

{\paragraph{Content.} The rest of the paper is organized as follows.
\sref{sec:background} provides the necessary notation, terminology
and concepts used in the paper.
\sref{sec:partialsat} introduces entailment and
verification for generic propositional formulas and discusses their
relative properties and use.
\sref{sec:partialsat-exist} lifts the discussion to
existentially-quantified formulas.
\sref{sec:concl} provides some conclusions and future-work suggestions.
}



==> arxiv-version/intro_v2.tex <==
% Although  CDCL 
% \cite{MSLM09HBSAT} 
% and SLS \cite{Maj09HBSAT} SAT solvers return  {\em total} truth assignments
% satisfying the input formula, other SAT procedures 

\TODO{Cambiare la narrazione:
\\- we wish... however...
\\- Proporre da
qualche parte ``satisfy'' as ``entailment''.
\\- far notare come
tipicamente evaluation to true.
}

 \newpage
\marg{need for PAS}
Many procedures for SAT and SAT-related problems
(e.g. OBDDs
\cite{bryant2}, Analytic Tableaux \cite{smullyan1}, DPLL
\cite{davis7}) rely their efficiency
on the detection of {\em partial} truth assignments $\mu$  satisfying an input
 propositional formula $\vi$, which allows to
state that (i) $\vi$ is satisfiable and (ii) all total 
assignments extending $\mu$ satisfy \vi. 
% state not only that $\vi$ is satisfiable, but also that all total 
% assignments extending $\mu$ satisfy \vi. 
In particular,
when it comes to SAT-based problems requiring
the {\em complete enumeration} of satisfying assignments (e.g. \#SAT
\cite{GomesSS21}, Lazy SMT \cite{BarrettSST21}, AllSAT and AllSMT
\cite{allsmt}, satisfiability of modal and description logics
\cite{SebastianiT21}, Weighted Model Integration \cite{MorPasSeb17}),
%
the ability of enumerating satisfying {partial} assignments which are
as small as possible is essential, because
%detecting that a partial assignment satisfies the input formula 
each of them
avoids the enumeration of the whole subtree
of total assignments extending it, whose size is exponential in the
number of unassigned propositions.

\marg{no definition}
Surprisingly,
% despite its widespread (implicit) usage of
% partial-assignment satisfiablity
% in algorithms and
%apart from the case of (tautology-free) CNF formulas,
there seems to be no general and universally-agreed definition of
partial-assignment satisfaction:
most authors do not
define partial-assignment satisfaction explicitly, or define it only when dealing with
(tautology-free) CNF formulas (e.g.  \cite{BuningK21});
%
\marg{algos diff notions}
also, different algorithms implictly implement different notions of
partial-assignment satisfaction (see below).
%
% In order to be useful, such a definition should at least guarantee
% that, if a partial assignment $\mu$ satisfies a formula \vi, then (i)
% \vi is satisfiable and (ii) all total truth assignments extending it
% satisfy \vi.~%\footnote{

%\begin{remark}
We stress the fact that this is not simply an issue of
the meaning of the word ``satisfy'': whichever ``verb'' one
might  use for it (e.g. ``satisfy'', ``entail'', ``imply'', ``evaluate to
true'',...), we would like a universally-agreed criterion
to extablishing that, if a partial truth-assignment ``verbs'' a formula
$\vi$, then (i) $\vi$ is satisfiable and (ii) all total truth
 assignments extending it satisfy $\vi$. 
\ignore{
we need a universally-agreed criterion
 complying with the two conditions (i) and (ii)
above.
} 
%\end{remark}
%}
% a criterion the sentence
% ``a partial truth assignment $\mu$ [verb] a formula $\vi$'' should
% imply that (i) \vi is satisfiable and (ii) that all total truth
% assignments extending it satisfy \vi. 

% a satisfying partial
% assignment can be generated instead of the whole subtree
% of total assignments extending it, whose size is exponential in the
% number of unassigned propositions.

% When we deal with (tautology-free) CNF formulas, the notion of
% partial-assignment satisfiablity is clear SPIEGA E CITA. BOTH PROPERTIES

\ignore{In this paper 
analyze in deep the notion of partial-assignment
satisfiability,
raising  a flag about the ambiguities and subtleties
of this concept,
and highlighting their practical consequences.

In this paper we
raise  a flag about the ambiguities and subtleties
of partial-assignment
satisfiability, in particular for  non-CNF or
existentially-quantified formulas, 
and investigate their practical consequences.
}
%\TODO{We wish to fill this gap...}

\RSTODO{move up?}
In this paper we want to address this issue explicitly. We
analyze the notion of partial-assignment
satisfiability,
raising  a flag about the ambiguities and subtleties
of this concept  --in particular when dealing with  non-CNF and
existentially-quantified formulas-- 
and we investigate their practical consequences.

\marg{$\entails$ vs. $\verifies$}
We start by noticing the following fact:
whereas for (tautology-free) CNF formulas
``{\em a partial truth assignment $\mu$ satisfies a formula $\vi$}''
may be indifferently be interpreted either as 
``$\mu$ {\em entails} $\vi$''
(i.e. ``all total assignments extending $\mu$
satisfy $\vi$'') or as ``$\mu$ {\em \verbverifies{}} $\vi$''
 (i.e. ``applying $\mu$ to $\vi$ makes $\vi$ true'') because in this
 case the two  concepts are equivalent,
 %
 for non-CNF formulas instead --and for
existentially-quantified formulas, even CNF ones--
{\em \verbverification{} is strictly stronger than entailment}, and they have
complementary properties. 
%
\ignore{
First we raise a flag on the fact that by
``{\em a partial truth assignment $\mu$ satisfies a formula $\vi$}'',
we may mean either that $\mu$ {\em entails} $\vi$
(i.e. that all total assignments extending $\mu$
satisfy $\vi$) or that $\mu$ {\em \verbverifies{}} $\vi$
 (i.e. that applying $\mu$ to $\vi$ makes $\vi$ true).
%
Typically most authors in the SAT community
leave this definition
implicit, or provide a definition only for (tautology-free) CNF
formulas (e.g. \cite{BuningK21}).
% where we notice that
% entailment and \verbverification{} concide. 
%
We notice that, whereas for (tautology-free) CNF formulas entailment 
and \verbverification{} are equivalent, for non-CNF formulas --and for
existentially-quantified formulas, even CNF ones--
{\em \verbverification{} is strictly stronger than entailment}, and they have
complementary properties. 
}
We also notice that standard
 (Tseitin-style) CNF-ization does not solve this
issue, because 
%with Tseitin CNF-ization 
it may lose 
information regarding partial-assignment entailment or \verbverification{}.
%\ignoreinshort{\TODO{Mention Kripke \& C e Stefano Tonetta?}}
%We stress the fact that the 

We also stress the fact that the distinction between entailment and \verbverification{}
is not only an issue of providing an universally-agreed definition of
partial-assignment satisfiability, but it also 
has important practical consequences. 
%
\RSTODO{Aggiungere $\verifies$ vs. equivalence}
\RSTODO{Although...}
On the one hand, checking entailment is computationally
much harder than checking
\verbverification{}. On the other hand, since partial assignments entailing
$\vi$ are in general subsets of those \verbverifying{} $\vi$, being able
to produce  partial assignments
{entailing} the input formula rather than {\verbverifying{}} it
 allows for producing smaller partial assignments,
and hence possibly drastically reducing their number. 
This may drive the development of more effective assignment-enumeration algorithms.
%
% When it comes to enumerating, in order to maximizing efficiency
% we would like to produce  partial assignments
% entailing the input formula, although most 
% algorithms give us only partial assignments
% \verbverifying{} it.

\marg{algos different notions of PAS}
To this extent we notice, e.g., that, when applied to non-CNF
formulas, 
OBDDs \cite{bryant2} implicitly enumerate partial assignment {entailing}
the input formulas,  whereas other procedures like Analytic Tableaux \cite{smullyan1} and
(non-CNF) DPLL \cite{davis7} implicitly enumerate partial assignment
{\verbverifying{}} them. 
%
Also, e.g., techniques like {\em pure-literal
filtering} 
%and {\em ghost-literal filtering} 
\cite{sebastiani07,BarrettSST21} in lazy
SMT 
implicitly aim at reducing a
total assignment to a partial one {\verbverifying{}} the input formula. 


%\TODO{Aggiungi riferimento a poll.\\}
\ignore{
\paragraph{A poll.}
In order to support the analysis, I've set up an email
poll among some current or past SAT PC and some SMT PC members, asking
for the truth/falsehood of five statements on the
notion of partial-assignment satisfiability.
The result are available at \cite{poll} %
%\footnote{\url{http://disi.unitn.it/rseba/partialsat_poll_2019.03.11.pdf}}
 and as an appendix submitted with this paper. 
Although only 20 out of 65 people replied, 
the result 
reveals the lack of general agreement among the repliers on the notion of
partial-assignment satisfiability and on its consequences: e.g.,
% since 
the repliers split evenly into supporters 
of entailment, of \verbverification{}, and people considering them equivalent.
}


\paragraph{Motivation.} The analysis presented in this paper was
triggered
by the effort of conceiving more efficient procedures for predicate
abstraction in SMT for improving Weighted Model Integration
\cite{MorPasSeb17,morettin_aij19},
which forced me to elaborate on the distinction between entailment
and \verbverification{}. Before then, I personally used to see
partial-assignment satisfiability as {entailment}
 (see \cite{gs-infocomp2000}) without paying attention to the distinction.

{\paragraph{Content.} The rest of the paper is organized as follows.
\sref{sec:background} provides the necessary notation, terminology
and concepts used in the paper.
\sref{sec:partialsat} introduces entailment and
\verbverification{} for generic propositional formulas and discusses their
relative properties and use.
\sref{sec:partialsat-exist} lifts the discussion to
existentially-quantified formulas.
\sref{sec:concl} provides some conclusions and future-work suggestions.
}



==> arxiv-version/partialsat-exist.tex <==
\subsection{\Verbverification{} and entailment of
  existentially-quantified formulas.}
\label{sec:partialsat-exist}

We extend the analysis of \sref{sec:partialsat-plain} to
existentially-quantified propositional formulas, %, and
% wonder about the meaning of 
% the sentence ``a \emph{partial} assignment $\mu$ satisfies 
% $\exists\allb\psi$".
 wishing to provide a satisfactory definition of partial-assignment
 satisfiability for this case as well.
Property~\ref{prop:total-shannon} paves our way, telling how to
extend the 
definitions of \verbverification{} and entailment
to existentially-quantified formulas. 

%property~\ref{prop:total-shannon} provides a natural way to leverage

The first possibility is to see partial-assignment satisfiability as
{\em \verbverification}, leveraging Definition~\ref{def:verification}
%and property~\ref{prop:total-shannon}
to the existentially-quantified
case by exploiting  Shannon expansion.
% By \eqref{eq:shannon} and
% Definition~\ref{def:verification},
% $\mu\verifies{} \shannonpsib$ iff
% \apply{(\shannonpsib)}{\mu} is $\top$, that is, iff there exists some
%  $\delta_i$ s.t. \apply{\apply{\psi}{\delta_i}}{\mu} is $\top$, that
%  is, iff there exists some $\delta_i$ s.t. $\mu\cup\delta_i$ \verbverifies{} $\psi$. 
%
%This leads to the following definition and relative property. 
%
\begin{definition}
\label{def:verification-exist}
 We say that a {\em partial} truth assignment $\mu$ on $\alla$ {\bf
   \verbverifies} $\exists
\allb.\psi$ if and only if, there exists a total truth assignment 
$\delta$ on $\allb$ s.t.
\ignore{the result of applying $\mu\cup\delta$ to 
$\psi$ is $\top$, that is,}
$\mu\cup\delta\verifies\psi$, that is, $\apply{\psi}{\mu\cup\delta}=\top$.
%\RSTODO{YES $\verifies$}
\end{definition}


\begin{theorem}
\label{prop:verification-exist}
Let   $\psi$ be a formula on
$\alla\cup\allb$ and $\mu$ be a partial assignment on \alla.
% and $\delta_i$ be total truth assignments on \allb. 
Then\\
%\begin{renumerate}
%\item
  $\mu\verifies\exists \allb. \psi$ iff $\mu\verifies\shannonpsib$. 
%\end{renumerate}
\end{theorem}

\begin{proof}
 By Definition~\ref{def:verification},  $\mu\verifies{} \shannonpsib$ iff
 $\apply{(\shannonpsib)}{\mu} = \top$, \\
 that is, 
 by \eqref{eq:shannon},
 iff there exists some
 $\delta_i$ s.t. $\apply{\apply{\psi}{\delta_i}}{\mu}=\top$ (i.e., $\apply{\psi}{\delta_i\cup\mu}=\top$),
 \\ that is, by Definition~\ref{def:verification}, iff there exists some $\delta_i$ s.t. $\mu\cup\delta_i\verifies\psi$,
 \\ that is, by Definition~\ref{def:verification-exist}, iff
 $\mu\verifies\exists \allb. \psi$.
 \hfill $\qed$
\end{proof}
\noindent Notice  that \cref{prop:verification-exist} is
{\em not} a straighforward consequence of
property~\ref{prop:total-shannon}, because equivalent formulas are not
necessarily verified by the same assignments
(property~\ref{prop:partial-verification}(ii)). 

One second possibility is to see partial-assignment satisfiability as
{\em entailment}, leveraging Definition~\ref{def:entailment}
and property~\ref{prop:total-shannon} to the existentially-quantified
case. %
This leads to the following definition and relative property. 
%
\begin{definition}
\label{def:entailment-exist}
We say that a {\em partial} truth assignment $\mu$ on $\alla$ {\bf entails}
$\exists \allb.\psi$, written $\mu\entails\exists \allb.\psi$,
if and only if , for every total truth assignment $\eta$ on $\alla$ 
extending $\mu$,
there exists a total truth assignment $\delta$ on $\allb$
s.t. $\eta\cup\delta$ satisfies $\psi$. 
%\RSTODO{YES $\entails$}
\end{definition}

\begin{theorem}
\label{prop:entailment-exist}
Let   $\psi$ be a formula on
$\alla\cup\allb$ and $\mu$ be a partial assignment on \alla.
% and $\delta_i$ be total truth assignments on \allb. 
Then\\
% \begin{renumerate}
% \item
  $\mu\entails\exists \allb. \psi$ iff $\mu\entails\shannonpsib$. 
% \end{renumerate}
\end{theorem}

\begin{proof}
  $\mu\entails \shannonpsib$ iff $\eta\models\shannonpsib$ for every total
assignment $\eta$ s.t. $\eta\supseteq\mu$, 
that is, by property~\ref{prop:total-shannon}, iff for every total
assignments $\eta$ s.t. $\eta\supseteq\mu$ exists a total assignment 
$\delta$ on \allb s.t. $\eta\cup\delta\models\psi$, that is, iff
$\mu\entails\exists \allb. \psi$. \hfill $\qed$
\end{proof}

%\begin{IGNOREINSHORT}
%\begin{remark}
%\label{remark:nestingorder}
  \noindent
  Notice the nesting order of forall/exists in
Definition~\ref{def:entailment-exist}: ``for every $\eta$ exists $\delta$
s.t. ...''. In fact, distinct $\eta$'s may satisfy distinct disjuncts 
$\apply{\psi}{\delta_i}$ in \shannonpsib{}, requiring distinct 
$\delta_i$'s.
\ignore{Therefore, we notice that the following statement, inverting the
quantification order, is \emph{not} a suitable definition for $\mu\entails\exists \allb.\psi$:
%
%\\
\\ \noindent
% {\bf (wrong) Definition.}
  ``{\em We say that a {\em partial} truth assignment $\mu$ on $\alla$ entails
  $\exists \allb.\psi$ if and only if, there exists a total truth
  assignment $\delta$ on $\allb$ s.t., for every total truth assignment
  $\eta$ extending $\mu$, $\eta\cup\delta$ satisfies $\psi$.}''
}
%\hfill $\diamond$
%\RSTODO{NO}
%\end{definition}
% 
%\end{remark}  
%\end{IGNOREINSHORT}



\begin{theorem}
\label{prop:stronger-exists}
Let $\psi$ be a formula on $\alla\cup\allb$ and $\mu$ be a partial truth
assignment over $\alla$.
Then
$\mu\entails\exists\allb.\psi$ if $\mu\verifies\exists\allb.\psi$, but
the converse does not hold. %, even if $\psi$ is tautology-free CNF.
\end{theorem}
\begin{proof}
  %Let $\vi\defas \shannonpsib{}$.
  From
  \cref{prop:stronger}$(b)$ with $\vi\defas \shannonpsib{}$
  we can deduce that $\mu\entails\shannonpsib{}$ if
  $\mu\verifies\shannonpsib{}$.
%   , but
% the converse does not hold.
By \cref{prop:verification-exist} and
\cref{prop:entailment-exist} we have that $\mu\entails\exists\allb.\psi$ if $\mu\verifies\exists\allb.\psi$.
\\The fact that the converse does not hold is shown in \cref{ex:exists-stronger}.
\hfill $\qed$
\end{proof}



% , that is,
% $\mu\verifies\exists\allb.\psi$ implies
% $\mu\entails\exists\allb.\psi$, {but not vice versa}.
% ,
% that is, \verbverification is strictly stronger than entailment even 
% %(Definition~\ref{def:verification-exist})
% is strictly
% stronger than $\mu\entails\exists\allb.\psi$.
% % (Definition~\ref{def:entailment-exist}).
\noindent


\begin{example}
\label{ex:exists-stronger}
  Consider $\mu\defas\set{A_1}$
  and the tautology-free CNF formula on $\alla\cup\allb$:\\
$
\begin{array}{lll}
\psi\defas  
& (B_1\vee B_2)\ \wedge & \\
& (\neg B_1 \vee \pos A_1) \wedge
(\neg B_1 \vee \pos A_2) \wedge
(B_1\vee \neg A_1 \vee \neg A_2)\ \wedge\ & \ \ \ \\
& (\neg B_2 \vee \pos A_1) \wedge
(\neg B_2 \vee \neg A_2) \wedge
(B_2\vee \neg A_1 \vee \pos A_2).\ & \ \ \ 
\\
  \shannonpsib= &
  \xcancel{(A_1\wedge A_2\wedge\neg A_2)}\vee (A_1\wedge A_2)\vee (A_1\wedge\neg A_2) 
\vee \xcancel{\bot}.\\
\end{array}
$\\
% We have that 
% $\shannonpsib=
% %
% \xcancel{(A_1\wedge A_2\wedge\neg A_2)}\vee (A_1\wedge A_2)\vee (A_1\wedge\neg A_2) 
% \vee \xcancel{\bot}
% $ %(the other disjunct is $\bot$)
Thus $\mu\entails\shannonpsib$ but 
$\mu\not\verifies\shannonpsib$,
so  that $\mu\entails\exists\allb.\psi$ but
$\mu\not\verifies\exists\allb.\psi$.
\hfill $\diamond$
\end{example}

Thus
\verbverification{} is strictly stronger than entailment also with
existentially-quantified formulas.
%
Remarkably, and unlike with the un-quantified case, this is the case 
 \emph{even if $\psi$ is a tautology-free CNF formula}! (See \cref{ex:exists-stronger}.)
Intuitively, this can be seen as a consequence of the fact that 
\shannonpsib is not in CNF even if $\psi$ is in CNF. 
%This is shown


%\RSTODO{Aggiungi esempio.}

% \TODO{Same embarassing problem: if $\exists \allb \vi_1 \equiv \exists
%   \allb \vi_2$, $\mu\verifies\vi_1$ does not imply $\mu\verifies\vi_2$.}

% \RSTODO{for $\exists \psi$, $\entails$ and $\verifies$ different
% even if $\vi$ CNF. CHECK!}
%\RSTODO{Speak of predicate abstraction. SMT?}
%\newpage



==> arxiv-version/partialsat-predabs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% A Relevant Example Application: Predicate Abstraction.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{A Relevant Example Application: Predicate Abstraction.}
\label{sec:partialsat-predabs}
% {\em Predicate abstraction}
% (see e.g. \cite{graf_predabs97,lahiriSMTTechniquesFast2006,cavada_fmcad07_predabs})
% has a crucial role in SW verification.
%\RSTODO{Estendere a SMT?} 
 
Given a propositional formula $\phi$ on $\allb$ and a set
%\RSTODO{TODO: Revise this subsection. }
$\mathbf{\Phi}\defas\set{\phi_i}_{i}$ of formulas on $\allb$ denoting relevant
``predicates'' and a set $\alla$ of fresh atom s.t. each $A_i$
labels $\phi_i$, 
then the {\em Predicate Abstraction} of $\phi$ wrt. $\mathbf{\Phi}$ is
defined as follows \cite{graf_predabs97}:
\begin{eqnarray}
  \label{eq:predabs}
 \predabsphi \defas
\exists \allb. %\left 
( \phi \wedge \bigwedge_{i} (A_i\iff \phi_i)
%\right 
) .
\end{eqnarray}
 \predabsphi{}
is typically computed as {\em projected anumeration}, i.e., as a disjunction of mutually-inconsistent partial
assignments (cubes) $\mu_j$ on \alla s.t. $\mu_j\entails
\predabsphi$ and 
$\bigvee_j\mu_j$ is equivalent to \predabsphi
\cite{lahiriSMTTechniquesFast2006,cavada_fmcad07_predabs}.
\footnote{Notice that predicate Abstraction is most often referred to SMT formulas
  $\phi$ and $\set{\phi_i}_i$, so that \eqref{eq:predabs} involves
  also the existential quantification of first-order theory-specific variables
  and $\mu_i$ are theory-consistent SMT assignments
  \cite{graf_predabs97,lahiriSMTTechniquesFast2006,cavada_fmcad07_predabs}.
However, restricting our discussion to the purely-propositional case suffices for our
purposes and makes the explanation much simpler.}

We notice that in the computation of such cubes the distinction between $\verifies$ and
$\entails$ may be very relevant: whereas %to comply with the definition,
it would be desirable to look for partial assignments $\mu_j$ %on $\alla$ 
{\em entailing} \predabsphi{}  to keep them small and hence reduce
their number,
% s.t. $\mu_j\entails\predabsphi$.
 most algorithms can reveal
%partial-assignment satisfaction
only when $\mu_j$ 
{\em \verbverifies{}} it, and 
are thus
incapable of producing partial assignments 
$\mu_j$ s.t. $\mu_j\entails\predabsphi$ and
$\mu_j\not\verifies\predabsphi$.
%
This happens every time that, % above issue raises by the fact that it may well be the case that,
for some $A_k$ and some $\mu^k$
on (subsets  of) $\alla\setminus \set{A_k}$,
{\em both} 
$\apply{(\phi\wedge\bigwedge_{i\neq k}(A_i\iff \phi_i))}{\mu^k} \wedge \phi_k$
and 
$\apply{(\phi\wedge\bigwedge_{i\neq k}(A_i\iff \phi_i))}{\mu^k} \wedge
\neg \phi_k$
 are satisfiable but they are satisfied by {\em distinct} sets of assignmets
 $\delta$ on \allb (Definition~\ref{def:entailment-exist}), so that
 $\mu_k\entails\predabsphi$ but 
 $\mu_k\not\verifies\predabsphi$.

\begin{example}
Consider the CNF formula
$\phi\defas(\neg B_1\vee B_2)\wedge (B_1\vee \neg B_2)$
and the ''predicate'' CNF formulas
$\Phi_1\defas B_1\wedge B_2$ and
$\Phi_2\defas \neg B_1\wedge B_2$.
Then
\begin{eqnarray}
  \label{eq:predabs1}
  \predabsphi &\defas & \exists B_1 B_2. \left (
 \begin{array}{lll}
(\neg B_1\vee B_2)\wedge (B_1\vee \neg B_2) & \wedge \\
(A_1 \iff (B_1\wedge B_2)) & \wedge \\
(A_2 \iff (B_1\wedge \neg B_2))
 \end{array}
  \right )
  \\
  \label{eq:predabs2}
  &\Leftrightarrow& (A_1 \wedge \neg A_2) \vee (\neg A_1 \wedge \neg A_2) 
  \\
  \label{eq:predabs3}
  &\Leftrightarrow& \neg A_2
\end{eqnarray}
Both \set{A_1,\neg A_2} and \set{\neg A_1,\neg A_2}
\verbverify{} \predabsphi,
whereas  \set{A_1} entails it without \verbverifying{} it.
Thus, if the algorithm is able to detect if
% a partial assignment $\mu_j$ is s.t.
$\mu_j\entails\predabsphi$ and
$\mu_j\not\verifies\predabsphi$, then it can return \eqref{eq:predabs3},
otherwise it can only return \eqref{eq:predabs2}.
\hfill $\diamond$
\end{example}

%  This is as shown
% in the next example
% 
 % $\mu_k\wedge A_k\verifies\predabsphi$
 % $\mu_k\wedge \neg A_k\verifies\predabsphi$
\noindent
Therefore, having algorithms able to stop extending $\mu_j$ as soon as 
$\mu_j\entails\predabsphi$,  even when 
$\mu_j\not\verifies\predabsphi$,  would produce much more compact
 formulas. 


==> arxiv-version/partialsat.tex <==

We address the following basic question:
{\em What should we mean by ``a {partial} assignment $\mu$ satisfies $\vi$"?}
%\RSTODO{Riscrivere questo primo paragrafo.}
We wish to provide a satisfactory definition of partial-assignment
satisfiability for a generic propositional formula ---i.e., non
only for (tautology-free) CNF. 
%
Ideally, a suitable definition of partial-assignment satisfiability
should verify all statements in property~\ref{prop:total-properties},
in particular (ii) and (iv). 
%
In practice, unfortunately, at least for generic (non-CNF) formulas, we show
 this is not the case. 

\subsection{\Verbverification{} and entailment of plain formulas.}
\label{sec:partialsat-plain}

\paragraph{Definitions.}
The first candidate definition of partial-assignment satisfaction,
which extends to partial assignments 
property~\ref{prop:total-properties}(iii),
is %to see it as
{\em \verbverification}. 
%
\begin{definition}
%  \marg{def of $\verifies$}
\label{def:verification}
We say that a {\em partial} truth assignment $\mu$  {\bf \verbverifies{}} $\varphi$ 
iff $\muof{\vi}=\tval$ (or, equivalently by
property~\ref{prop:eval-simplifies}, iff $\applymuvi=\top$).
%
We denote this fact with ``$\mu\verifies\varphi$''.
\end{definition}

\noindent
We stress the fact that \verbverification{} is a {\em semantic}
definition. Nevertheless,
due to property~\ref{prop:eval-simplifies}, it 
has also an easy-to-check
syntactic definition: $\mu\verifies\vi$ iff $\applymuvi=\top$. 
%


The second candidate definition of partial-assignment satisfaction, which extends to partial assignments 
property~\ref{prop:total-properties}(i),
is {\em entailment}. 

\begin{definition}
\label{def:entailment}
  We say that a {\em partial} truth assignment $\mu$  {\bf entails} $\varphi$
if and only if, for every total truth assignments $\eta$
s.t.$\mu\subseteq\eta$, 
$\eta$ satisfies $\varphi$ (or equivalently, iff $\applymuvi$ is
valid). 
%
We denote this fact with ``$\mu\entails\varphi$''.
\end{definition}

%\noindent
%\noindent
% In substance,
% Definition~\ref{def:verification} extends to partial assignments 
% property~\ref{prop:total-properties}(iii),
% whereas 
% Definition~\ref{def:entailment} extends to partial
% assignments property~\ref{prop:total-properties}(i).
%
% We stress the fact that both \verbverification{} and entailment are {\em semantic}
% definitions, although,
% due to property~\ref{prop:eval-simplifies}, \verbverification{}
% has also an easy-to-check
% syntactic characterization: $\mu\verifies\vi$ iff $\applymuvi=\top$. 
% by property~\ref{prop:eval-simplifies}, $\mu$ \verbverifies{} $\varphi$ 
% if and only if the result of applying $\mu$ to $\varphi$ is $\top$.

\paragraph{\Verbverification{} vs. Entailment.}
%\marg{$\verifies$ stronger than $\entails$}
We show the following facts. 
When the formula $\vi$ is a tautology-free CNF
% (and does not contain
% valid clauses, which however are easy to eliminate by preprocessing)
then
%Definitions~\ref{def:verification} and \ref{def:entailment}
\verbverification{} and entailment
coincide: 
$\mu\verifies\varphi$ iff $\mu\entails\varphi$.
%\footnote{ 
\ignore{%% moved to explicit proofs.
  In fact, if $\mu\verifies\vi$ then,  for every $\eta$ s.t.
$\eta\supseteq\mu$, $\eta\verifies\vi$ and thus $\eta\models\vi$, hence
$\mu\entails\vi$;
also, if $\mu\entails\vi$ then $\applymuvi$ is a valid
  CNF formula which does not contain valid clauses, so that $\applymuvi$
  must be $\top$, hence $\mu\verifies\vi$.
}
\ignore{%
(We conjecture that this is the reason why the distinction between
these two concepts 
% \verbverification{} and entailment
has been long overlooked in the literature.)}
%}
% We guess this equivalence is the reason why these two concepts are rarely
% distinguished in the literature.
%
Unfortunately, \emph{with generic %(non-CNF)
formulas 
\verbverification{} and entailment
%  Definitions~\ref{def:verification} and  \ref{def:entailment}
  do not coincide, the former being
strictly stronger than the latter}. 
%\noindent
%In fact, as above, if $\mu\verifies\vi$ then obviously
% ,  for every $\eta$ s.t.
% $\eta\supseteq\mu$, $\eta\verifies\vi$ and thus $\eta\models\vi$, hence
%$\mu\entails\vi$, whereas {\em the converse is not true}:
%
% E.g.,
% if $\vi\defas(A_1\wedge A_2)\vee (A_1\wedge \neg A_2)$ and 
% $\mu\defas\set{A_1}$, 
% then 
% $\mu\entails\vi$ but $\mu\not\verifies\vi$.
% %
These facts are illustrated in the following result.

\begin{theorem}
\label{prop:stronger}
\label{prop:equivalentifcnf}
Let \vi be a formula and $\mu$ be a partial truth
assignment over its atoms.
\begin{itemize}
\item[(a)] If \vi{} a tautology-free CNF, then
$\mu\entails\vi$ iff $\mu\verifies\vi$.
\item[(b)] If \vi{} is a generic formula, then
$\mu\entails\vi$ if $\mu\verifies\vi$, but the converse does not hold.
\end{itemize}


% : 
% $\mu\verifies\vi \thus \mu\entails\vi$ but 
% $\mu\entails\vi \not\thus \mu\verifies\vi$.
\end{theorem}
\begin{proof}
$(a)$: Let $\vi$ be a tautology-free CNF. 
If $\mu\entails\vi$, then $\applymuvi$ is a valid
  CNF formula which does not contain valid clauses, so that
  $\applymuvi=\top$, hence $\mu\verifies\vi$  by
  property~\ref{prop:eval-simplifies}.\\
$(a)$ and $(b)$:
If $\mu\verifies\vi$ then,  for every $\eta$ s.t.
$\eta\supseteq\mu$, $\eta\verifies\vi$ and thus $\eta\models\vi$, hence
$\mu\entails\vi$.\\
$(b)$: The fact that the converse does not hold is shown in \cref{ex:stronger}.
\hfill $\qed$
% \ \\
%   If $\mu\verifies\vi$ then,  for every $\eta$ s.t.
% $\eta\supseteq\mu$, $\eta\verifies\vi$ and thus $\eta\models\vi$, hence
% $\mu\entails\vi$.\\
% If $\vi$ is a tautology-free CNF and
% if $\mu\entails\vi$, then $\applymuvi$ is a valid
%   CNF formula which does not contain valid clauses, so that
%   $\applymuvi=\top$, hence $\mu\verifies\vi$  by
%   property~\ref{prop:eval-simplifies}.\\
% % Let $\vi\defas(A_1\wedge A_2)\vee (A_1\wedge \neg A_2)$ and 
% % $\mu\defas\set{A_1}$.
% % Then 
% % $\mu\entails\vi$ but $\mu\not\verifies\vi$.
% The fact that the converse does not hold is shown in \cref{ex:stronger}.
% \hfill $\diamond$
\end{proof}
%\ignore{%
  \begin{example}
  \label{ex:stronger}
%  \RSTODO{move inside above proof?}
Let $\vi\defas(A_1\wedge A_2)\vee (A_1\wedge \neg A_2)$ and 
$\mu\defas\set{A_1}$.
Then 
$\mu\entails\vi$ but $\mu\not\verifies\vi$.
%  
\end{example}
%}
\noindent
Hereafter we implicitly assume w.l.o.g. that all CNF formulas are tautology free.

%\marg{properties of $\verifies$ and $\entails$}
We try to build a counterpart of property~\ref{prop:total-properties}
for Definitions~\ref{def:verification} and
\ref{def:entailment} respectively, but in both cases we fail to
achieve all points (i)-(iv), % in property~\ref{prop:total-properties},
resulting into complementary situations.
%
%\subsubsection{Pros and cons of partial-assignment satisfiability as verification.}
%%% Validation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \ignore{From Definition~\ref{def:verification}
% we easily derive the following facts. }
The following properties follow straightforward from Definitions~\ref{def:verification} and  \ref{def:entailment}.
(Here ``\oksym{}'' \resp{``\noksym{}''} denotes facts from
property~\ref{prop:total-properties} which are \resp{are not} preserved.)

\begin{property}
\label{prop:partial-verification}
Let $\mu$ be a partial truth assignment on \alla{} and
$\vi,\vione,\vitwo$ be formulas on \alla. 
\begin{renumerate}
\item \noksym{}
If $\mu\verifies\varphi$ then $\andmu\entails\varphi$, {but not vice versa}.
\item \noksym{}
If $\vione$ and $\vitwo$ are  equivalent, this {does not} imply
that $\mu\verifies\vione$ iff $\mu\verifies\vitwo$.
\item \oksym{}
  $\mu\verifies\varphi$ iff \applymuvi{} is $\top$
     (also, iff $\muof{\vi}= \tval$ by property~\ref{prop:eval-simplifies}). 

\item \oksym{}
Checking
$\mu\verifies\vi$  requires at most a polynomial amount of steps.
\end{renumerate}  
\end{property}

%\subsubsection{Pros and cons of partial-assignment satisfiability as entailment.}
%%% Entailment
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ignore{From Definition~\ref{def:entailment}
we easily derive the following.}

\begin{property}
\label{prop:partial-entailment}
Let $\mu$ be a partial truth assignment on \alla{} and
$\vi,\vione,\vitwo$ be formulas on \alla. 
\begin{renumerate}
\item \oksym{}
$\mu\entails\varphi$ iff $\andmu\entails\varphi$.
\item \oksym{}
If $\vione$ and $\vitwo$ are  equivalent, then 
$\mu\entails\vione$ iff $\mu\entails\vitwo$.
\item \noksym{}
  $\mu\entails\varphi$ iff \applymuvi{} is a valid formula, not
  necessarily $\top$
   (also, in general $\muof{\vi} \neq \tval$). 
\item \noksym{}
Checking
$\mu\entails\vi$ is \emph{co-NP-complete}.
\ignore{%trivial
  \footnote{In fact, checking the validity of \vi{}
translates into verifying that the empty assignment
entails it.}}
\end{renumerate}  
\end{property}

\begin{example}
  \label{ex:embarassing}
  Let $\vi_1\defas(A_1\wedge A_2)\vee (A_1\wedge \neg A_2)$,
  $\vi_2\defas A_1$ and 
$\mu\defas\set{A_1}$.
Then
$\vi_1\equiv\vi_2$, $\apply{\vi_1}{\mu} = A_2\vee\neg A_2\neq \top$ and $\apply{\vi_2}{\mu}=\top$.
Thus
$\mu\entails\vi_1$ and $\mu\entails\vi_2$, whereas
$\mu\not\verifies\vi_1$ but $\mu\verifies\vi_2$.
\hfill $\diamond$
\end{example}


%\marg{Embarassing $\verifies$}
From a theoretical viewpoint, \cref{ex:embarassing} spotlights the difference between
property~\ref{prop:partial-verification}(ii) and
property~\ref{prop:partial-entailment}(ii) (see also  Property~\ref{prop:total-properties}(ii)):
%
\emph{whereas entailment  matches the intuition 
%and theoretical requirement
that equivalent %although syntactically different
formulas should be satisfied by the same (partial) assignments,
\verbverification{} does not}. 
% One main advantage of adopting entailment
% %as a definition of
% %Definition~\ref{def:entailment} as
% instead is that it matches the intuition 
% and theoretical requirement
% that equivalent formulas should be satisfied by the same assignments,
% even partial ones (Property~\ref{prop:partial-entailment}(ii)), whereas 
% %
% one main drawback of \verbverification{} is that 
% that equivalent although syntactically different 
% formulas may be \verbverified{} by different sets of partial
% assignments  (Property~\ref{prop:partial-verification}(ii)), 
The latter fact looks theoretically awkward. 
%even partial (Property~\ref{prop:partial-entailment}(ii)). 
%
% In particular, we believe this would be an embarrassing fact
% if we adopted \verbverification{} as the general definition of  partial-assignment
% satisfiability.
% In particular we believe that, 
% if we adopted \verbverification{} as the general definition of  partial-assignment
% satisfiability,
% then it would be embarrassing  to have that equivalent formulas were not ``satisfied''
% by the same assignments.
%
In particular, 
if we adopted \verbverification{} as the general definition of  partial-assignment
satisfiability,
then  we believe that it would be embarrassing to have that equivalent formulas were not ``satisfied''
by the same assignments.


%\TODO{We believe this is quite embarassing...}

% On the one hand, 
% the advantage of adopting entailment
% %as a definition of
% %Definition~\ref{def:entailment} as
% for checking
% partial-assignment satisfiability is that it matches the intuition 
% and theoretical requirement
% that equivalent formulas should be satisfied by the same assignments,
% even partial ones (Property~\ref{prop:partial-entailment}(ii)). 
% %
% On the other hand, the price to pay is that the resulting problem 
% is co-NP-complete  (Property~\ref{prop:partial-entailment}(iv)),
% because it is equivalent to checking the validity of the residual \applymuvi.


%\NOTE{Spiegare. }
%\begin{IGNOREINSHORT}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Other possible partial-satisfaction relations.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newpage
\subsection{Other candidate forms of partial-assignment satisfaction.}
\label{sec:partialsat-others}
%\marg{other  candidate forms of satisfiability}
Given the above facts, we wonder if we could use other notions
of partial-assignment satisfiability. (E.g., we could enrich
$\verifies$ with some form of formula simplification.)
In particular, we wonder if there exists some suitable notion of
partial-assignment satisfaction which is strictly stronger then 
entailment and fixes the ``embarrassing fact'' for \verbverification{} of
Property~\ref{prop:partial-verification}(ii).
The following theorem states this is not the case.
%
\ignore{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{theorem}
  \RSTODO{rivedere la parte ``generical relation. Aggiungere ``if
    $\mu\genericentails\vi$, then $\mu\cup\mu'\genericentails\vi$''
    per dire che comunque non puo' essere piu' debile di
    $\entails$. oppure dire esplicitamente che non e' piu' debole di $\entails$.}
  \RSTODO{riscrivere come: ``if (a), (b) and $\genericentails$ matches
    equivalence, then $\mu\genericentails\vi$ iff $\mu\entails\vi$??
    similar proof by absurd}
\label{uniqueness:teo}
Let $\genericentails$ denote some relation between a partial
truth assignment  and a Boolean formula such that $\mu\entails\vi$ if
$\mu\genericentails\vi$, and
% \RSTODO{sostituire (a) con ``if $\eta$ total for $\vi$, then
%   $\eta\genericentails\vi$ iff
%   $\eta\models\vi$? Da questo deriva anche (b)?}
\begin{aenumerate}
\item
   if $\eta$ is total for $\vi$, then
   $\eta\genericentails\vi$ iff
   $\eta\models\vi$;
\item for every $\mu$, $\vi_1$ and $\vi_2$, if $\mu\genericentails\vi_1\wedge\vi_2$, then $\mu\genericentails\vi_1$ and
  $\mu\genericentails\vi_2$;
\item there exist $\mu$ and $\vi$ s.t. $\mu\entails\vi$ and $\mu\not\genericentails\vi$ .
%\item  if $\mu\genericentails\vi$ then $\mu\entails\vi$;
\end{aenumerate}
Then there exist $\mu'$, $\vi_1$ and $\vi_2$ s.t. $\vi_1\equiv\vi_2$, 
$\mu'\genericentails\vi_1$ and $\mu'\not\genericentails\vi_2$.
\end{theorem}
\begin{proof}
%% PROOF VERIFICATA
  Consider $\mu$ and $\vi$ as in point {\em (c)}.
  Let $\mu'\defas\mu$,
  $\vi_1\defas\andmu$ and $\vi_2\defas\andmu\wedge\varphi$.
  Then $\vi_1\equiv\vi_2$ because $\mu\entails\vi$ and because of
  Property~\ref{prop:partial-entailment}(i); also, $\mu'\genericentails\vi_1$
  by point {\em (a)} and $\mu'\not\genericentails\vi_2$ by point {\em
    (b)}.
  \hfill $\qed$
\end{proof}
}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% RISCRITTA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{theorem}
  \label{uniqueness:teo}
  Let $\genericentails$ denote some relation
  such that
%   for every $\mu$ and $\vi$,  $\mu\entails\vi$ if
% $\mu\genericentails\vi$,
% and
\begin{aenumerate}
\item for every $\mu$ and $\vi$,  $\mu\entails\vi$ if
$\mu\genericentails\vi$;
\item{\label{item:total}}
   for every $\eta$ and $\vi$,
%   \RSTODO{ma (b) non deriva da (a)??}
   if $\eta$ is total for the set of atoms in $\vi$, then
   $\eta\genericentails\vi$ iff
   $\eta\models\vi$;
 \item{\label{item:and}} for every $\mu$, $\vi_1$ and $\vi_2$,
   if $\mu\genericentails\vi_1\wedge\vi_2$, then $\mu\genericentails\vi_1$ and
  $\mu\genericentails\vi_2$;
\item for every $\mu$, $\vi_1$ and $\vi_2$,
  if $\vi_1\equiv\vi_2$, then $\mu\genericentails\vi_1$ iff
  $\mu\genericentails\vi_2$
\end{aenumerate}
Then, for every $\mu$, $\vi$, we have that $\mu\genericentails\vi$ if and only if $\mu\entails\vi$.
\end{theorem}
%\cref{item:total}
\begin{proof}
  The ``only if'' part  is hypothesis {\em (a)}.\\
  The ``if'' part: By absurd, suppose there exist $\mu$ and $\vi$ s.t. $\mu\entails\vi$ and $\mu\not\genericentails\vi$ .
  \\Let %$\mu'\defas\mu$,
  $\vi_1\defas\andmu$ and $\vi_2\defas\andmu\wedge\varphi$.
  Then we have that:
  \\$\vi_1\equiv\vi_2$, because $\mu\entails\vi$, and hence $\andmu\entails\vi$ because of
  Property~\ref{prop:partial-entailment}(i);
  \\$\mu\genericentails\vi_1$,
  because of hypothesis {\em (b)};
  \\$\mu\not\genericentails\vi_2$, because of hypothesis {\em
    (c)}.
  \\ The latter three facts violate hypothesis {\em (d)}.
  \hfill $\qed$
\end{proof}



Theorem \ref{uniqueness:teo} says that entailment is
the only relation
which
$(a)$ is stronger or equal than entailment,
$(b)$ extends to partial assignments the standard notion of
total-assignment satisfaction,
$(c)$ maintains the standard semantics of
$\wedge$, and
$(d)$ verifies
Property~\ref{prop:partial-entailment}(ii).
Thus, any such relation $\genericentails$ which is strictly stronger
that $\entails$ suffers for
the same ``embarrassing fact'' of
Property~\ref{prop:partial-verification}(ii).


%
  \begin{example}
    % Let ``$\genericentails$'' denote a variant of $\verifies$ such
    % that $\mu\genericentails\vi$ 
    % implements a syntactic check which applies also the reduction
    % ``$l\vee \neg l \Rightarrow \top$'', $l$ being literals, while computing the residual
    % \applymuvi{}.
%
    Let ``$\genericentails$'' denote a variant of $\verifies$ such
    that $\mu\genericentails\vi$ 
    implements a syntactic check which adds %the reduction
    ``$l\vee \neg l \Rightarrow \top$'', $l$ being a literal, to the
    rules used in \cref{fig:boolprop} for computing the residual
    \applymuvi{}.
%
    Thus, considering the formula $\vi_1$ of \cref{ex:embarassing} we
    have $\mu\genericentails\vi_1$. 

    Nevertheless,    let
$\mu\defas\set{A_1,..,A_M}$ s.t.
$\vi\defas\bigvee_{i=1}^M (A_i\wedge cube_i)$ s.t. each $cube_i$ is a
non-unary cube and $\bigvee_{i=1}^M cube_i$ is
valid and does not contain occurrences of the atoms $A_1,..,A_M$. Then 
$\mu\entails\vi$ but $\mu\not\genericentails\vi$, because
\applymuvi{} is the valid formula $\bigvee_i
cube_i$ which is not simplified by the above reduction.
If $\vi_2\defas\bigwedge\mu$, then $\vi\equiv \vi_2$,
$\mu\not\genericentails\vi$ but $\mu\genericentails\vi_2$,
whereas $\mu\entails\vi$ and $\mu\entails\vi_2$. Thus the ``embarrassing
fact'' above applies also to $\genericentails$. 
\hfill $\diamond$
%}  
\end{example}  

\ignore{
\begin{IGNOREINSHORT}
  \begin{example}
%    \RSTODO{Usare da qualche? Utile?}
%    ~\footnote{%
Let
$\mu\defas\set{A_1,..,A_M}$ s.t. $M<N$ and
$\vi\defas\bigvee_i (A_i\wedge cube_i)$ s.t. each $cube_i$ is a cube and $\bigvee_i cube_i$ is
valid and does not contain occurrences of the atoms $A_1,..,A_M$. Then 
$\mu\entails\vi$ but \applymuvi{} is the valid formula $\bigvee_i
cube_i$, so that $\mu\not\verifies\vi$. \hfill $\diamond$
%}  
\end{example}  
\end{IGNOREINSHORT}
}



==> arxiv-version/partialsat.tex.1 <==
%\input{fig_threevalues}
% 
{What do we mean by ``a \emph{partial} assignment $\mu$ satisfies $\vi$"?}
We wish to provide a satisfactory definition of partial-assignment
satisfiability for a generic propositional formula ---i.e., non
necessarily (tautology-free) CNF. 
%

\paragraph{\Verbvalidation{} vs. Entailment.}
Ideally, a suitable definition of partial-assignment satisfiability
should verify all statements in Property~\ref{prop:total-properties},
in particular (ii) and (iv). 
%
In practice, unfortunately, at least for generic (non-CNF) formulas, we see
 this is not the case. 

 One first possibility is to see partial-assignment satisfiability as
{\em \verbvalidation}. 
%
\begin{definition}
\label{def:validation}
We say that a {\em partial} truth assignment $\mu$  {\bf \verbvalidates{}} $\varphi$ 
iff $\muof{\vi}=\tval$ (or, equivalently by
Property~\ref{prop:eval-simplifies}, iff $\apply{\mu}{\vi}=\top$).
%
We denote this fact with ``$\mu\validates\varphi$''.
\end{definition}
%
One second possibility is to see partial-assignment satisfiability as
{\em entailment}. 

\begin{definition}
\label{def:entailment}
  We say that a {\em partial} truth assignment $\mu$  {\bf entails} $\varphi$
if and only if, for every total truth assignments $\eta$
s.t.$\mu\subseteq\eta$, 
$\eta$ satisfies $\varphi$. 
%
We denote this fact with ``$\mu\entails\varphi$''.
\end{definition}

\noindent
%\noindent
In substance,
Definition~\ref{def:validation} extends to partial assignments 
Property~\ref{prop:total-properties}(iii),
whereas 
Definition~\ref{def:entailment} extends to partial
assignments Property~\ref{prop:total-properties}(i).
%
Notice that both \verbvalidation{} and entailment are {\em semantic}
definitions.
Due to Property~\ref{prop:eval-simplifies}, \verbvalidation{}
has also an easy-to-check
syntactic characterization as ``$\apply{\mu}{\vi}=\top$''. 
% by Property~\ref{prop:eval-simplifies}, $\mu$ \verbvalidates{} $\varphi$ 
% if and only if the result of applying $\mu$ to $\varphi$ is $\top$.



When the formula $\vi$ is in CNF and does not contain
valid clauses --which however are easy to eliminate by preprocessing-- 
then Definitions~\ref{def:validation} and
\ref{def:entailment}  are equivalent: 
$\mu\validates\varphi$ iff $\mu\entails\varphi$.
%\footnote{ 
In fact, if $\mu\validates\vi$ then,  for every $\eta$ s.t.
$\eta\supseteq\mu$, $\eta\validates\vi$ and thus $\eta\models\vi$, hence
$\mu\entails\vi$;
also, if $\mu\entails\vi$ then $\applymuvi$ is a valid
  CNF formula which does not contain valid clauses, so that $\applymuvi$
  must be $\top$, hence $\mu\validates\vi$.
%}
% We guess this equivalence is the reason why these two concepts are rarely
% distinguished in the literature.


Unfortunately, when dealing with generic (non-CNF) formulas, 
we notice that \emph{Definitions~\ref{def:validation} and
\ref{def:entailment}  are not equivalent, the former being
strictly stronger than the latter}. 
%\noindent
In fact, as above, if $\mu\validates\vi$ then obviously
% ,  for every $\eta$ s.t.
% $\eta\supseteq\mu$, $\eta\validates\vi$ and thus $\eta\models\vi$, hence
$\mu\entails\vi$, whereas {\em the converse is not true}: e.g.,
if $\vi\defas(A_1\wedge A_2)\vee (A_1\wedge \neg A_2)$ and 
$\mu\defas\set{A_1}$, 
then 
$\mu\entails\vi$ but $\mu\not\validates\vi$.
%
This leads to the following statement.

\begin{proposition}
\label{prop:stronger}
If a partial truth assignment $\mu$ {\verbvalidates{}}
$\varphi$, then it also {entails} $\varphi$, but the converse does
not hold.
% : 
% $\mu\validates\vi \thus \mu\entails\vi$ but 
% $\mu\entails\vi \not\thus \mu\validates\vi$.
\end{proposition}
%
\begin{IGNOREINSHORT}
\begin{example}
%~\footnote{%
Let
$\mu\defas\set{A_1,..,A_M}$ s.t. $M<N$ and
$\vi\defas\bigvee_i (A_i\wedge cube_i)$ s.t. each $cube_i$ is a cube and $\bigvee_i cube_i$ is
valid and does not contain occurrences of the atoms $A_1,..,A_M$. Then 
$\mu\entails\vi$ but \applymuvi{} is the valid formula $\bigvee_i
cube_i$, so that $\mu\not\validates\vi$. \hfill $\diamond$
%}  
\end{example}  
\end{IGNOREINSHORT}


We try to build a counterpart of Property~\ref{prop:total-properties}
for Definitions~\ref{def:validation} and
\ref{def:entailment} respectively, but in both cases we fail to
achieve all points (i)-(iv) in Property~\ref{prop:total-properties},
resulting into complementary situations.
%

%\subsubsection{Pros and cons of partial-assignment satisfiability as validation.}
%%% Validation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
From Definition~\ref{def:validation}
we easily derive the following facts. 
(Here ``\oksym{}'' \resp{``\noksym{}''} denotes facts from
Property~\ref{prop:total-properties} which are \resp{are not} preserved.)

\begin{property}
\label{prop:partial-validation}
Let $\mu$ be a partial truth assignment on \alla{} and
$\vi,\vione,\vitwo$ be formulas on \alla. 
\begin{renumerate}
\item \noksym{}
If $\mu\validates\varphi$ then $\andmu\entails\varphi$, {but not vice versa}.
\item \noksym{}
If $\vione$ and $\vitwo$ are  equivalent, this {does not} imply
that $\mu\validates\vione$ iff $\mu\validates\vitwo$.
\item \oksym{}
  $\mu\validates\varphi$ iff \applymuvi{} is $\top$
     (also, iff $\muof{\vi}= \tval$ by Property~\ref{prop:eval-simplifies}). 

\item \oksym{}
Checking
$\mu\validates\vi$  requires at most a polynomial amount of steps.
\end{renumerate}  
\end{property}

%\subsubsection{Pros and cons of partial-assignment satisfiability as entailment.}
%%% Entailment
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
From Definition~\ref{def:entailment}
we easily derive the following. 

\begin{property}
\label{prop:partial-entailment}
Let $\mu$ be a partial truth assignment on \alla{} and
$\vi,\vione,\vitwo$ be formulas on \alla. 
\begin{renumerate}
\item \oksym{}
$\mu\models\varphi$ iff $\andmu\entails\varphi$.
\item \oksym{}
If $\vione$ and $\vitwo$ are  equivalent, then 
$\mu\models\vione$ iff $\mu\models\vitwo$.
\item \noksym{}
  $\mu\models\varphi$ iff \applymuvi{} is a valid formula, not
  necessarily $\top$
   (also, in general $\muof{\vi} \neq \tval$). 
\item \noksym{}
Checking
$\mu\entails\vi$ is \emph{co-NP-complete}.
\footnote{In fact, checking the validity of \vi{}
translates into verifying that the empty assignment
entails it.}
\end{renumerate}  
\end{property}
\noindent

For instance we notice that, when applied to satisfiable formulas,
%
OBDDs \cite{bryant2} produce branches representing
partial assignments which {\em entail} the input formula
(Definition~\ref{def:entailment}), because if $\mu\entails\vi$ then
\applymuvi is
valid (Property~\ref{prop:partial-entailment}(iii)), so that its corresponding 
sub-OBDD is reduced into the $\top$ node.
%
Instead SAT/AllSAT algorithms like \new{Analytic Tableaux} 
\footnote{Notice that Analytic Tableaux may generate duplicated
 or subsumed  assignments (see \cite{dagostino1,gs-infocomp2000})}
\cite{smullyan1} 
or ``classic'' \new{DPLL}~%
\footnote{Classic DPLL procedure \cite{davis7} was
  designed to work for CNF  
  formulas. Nevertheless it is easy to produce non-CNF a version of this
procedure (see e.g. \cite{armando5}).} 
%
\cite{davis7} produce branches representing
partial assignments which {\em \verbvalidate} the input formula
(Definition~\ref{def:validation}) because, unlike with OBDDs,
as soon as it is produced (a branch corresponding to) an assignment
$\mu$ s.t. 
$\mu\entails\vi$ but $\mu\not\validates\vi$, they do not realize it and
proceed the search until they extend it to some $\mu'\supset\mu$ s.t. 
$\mu'\validates\vi$, extending the search tree of up to
$2^{||\mu'||-||\mu||}$ branches.  
%
%\RSTODO{espandi un po' e spiaga perche'. example?}

%\input{figure.tex}
\input{figure_long.tex}
%
\begin{example}
%  \RSTODO{estendere a formula con 2 congiunti simili. Aggiungere XDDs? }
Consider $\vi\defas\mainwff$. 
  Figure~\ref{fig:comparison} 
represents the OBDD for $\vi$ and 
the search trees corresponding to 
All-SAT executions of Analytic
Tableaux and 
(non-CNF) DPLL on $\vi$. 
\begin{IGNOREINSHORT}
\footnote{Here in DPLL the pure-literal rule \cite{davis7} is not used because 
 in All-SAT it may hinder the enumeration of
 some relevant models (see, e.g., \cite{sebastiani_frocos07}).}  
\end{IGNOREINSHORT}
The former produces the single assignment
\singlemu{}. Notice that $\singlemu\entails\vi$ but $\singlemu\not
\validates\vi$.  The latter two produce the assignments \allmus{}.

Notice that neither Analytic Tableaux nor DPLL can produce \singlemu{} alone.
\hfill $\diamond$
\end{example}

\TODO{Riscrivi prossimo paragrafo}
\marg{\Verbvalidation{} vs. Entailment.}
The advantage of adopting \verbvalidation{} for checking
% as a definition of
partial-assignment satisfiability is that it matches the intuition
and practical need that the process of checking it should be fast (Property~\ref{prop:partial-validation}(iv)).  
%
The main drawback is that 
that equivalent although syntactically different 
formulas may be satisfied by different sets of partial
assignments  (Property~\ref{prop:partial-validation}(ii)), 
which looks theoretically awkward. 
%even partial (Property~\ref{prop:partial-entailment}(ii)). 
\ignoreinshort{%
We believe this would be an embarrassing fact
if we adopted \verbvalidation{} as the definition of  partial-assignment
satisfiability for non-CNF formulas.
}

%\TODO{We believe this is quite embarassing...}

On the one hand, 
the advantage of adopting entailment
%as a definition of
%Definition~\ref{def:entailment} as
for checking
partial-assignment satisfiability is that it matches the intuition 
and theoretical requirement
that equivalent formulas should be satisfied by the same assignments,
even partial ones (Property~\ref{prop:partial-entailment}(ii)). 
%
On the other hand, the price to pay is that the resulting problem 
is co-NP-complete  (Property~\ref{prop:partial-entailment}(iv)),
because it is equivalent to checking the validity of the residual \applymuvi.


\smallskip
Due to Proposition~\ref{prop:stronger}, every
 partial assignments entailing the input formula is  a \emph{subset}
 of some other(s) \verbvalidating{} it.
Therefore, for an assignment-enumeration algorithm,
 being able to enumerate partial 
assignments entailing the input formula rather than simply \verbvalidating{}
it  may (even drastically) reduce the number of the satisfying assignment
enumerated. 
%



%\NOTE{Spiegare. }
\begin{IGNOREINSHORT}  
\paragraph{Other possible partial-satisfaction relations.}
Given the above facts, we wonder if we could use other notions
of partial-assignment satisfiability (e.g., we could enrich
$\validates$ with some form of formula simplification).
In particular, we wonder if there exists some suitable notion of
partial-assignment satisfaction which is strictly stronger than
entailment and fixes the ``embarassing issue'' of
Property~\ref{prop:partial-validation}(ii).
The following theorem states this is not the case.
\begin{theorem}
\label{uniqueness:teo}
Let $\genericentails$ denote some generical relation between a (possibly partial)
truth assignment  and a Boolean formula, such that
% \RSTODO{sostituire (a) con ``if $\eta$ total for $\vi$, then
%   $\eta\genericentails\vi$ iff
%   $\eta\models\vi$? Da questo deriva anche (b)?}
\begin{aenumerate}
\item  if $\eta$ is total for $\vi$, then
  $\eta\genericentails\vi$ iff
  $\eta\models\vi$;
\item for every $\mu$, $\vi_1$ and $\vi_2$, if $\mu\genericentails\vi_1\wedge\vi_2$, then $\mu\genericentails\vi_1$ and
  $\mu\genericentails\vi_2$;
\item there exist $\mu$ and $\vi$ s.t. $\mu\entails\vi$ and $\mu\not\genericentails\vi$ .
\end{aenumerate}
Then there exist $\mu'$, $\psi_1$ and $\psi_2$ s.t. $\psi_1\equiv\psi_2$, 
$\mu'\genericentails\psi_1$ and $\mu'\not\genericentails\psi_2$.
\end{theorem}
\begin{proof}
%% PROOF VERIFICATA
  Consider $\mu$ and $\vi$ as in point {\em (c)}.
  Let $\mu'\defas\mu$,
  $\psi_1\defas\andmu$ and $\psi_2\defas\andmu\wedge\varphi$.
  Then $\psi_1\equiv\psi_2$ because $\mu\entails\vi$ and because of
  Property~\ref{prop:partial-entailment}(i); also, $\mu'\genericentails\psi_1$
  by point {\em (a)} and $\mu'\not\genericentails\psi_2$ by point {\em
    (b)}.
  \hfill $\diamond$
\end{proof}
Theorem \ref{uniqueness:teo} says that entailment is
the only relation
which extends to partial assignments the standard notion of
total-assignment satisfaction
(point $(a)$), maintains the standard semantics of
$\wedge$ (point $(b)$) and verifies
Property~\ref{prop:partial-entailment}(ii).
Any relation $\genericentails$ which is strictly stronger than $\models$ suffers for
the same ``embarassing issue'' of
Property~\ref{prop:partial-validation}(ii) (point $(c)$).
% Theorem \ref{uniqueness:teo} says that if a relation $\genericentails$
% extends to partial assignments the standard notion of satisfaction
% (point $(a)$), maintains the standard semantics of
% $\wedge$ (point $(b)$) and
% is strictly stronger than entailment (point $(c)$), than it does not verify
% Property~\ref{prop:partial-entailment}(ii), that is, it suffers for
% the same ``embarassing issue'' of
% Property~\ref{prop:partial-validation}(ii).
\end{IGNOREINSHORT}

\paragraph{Dealing with CNF-ized formulas.}
One may argue that in SAT/AllSAT the distinction between $\validates$ and
$\entails$ is not much relevant in practice, because we can
CNF-ize upfront the input formulas ---typically by
variants of Tseitin CNF-ization--- removing tautological clauses, and this
distinction does not hold for (tautology-free) CNF
formulas.
%
However, we notice that with Tseitin CNF-ization we may loose
information regarding entailment or \verbvalidation{}. In fact, if
$\psi$ on $\alla\cup\allb$ is the result of Tseitin CNF-izing $\vi$,
then:
\begin{itemize}
% \item 
% If $\mu\cup\gamma\validates\phi$ for some total truth assignment
%   $\gamma$, then $\mu\validates\vi$.
% \item 
% If $\mu\cup\gamma\entails\phi$ for some total truth assignment
%   $\gamma$, then $\mu\entails\vi$.
\item 
$\mu\validates\vi$ \emph{does not imply} that there exists a total assignment
  $\delta$ on \allb s.t. $\mu\cup\delta\validates\psi$;
\item 
$\mu\entails\vi$ \emph{does not imply} that there exists a total assignment
  $\delta$ on \allb s.t. $\mu\cup\delta\entails\psi$.
\end{itemize}

\begin{example}
Consider $\vi\defas A_1 \vee (A_2\wedge A_3)$ 
and its Tseitin CNF-ized version:\\
$
\begin{array}{lll}
\psi\defas & (A_1\vee  B_1)\ \wedge \\
& (\neg B_1 \vee  A_2) \wedge
(\neg B_1 \vee  A_3) \wedge 
(B_1\vee \neg A_2 \vee \neg A_3) & \ \ \ //\ B_1 \iff (A_2\wedge A_3). \\
\end{array}
$\\
On the one hand, $\mu\defas \set{A_1}$ is such that $\mu\validates\vi$. 
On the other hand, there is no total truth assignment $\delta$ on
\set{B_1} s.t. $\mu\cup\delta\validates\psi$. In fact, neither 
$\set{A_1,B_1}\validates\psi$ nor $\set{A_1,\neg B_1}\validates\psi$.

Consider $\vi\defas
(A_1\wedge \pos A_2)\vee (A_1\wedge\neg A_2) 
$ 
and its Tseitin CNF-ized version:\\
$
\begin{array}{lll}
\psi\defas  
& (B_1\vee B_2)\ \wedge & \\
& (\neg B_1 \vee \pos A_1) \wedge
(\neg B_1 \vee \pos A_2) \wedge
(B_1\vee \neg A_1 \vee \neg A_2)\ \wedge\ & \ \ \ //\ B_1 \iff (A_1\wedge \pos A_2) \\
& (\neg B_2 \vee \pos A_1) \wedge
(\neg B_2 \vee \neg A_2) \wedge
(B_2\vee \neg A_1 \vee \pos A_2).\ & \ \ \ //\ B_2 \iff (A_1\wedge \neg A_2) 
\end{array}
%
% \psi\defas
% (B_1\vee B_2) \wedge
% (\neg B_1 \vee A_1) \wedge
% (\neg B_1 \vee A_2) \wedge
% (B_1\vee \neg A_1 \vee \neg A_2) \wedge
% (\neg B_2 \vee \neg A_1) \wedge
% (\neg B_2 \vee \neg A_2) \wedge
% (B_2\vee \neg A_1 \vee A_2)   
$\\
Although $\mu\defas \set{A_1}$ is such that $\mu\entails\vi$,
%On the other hand,
 there is no total truth assignment $\delta$ on
\set{B_1,B_2} s.t. $\mu\cup\delta\entails\psi$:
$\set{A_1,B_1,\neg B_2}\not\entails \psi$ since
$\set{A_1,\neg A_2,B_1,\neg B_2}\not\entails \psi$;
$\set{A_1,\neg B_1,B_2}\not\entails \psi$
since $\set{A_1,A_2,\neg B_1,B_2}\not\entails \psi$;
$\set{A_1,B_1,B_2}$ and $\set{A_1,\neg B_1,\neg B_2}$ are both inconsistent
with $\psi$.
\hfill $\diamond$
\end{example}

\ignore{%%%%%%%%%%
\begin{proposition}
 \RSTODO{PROVA e scrivi controesempi. Scrivi in background l'equivalente controparte per $\eta \models\vi$\\}
Let $\vi$ be a generic (non-CNF)
formula on \alla and let $\psi$ on $\alla\cup\allb$ be the result of
CNF-izing \vi by applying standard Tseitin CNF-ization 
\cite{tseitin1} and removing valid clauses from $\psi$ if any, \allb
being the set of fresh propositions introduced in the process. Then:
\begin{itemize}
\item 
If $\mu\cup\gamma\validates\psi$ for some total truth assignment
  $\gamma$, then $\mu\validates\vi$.
\item 
If $\mu\cup\gamma\entails\psi$ for some total truth assignment
  $\gamma$, then $\mu\entails\vi$.
\item 
$\mu\validates\vi$ \emph{does not imply} that there exists a total assignment
  $\delta$ on \allb s.t. $\mu\cup\delta\validates\vi$
\item 
$\mu\entails\vi$ \emph{does not imply} that there exists a total assignment
  $\delta$ on \allb s.t. $\mu\cup\delta\entails\vi$
\end{itemize}

%Then $\mu\validates\vi$, but
%$\mu\entails\vi$
\end{proposition}
}


==> arxiv-version/partialsat.tex.2 <==
%\input{fig_threevalues}
% 
{What do we mean by ``a \emph{partial} assignment $\mu$ satisfies $\vi$"?}
We wish to provide a satisfactory definition of partial-assignment
satisfiability for a generic propositional formula ---i.e., non
necessarily (tautology-free) CNF. 
%

\paragraph{\Verbvalidation{} vs. Entailment.}
Ideally, a suitable definition of partial-assignment satisfiability
should verify all statements in Property~\ref{prop:total-properties},
in particular (ii) and (iv). 
%
In practice, unfortunately, at least for generic (non-CNF) formulas, we see
 this is not the case. 

 One first possibility is to see partial-assignment satisfiability as
{\em \verbvalidation}. 
%
\begin{definition}
\label{def:validation}
We say that a {\em partial} truth assignment $\mu$  {\bf \verbvalidates{}} $\varphi$ 
iff $\muof{\vi}=\tval$ (or, equivalently by
Property~\ref{prop:eval-simplifies}, iff $\apply{\mu}{\vi}=\top$).
%
We denote this fact with ``$\mu\validates\varphi$''.
\end{definition}
%
One second possibility is to see partial-assignment satisfiability as
{\em entailment}. 

\begin{definition}
\label{def:entailment}
  We say that a {\em partial} truth assignment $\mu$  {\bf entails} $\varphi$
if and only if, for every total truth assignments $\eta$
s.t.$\mu\subseteq\eta$, 
$\eta$ satisfies $\varphi$. 
%
We denote this fact with ``$\mu\entails\varphi$''.
\end{definition}

\noindent
%\noindent
In substance,
Definition~\ref{def:validation} extends to partial assignments 
Property~\ref{prop:total-properties}(iii),
whereas 
Definition~\ref{def:entailment} extends to partial
assignments Property~\ref{prop:total-properties}(i).
%
Notice that both \verbvalidation{} and entailment are {\em semantic}
definitions.
Due to Property~\ref{prop:eval-simplifies}, \verbvalidation{}
has also an easy-to-check
syntactic characterization as ``$\apply{\mu}{\vi}=\top$''. 
% by Property~\ref{prop:eval-simplifies}, $\mu$ \verbvalidates{} $\varphi$ 
% if and only if the result of applying $\mu$ to $\varphi$ is $\top$.



When the formula $\vi$ is in CNF and does not contain
valid clauses --which however are easy to eliminate by preprocessing-- 
then Definitions~\ref{def:validation} and
\ref{def:entailment}  are equivalent: 
$\mu\validates\varphi$ iff $\mu\entails\varphi$.
%\footnote{ 
In fact, if $\mu\validates\vi$ then,  for every $\eta$ s.t.
$\eta\supseteq\mu$, $\eta\validates\vi$ and thus $\eta\models\vi$, hence
$\mu\entails\vi$;
also, if $\mu\entails\vi$ then $\applymuvi$ is a valid
  CNF formula which does not contain valid clauses, so that $\applymuvi$
  must be $\top$, hence $\mu\validates\vi$.
%}
% We guess this equivalence is the reason why these two concepts are rarely
% distinguished in the literature.


Unfortunately, when dealing with generic (non-CNF) formulas, 
we notice that \emph{Definitions~\ref{def:validation} and
\ref{def:entailment}  are not equivalent, the former being
strictly stronger than the latter}. 
%\noindent
In fact, as above, if $\mu\validates\vi$ then obviously
% ,  for every $\eta$ s.t.
% $\eta\supseteq\mu$, $\eta\validates\vi$ and thus $\eta\models\vi$, hence
$\mu\entails\vi$, whereas {\em the converse is not true}: e.g.,
if $\vi\defas(A_1\wedge A_2)\vee (A_1\wedge \neg A_2)$ and 
$\mu\defas\set{A_1}$, 
then 
$\mu\entails\vi$ but $\mu\not\validates\vi$.
%
This leads to the following statement.

\begin{proposition}
\label{prop:stronger}
If a partial truth assignment $\mu$ {\verbvalidates{}}
$\varphi$, then it also {entails} $\varphi$, but the converse does
not hold.
% : 
% $\mu\validates\vi \thus \mu\entails\vi$ but 
% $\mu\entails\vi \not\thus \mu\validates\vi$.
\end{proposition}
%
\begin{IGNOREINSHORT}
\begin{example}
%~\footnote{%
Let
$\mu\defas\set{A_1,..,A_M}$ s.t. $M<N$ and
$\vi\defas\bigvee_i (A_i\wedge cube_i)$ s.t. each $cube_i$ is a cube and $\bigvee_i cube_i$ is
valid and does not contain occurrences of the atoms $A_1,..,A_M$. Then 
$\mu\entails\vi$ but \applymuvi{} is the valid formula $\bigvee_i
cube_i$, so that $\mu\not\validates\vi$. \hfill $\diamond$
%}  
\end{example}  
\end{IGNOREINSHORT}


We try to build a counterpart of Property~\ref{prop:total-properties}
for Definitions~\ref{def:validation} and
\ref{def:entailment} respectively, but in both cases we fail to
achieve all points (i)-(iv) in Property~\ref{prop:total-properties},
resulting into complementary situations.
%

%\subsubsection{Pros and cons of partial-assignment satisfiability as validation.}
%%% Validation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
From Definition~\ref{def:validation}
we easily derive the following facts. 
(Here ``\oksym{}'' \resp{``\noksym{}''} denotes facts from
Property~\ref{prop:total-properties} which are \resp{are not} preserved.)

\begin{property}
\label{prop:partial-validation}
Let $\mu$ be a partial truth assignment on \alla{} and
$\vi,\vione,\vitwo$ be formulas on \alla. 
\begin{renumerate}
\item \noksym{}
If $\mu\validates\varphi$ then $\andmu\entails\varphi$, {but not vice versa}.
\item \noksym{}
If $\vione$ and $\vitwo$ are  equivalent, this {does not} imply
that $\mu\validates\vione$ iff $\mu\validates\vitwo$.
\item \oksym{}
  $\mu\validates\varphi$ iff \applymuvi{} is $\top$
     (also, iff $\muof{\vi}= \tval$ by Property~\ref{prop:eval-simplifies}). 

\item \oksym{}
Checking
$\mu\validates\vi$  requires at most a polynomial amount of steps.
\end{renumerate}  
\end{property}

%\subsubsection{Pros and cons of partial-assignment satisfiability as entailment.}
%%% Entailment
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
From Definition~\ref{def:entailment}
we easily derive the following. 

\begin{property}
\label{prop:partial-entailment}
Let $\mu$ be a partial truth assignment on \alla{} and
$\vi,\vione,\vitwo$ be formulas on \alla. 
\begin{renumerate}
\item \oksym{}
$\mu\models\varphi$ iff $\andmu\entails\varphi$.
\item \oksym{}
If $\vione$ and $\vitwo$ are  equivalent, then 
$\mu\models\vione$ iff $\mu\models\vitwo$.
\item \noksym{}
  $\mu\models\varphi$ iff \applymuvi{} is a valid formula, not
  necessarily $\top$
   (also, in general $\muof{\vi} \neq \tval$). 
\item \noksym{}
Checking
$\mu\entails\vi$ is \emph{co-NP-complete}.
\footnote{In fact, checking the validity of \vi{}
translates into verifying that the empty assignment
entails it.}
\end{renumerate}  
\end{property}
\noindent


\TODO{Riscrivi prossimo paragrafo}
\marg{\Verbvalidation{} vs. Entailment.}
The advantage of adopting \verbvalidation{} for checking
% as a definition of
partial-assignment satisfiability is that it matches the intuition
and practical need that the process of checking it should be fast (Property~\ref{prop:partial-validation}(iv)).  
%
The main drawback is that 
that equivalent although syntactically different 
formulas may be satisfied by different sets of partial
assignments  (Property~\ref{prop:partial-validation}(ii)), 
which looks theoretically awkward. 
%even partial (Property~\ref{prop:partial-entailment}(ii)). 
\ignoreinshort{%
We believe this would be an embarrassing fact
if we adopted \verbvalidation{} as the definition of  partial-assignment
satisfiability for non-CNF formulas.
}

%\TODO{We believe this is quite embarassing...}

On the one hand, 
the advantage of adopting entailment
%as a definition of
%Definition~\ref{def:entailment} as
for checking
partial-assignment satisfiability is that it matches the intuition 
and theoretical requirement
that equivalent formulas should be satisfied by the same assignments,
even partial ones (Property~\ref{prop:partial-entailment}(ii)). 
%
On the other hand, the price to pay is that the resulting problem 
is co-NP-complete  (Property~\ref{prop:partial-entailment}(iv)),
because it is equivalent to checking the validity of the residual \applymuvi.


\smallskip
Due to Proposition~\ref{prop:stronger}, every
 partial assignments entailing the input formula is  a \emph{subset}
 of some other(s) \verbvalidating{} it.
Therefore, for an assignment-enumeration algorithm,
 being able to enumerate partial 
assignments entailing the input formula rather than simply \verbvalidating{}
it  may (even drastically) reduce the number of the satisfying assignment
enumerated. 
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Procedures using \verbvalidation and entailment.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Procedures using \verbvalidation{} and entailment.}
We notice that, when applied to satisfiable formulas,
algorithms like \new{Analytic Tableaux}~\footnote{Notice that Analytic Tableaux may generate duplicated
 or subsumed  assignments (see \cite{dagostino1,gs-infocomp2000})}
\cite{smullyan1} 
or ``classic'' \new{DPLL}~%
\footnote{Classic DPLL procedure \cite{davis7} was
  designed to work for CNF  
  formulas. Nevertheless it is easy to produce non-CNF a version of this
procedure (see e.g. \cite{armando5}).} 
%
\cite{davis7} produce branches representing
partial assignments which {\em \verbvalidate} the input formula
(Definition~\ref{def:validation}). Consequently, 
as soon as these procedures produce (a branch corresponding to) an assignment
$\mu$ s.t. 
$\mu\entails\vi$ but $\mu\not\validates\vi$, they cannot realize this
fact and
proceed the search until they extend it to some $\mu'\supset\mu$ s.t. 
$\mu'\validates\vi$. This causes an extension of the search tree of up to
$2^{||\mu'||-||\mu||}$ branches.  
%
OBDDs instead \cite{bryant2} produce branches representing
partial assignments which {\em entail} the input formula
(Definition~\ref{def:entailment}), because if $\mu\entails\vi$ then
\applymuvi is
valid (Property~\ref{prop:partial-entailment}(iii)), so that its corresponding 
sub-OBDD is reduced into the $\top$ node.
%\input{figure.tex}
\input{figure_long.tex}
%
\begin{example}
Consider $\vi\defas\mainwff$. 
  Figure~\ref{fig:comparison} 
represents 
the search trees corresponding to 
All-SAT executions of Analytic
Tableaux and 
(non-CNF) DPLL on $\vi$,%
\footnote{Here in DPLL the pure-literal rule \cite{davis7} is not used because 
 in All-SAT it may hinder the enumeration of
 some relevant models (see, e.g., \cite{sebastiani_frocos07}).}  
and the OBDD for $\vi$.
The former two produce the assignments \allmus{}.
The latter produces the single assignment
\singlemu{}, s.t. $\singlemu\entails\vi$ but $\singlemu\not
\validates\vi$.
% Notice that neither Analytic Tableaux nor DPLL can produce \singlemu{} alone.
\hfill$\diamond$
\end{example}
\TODO{Aggiungere XDDs? }


%\NOTE{Spiegare. }
%\begin{IGNOREINSHORT}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Other possible partial-satisfaction relations.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Other possible partial-satisfaction relations.}
Given the above facts, we wonder if we could use other notions
of partial-assignment satisfiability (e.g., we could enrich
$\validates$ with some form of formula simplification).
In particular, we wonder if there exists some suitable notion of
partial-assignment satisfaction which is strictly stronger than
entailment and fixes the ``embarassing issue'' of
Property~\ref{prop:partial-validation}(ii).
The following theorem states this is not the case.
\begin{theorem}
\label{uniqueness:teo}
Let $\genericentails$ denote some generical relation between a (possibly partial)
truth assignment  and a Boolean formula, such that
% \RSTODO{sostituire (a) con ``if $\eta$ total for $\vi$, then
%   $\eta\genericentails\vi$ iff
%   $\eta\models\vi$? Da questo deriva anche (b)?}
\begin{aenumerate}
\item  if $\eta$ is total for $\vi$, then
  $\eta\genericentails\vi$ iff
  $\eta\models\vi$;
\item for every $\mu$, $\vi_1$ and $\vi_2$, if $\mu\genericentails\vi_1\wedge\vi_2$, then $\mu\genericentails\vi_1$ and
  $\mu\genericentails\vi_2$;
\item there exist $\mu$ and $\vi$ s.t. $\mu\entails\vi$ and $\mu\not\genericentails\vi$ .
\end{aenumerate}
Then there exist $\mu'$, $\psi_1$ and $\psi_2$ s.t. $\psi_1\equiv\psi_2$, 
$\mu'\genericentails\psi_1$ and $\mu'\not\genericentails\psi_2$.
\end{theorem}
\begin{proof}
%% PROOF VERIFICATA
  Consider $\mu$ and $\vi$ as in point {\em (c)}.
  Let $\mu'\defas\mu$,
  $\psi_1\defas\andmu$ and $\psi_2\defas\andmu\wedge\varphi$.
  Then $\psi_1\equiv\psi_2$ because $\mu\entails\vi$ and because of
  Property~\ref{prop:partial-entailment}(i); also, $\mu'\genericentails\psi_1$
  by point {\em (a)} and $\mu'\not\genericentails\psi_2$ by point {\em
    (b)}.
  \hfill $\diamond$
\end{proof}
Theorem \ref{uniqueness:teo} says that entailment is
the only relation
which extends to partial assignments the standard notion of
total-assignment satisfaction
(point $(a)$), maintains the standard semantics of
$\wedge$ (point $(b)$) and verifies
Property~\ref{prop:partial-entailment}(ii).
Any relation $\genericentails$ which is strictly stronger than $\models$ suffers for
the same ``embarassing issue'' of
Property~\ref{prop:partial-validation}(ii) (point $(c)$).
% Theorem \ref{uniqueness:teo} says that if a relation $\genericentails$
% extends to partial assignments the standard notion of satisfaction
% (point $(a)$), maintains the standard semantics of
% $\wedge$ (point $(b)$) and
% is strictly stronger than entailment (point $(c)$), than it does not verify
% Property~\ref{prop:partial-entailment}(ii), that is, it suffers for
% the same ``embarassing issue'' of
% Property~\ref{prop:partial-validation}(ii).
%\end{IGNOREINSHORT}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Dealing with CNF-ized formulas.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Dealing with CNF-ized formulas.}
One may argue that in SAT/AllSAT the distinction between $\validates$ and
$\entails$ is not much relevant in practice, because we can
CNF-ize upfront the input formulas ---typically by
variants of Tseitin CNF-ization--- removing tautological clauses, and this
distinction does not hold for (tautology-free) CNF
formulas.
%
However, we notice that with Tseitin CNF-ization we may loose
information regarding entailment or \verbvalidation{}. In fact, if
$\psi$ on $\alla\cup\allb$ is the result of Tseitin CNF-izing $\vi$,
then:
\begin{itemize}
% \item 
% If $\mu\cup\gamma\validates\phi$ for some total truth assignment
%   $\gamma$, then $\mu\validates\vi$.
% \item 
% If $\mu\cup\gamma\entails\phi$ for some total truth assignment
%   $\gamma$, then $\mu\entails\vi$.
\item 
$\mu\validates\vi$ \emph{does not imply} that there exists a total assignment
  $\delta$ on \allb s.t. $\mu\cup\delta\validates\psi$;
\item 
$\mu\entails\vi$ \emph{does not imply} that there exists a total assignment
  $\delta$ on \allb s.t. $\mu\cup\delta\entails\psi$.
\end{itemize}

\begin{example}
Consider $\vi\defas A_1 \vee (A_2\wedge A_3)$ 
and its Tseitin CNF-ized version:\\
$
\begin{array}{lll}
\psi\defas & (A_1\vee  B_1)\ \wedge \\
& (\neg B_1 \vee  A_2) \wedge
(\neg B_1 \vee  A_3) \wedge 
(B_1\vee \neg A_2 \vee \neg A_3) & \ \ \ //\ B_1 \iff (A_2\wedge A_3). \\
\end{array}
$\\
On the one hand, $\mu\defas \set{A_1}$ is such that $\mu\validates\vi$. 
On the other hand, there is no total truth assignment $\delta$ on
\set{B_1} s.t. $\mu\cup\delta\validates\psi$. In fact, neither 
$\set{A_1,B_1}\validates\psi$ nor $\set{A_1,\neg B_1}\validates\psi$.

Consider $\vi\defas
(A_1\wedge \pos A_2)\vee (A_1\wedge\neg A_2) 
$ 
and its Tseitin CNF-ized version:\\
$
\begin{array}{lll}
\psi\defas  
& (B_1\vee B_2)\ \wedge & \\
& (\neg B_1 \vee \pos A_1) \wedge
(\neg B_1 \vee \pos A_2) \wedge
(B_1\vee \neg A_1 \vee \neg A_2)\ \wedge\ & \ \ \ //\ B_1 \iff (A_1\wedge \pos A_2) \\
& (\neg B_2 \vee \pos A_1) \wedge
(\neg B_2 \vee \neg A_2) \wedge
(B_2\vee \neg A_1 \vee \pos A_2).\ & \ \ \ //\ B_2 \iff (A_1\wedge \neg A_2) 
\end{array}
%
% \psi\defas
% (B_1\vee B_2) \wedge
% (\neg B_1 \vee A_1) \wedge
% (\neg B_1 \vee A_2) \wedge
% (B_1\vee \neg A_1 \vee \neg A_2) \wedge
% (\neg B_2 \vee \neg A_1) \wedge
% (\neg B_2 \vee \neg A_2) \wedge
% (B_2\vee \neg A_1 \vee A_2)   
$\\
Although $\mu\defas \set{A_1}$ is such that $\mu\entails\vi$,
%On the other hand,
 there is no total truth assignment $\delta$ on
\set{B_1,B_2} s.t. $\mu\cup\delta\entails\psi$:
$\set{A_1,B_1,\neg B_2}\not\entails \psi$ since
$\set{A_1,\neg A_2,B_1,\neg B_2}\not\entails \psi$;
$\set{A_1,\neg B_1,B_2}\not\entails \psi$
since $\set{A_1,A_2,\neg B_1,B_2}\not\entails \psi$;
$\set{A_1,B_1,B_2}$ and $\set{A_1,\neg B_1,\neg B_2}$ are both inconsistent
with $\psi$.
\hfill $\diamond$
\end{example}

\ignore{%%%%%%%%%%
\begin{proposition}
 \RSTODO{PROVA e scrivi controesempi. Scrivi in background l'equivalente controparte per $\eta \models\vi$\\}
Let $\vi$ be a generic (non-CNF)
formula on \alla and let $\psi$ on $\alla\cup\allb$ be the result of
CNF-izing \vi by applying standard Tseitin CNF-ization 
\cite{tseitin1} and removing valid clauses from $\psi$ if any, \allb
being the set of fresh propositions introduced in the process. Then:
\begin{itemize}
\item 
If $\mu\cup\gamma\validates\psi$ for some total truth assignment
  $\gamma$, then $\mu\validates\vi$.
\item 
If $\mu\cup\gamma\entails\psi$ for some total truth assignment
  $\gamma$, then $\mu\entails\vi$.
\item 
$\mu\validates\vi$ \emph{does not imply} that there exists a total assignment
  $\delta$ on \allb s.t. $\mu\cup\delta\validates\vi$
\item 
$\mu\entails\vi$ \emph{does not imply} that there exists a total assignment
  $\delta$ on \allb s.t. $\mu\cup\delta\entails\vi$
\end{itemize}

%Then $\mu\validates\vi$, but
%$\mu\entails\vi$
\end{proposition}
}


==> arxiv-version/practical.tex <==
%\newpage
% \TODO{dal punto di vista della soddisfcibilità non fa grande
%   differenza. Dal punto di vista dell'enumerazione si.}

In this section we analyze the practical consequences of adopting
\verbverification{} or entailment as a partial-assignment
satisfiability tests in search procedures for satisfiability and
enumeration and in formula compilation. In particular,
when entailment and verification do not coincide, we analyze the
tradeoff between the extra cost of entailment versus the benefits it may
produce. 

%\subsection{\Verbverification{} vs. entailment in practice}
\subsection{\Verbverification{} vs. entailment in solving, enumeration
and compilation}
\paragraph{\Verbverification{} vs. entailment for native CNF formulas.}
%\marg{$\verifies$ vs $\entails$ with CNF}
  When the input formula is natively in CNF, the 
  distinction between \verbverification{} and entailment is not relevant, because these two concepts
  coincide. (We conjecture that this is the main reason why the distinction between
\verbverification{} and entailment has been long overlooked in the literature.)
%
For satisfiability of CNF formulas, CDCL SAT solvers directly produce
  {\em total} truth assignments, because it is not worth to perform
  intermediate satisfiability checks. 

\paragraph{\Verbverification{} vs. entailment in satisfiability.}
%\marg{$\verifies$ vs $\entails$ in SAT}
In plain satisfiability we need
finding only one total assignment $\eta$ extending $\mu$ which satisfy
$\vi$.
Therefore
entailment produces no benefits
wrt. \verbverification{} and is more expensive, so that the latter is
always preferred.


\smallskip
The scenario changes when we deal with
enumeration-based algorithms applied to non-CNF formulas, or to
existentially-quantified formulas, or to CNF-ized formulas.

%\paragraph{Pros and cons of \verbverification{} and entailment.}
\paragraph{\Verbverification{} vs.  entailment for enumeration on
  non-CNF formulas.}
The analysis in \sref{sec:partialsat-plain} shows the following facts.
On the one hand, the advantage of adopting \verbverification{} rather than entailment for checking
%\marg{$\verifies$ faster than $\entails$...}
% as a definition of
partial-assignment satisfiability is that
it matches the intuition
and practical need that satisfiability checking should be fast,
since
 checking \verbverification{}
is polynomial (property~\ref{prop:partial-verification}(iv)) and easier
to implement, whereas checking
entailment is co-NP-complete  (property~\ref{prop:partial-entailment}(iv)),
because it is equivalent to checking the validity of the residual \applymuvi{}.
%
%\marg{... but not so much}
We stress the fact, however, that if $\mu\entails\vi$, then the residual
\applymuvi{} is typically much smaller than \vi with a much
smaller search space, since its
variables are only (a subset of) the variables which are not assigned
by $\mu$, 
so that in many actual situations the above fact could not be a major issue.



On the other hand, a main advantage of adopting entailment on
enumeration is that,
due to \cref{prop:stronger}, every
 partial assignments entailing the input formula is  a \emph{sub-assignment}
 of some other(s) \verbverifying{} it.
%
 Consequently, 
as soon as one verification-based enumeration procedure produces (a branch corresponding to) an assignment
$\mu$ s.t. 
$\mu\entails\vi$ but $\mu\not\verifies\vi$, it cannot realize this
fact and thus
proceeds the search to extend $\mu$ to some $\mu'\supset\mu$ s.t. 
$\mu'\verifies\vi$. This causes an extension of the search tree of up to
$2^{|\mu'|-|\mu|}$ branches.  
%
Therefore, for an assignment-enumeration algorithm,
 being able to enumerate partial 
assignments entailing the input formula rather than simply \verbverifying{}
it  may (even drastically) reduce the number of the satisfying assignment
enumerated. 

%\paragraph{Improving \verbverification.}
Also, the analysis in \sref{sec:partialsat-others} shows that
%\RSTODO{TODO: move this paragraph below?} 
alternative forms of partial-assignment satisfiability extending
\verbverification{} ---e.g.,
adding further simplifications for the residual $\applymuvi$  like unit-propagation
or the removal of basic valid subformulas--- cannot fill %completely
the  gap wrt. entailment, whose theoretical properties are specific.


\paragraph{\Verbverification{} vs. entailment for
  projected enumeration.}
The analysis in \sref{sec:partialsat-exist} shows that
% Due to \cref{prop:stronger-exists}
the above considerations for non-CNF formulas extend automatically to procedures for projected
enumeration (e.g. projected AllSAT/AllSMT, projected \#SAT/\#SMT),
even on CNF formulas, because projected enumeration
consists in enumeration on an
existentially-quantified formula $\exists \allb.\psi$, $\allb$ being
the  non-relevant atoms to be projected away.
The same considerations apply  also to other applications like the
computation of 
  preimages in symbolic model checking \cite{burch1} or
 predicate abstraction in SW verification \cite{graf_predabs97,lahiriSMTTechniquesFast2006}. 

%\TODO{Parlare di enumeratio per non-CNF e projected enumeration in generale}



\paragraph{\Verbverification{} vs. entailment for
  CNF-ized non-CNF formulas.}
%\RSTODO{TODO: revise this paragraph} 
The analysis in \sref{sec:partialsat-cnf} shows that,
although verification and entailment coincide for CNF formulas, 
the problem with non-CNF formulas cannot be fixed by simply CNF-izing a formula
upfront \cite{tseitin1,plaistedStructurepreservingClauseForm1986}
and running a CNF enumeration procedure based on partial-assignment
verification, projecting out the fresh variables introduced by the CNF-ization.
In fact, a partial assignment over the original
    atoms may entail the existentially-quantified CNF-ized
    formula without \verbverifying{} it.
Also, even adopting the  CNF-ization technique \PlaistedCNF(\NNF{\vi}) we proposed in
\cite{masinaCNFConversionDisjoint2023}, although improving
the enumeration process, does not fill the gap between
\verbverification{} and entailment in this case.

\ignore{CNF-izing upfront the non-CNF formula with the standard
  techniques \cite{tseitin1,plaistedStructurepreservingClauseForm1986}
  does not fix issues $(a)$-$(c)$, since fresh atoms are
  introduced, and \emph{a partial assignment over the original
    atoms may entail the existentially-quantified CNF-ized
    formula without \verbverifying{} it.}
  }
%
%In fact, %  This is important because it shows that,

\paragraph{\Verbverification{} and entailment in formula compilation.}
%\RSTODO{aggiungi citazioni}
With formula compilers a formula $\vi$ is encoded into a
format which makes assignment enumeration straightforward \cite{darwicheKnowledgeCompilationMap2002}.\\
%
d-DNNF formulas are NNF DAGs which are {\em decomposable} (i.e., all
conjunctive subformulas $\vi_1\wedge \vi_2$ are such that $\vi_1$ and
$\vi_2$ do not share atoms) and {\em deterministic} (i.e., all
disjunctive subformulas $\vi_1\vee \vi_2$ are such that $\vi_1$ and
$\vi_2$ are mutually inconsistent)  \cite{darwicheCompilerDeterministicDecomposable2002}.
%
The d-DNNF compilers typically implement a top-down search, implicitly
%\RSTODO{Spostare fuori dall'esempio?}
adopting \verbverification{} ($\applymuvi=\top$) 
as partial-assignment satisfiability test \cite{DarwicheDNNF-ACM01}.

OBDDs~\cite{bryant2} and SDDs~\cite{darwicheSDDNewCanonical2011} are subcases of
d-DNNFs \cite{darwicheKnowledgeCompilationMap2002} which are canonical under some
order condition  ---i.e., two equivalent subformulas \vione{} and
\vitwo{} are encoded into the same OBDD or SDD, and as such are shared
inside the DAG representation.
The OBDD and SDD compilers typically build the encoding
bottom-up, and they are able to encode 
$\applymuvi$ into $\top$ as soon as $\applymuvi$ becomes valid.
(That is, they implicitly use entailment as partial-assignment satisfiability test.) 


% \TODO{TODO\\
% - d-DNNF (based on \verbverification{}) vs. OBDDs and
% SDDs (based on entailment)\\
% - enumeration via OBDDs and SDDs\\
% - Theory OBDDs and SDDs \cite{MicheluttiEcai24}
% }


\paragraph{\Verbverification{} and entailment for \#SMT and WMI.}
%\paragraph{Effectiveness vs. efficiency for \#SMT and WMI.}
With some enumeration-based techniques (e.g. \#SMT \cite{chisticov15,PhanM15} and WMI
\cite{morettin_aij19,spallittaEnhancingSMTbasedWeighted2024a})
the total cost of {\em processing} each enumerated partial assignment dominates that of
the enumeration itself.
%
(E.g., with WMI each satisfying assignment $\mu$ corresponds to a polytope, and
for each $\mu$ it is necessary to compute
the integral of some multivariate function over such polytope.)
Therefore, in this context the {\em effectiveness} of enumeration in
reducing the number of assignments generated is even more important
that the {\em efficiency} in terms of CPU time required to enumerate them.   
\ignore{(Specialized techniques to reduce the number of enumerated assignments in WMI have been
proposed in \cite{morettin_aij19,spallittaEnhancingSMTbasedWeighted2024a}.)}
Therefore,  with entailment-based enumeration  the reduced number of assignments produced, and hence of
integrals computed, should definitely compensate the extra cost of
entailment checking. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%% Procedures using \verbverification and entailment.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Procedures using either \verbverification{} or entailment.}
\subsection{\Verbverification{} vs. entailment in search
  procedures and formula compilers.}
When applied to satisfiable formulas,
%\RSTODO{add example enumeration of CNF-ized formula?}
algorithms like \new{Analytic Tableaux}~\footnote{Notice that Analytic Tableaux may generate duplicated
 or subsumed  assignments (see \cite{dagostino1,gs-infocomp2000})}
\cite{smullyan1} 
or ``classic'' \new{DPLL}~%
\footnote{Classic DPLL procedure \cite{davis7} was
  designed to work for CNF  
  formulas. Nevertheless it is easy to produce non-CNF a version of this
procedure (see e.g. \cite{armando5}).} 
%
\cite{davis7}, or even recent sophisticate AllSAT procedures for circuits~\cite{friedAllSATCombinationalCircuits2023},
 produce branches representing
partial assignments which {\em \verbverify} the input formula.
The same happens with enumeration algorithms for d-DNNF formulas,
which resemble the  tableaux enumeration algorithm,
with the restriction that the formulas they are applied to
are deterministic and decomposable NNFs, 
% (i.e., all conjunctive subformulas $\vi_1\wedge \vi_2$
% are such that $\vi_1$ and $\vi_2$ do not share atoms) 
%\RSTODO{aggiungi citazioni}
% and deterministic
% (i.e., all disjunctive subformulas $\vi_1\vee \vi_2$
% are such that $\vi_1$ and $\vi_2$ are mutually inconsistent),
so that
the enumerated assignment are pairwise disjoint and straighforward to
compute, because the enumeration reduces to the traversal of the and-or %d-DNNF
DAG without encountering inconsistent branches
\cite{DarwicheDNNF-ACM01}.
%\cite{darwicheCompilerDeterministicDecomposable2002,darwicheKnowledgeCompilationMap2002,lagniezLeveragingDecisionDNNFCompilation2024}. 

\ignore{%% SPOSTATO SOPRA
  Consequently, 
as soon as these procedures produce (a branch corresponding to) an assignment
$\mu$ s.t. 
$\mu\entails\vi$ but $\mu\not\verifies\vi$, they cannot realize this
fact and
proceed the search until they extend it to some $\mu'\supset\mu$ s.t. 
$\mu'\verifies\vi$. This causes an extension of the search tree of up to
$2^{|\mu'|-|\mu|}$ branches.  
}

% %%%%% EXAMPLE tableaux, DPLL, d-DNNF enumeration
\begin{example}
\label{ex:enumeration-basic}
%\marg{tableaux, DPLL, d-DNNF enumeration}
Consider $\vi\defas\mainwff$.\\
Notice that the single assignment $\mu\defas\singlemu{}$
subsumes all total truth assignments satisfying \vi and
is such that
$\mu\entails\vi$ but $\mu\not
\verifies\vi$, since $\applymuvi=(\Atwo\vee\nAtwo)\wedge(\Afour\vee\nAfour)$.

Figure~\ref{fig:search} 
represents 
the search trees corresponding to 
AllSAT executions of Analytic
Tableaux and %d-DNNF enumeration and 
(non-CNF) DPLL  
on $\vi$,%
\footnote{Here in DPLL the pure-literal rule \cite{davis7} is not used because 
 in All-SAT it may hinder the enumeration of
 relevant models (see, e.g., \cite{sebastiani_frocos07}).}
\footnote{The search trees may vary with the ordering by
  which variables and subformulas are analyzed.}
Since (the DAG version of) $\vi$ is already in d-DNNF
(\cref{fig:compilers}), in this case the d-DNNF enumeration resembles the
tableaux enumeration. 
In all cases the enumeration produces:~%
\\\allmus{}.
Notice that all the assignments produced are total.
Notice also that neither Analytic Tableaux nor DPLL nor d-DNNF
enumeration in this case can produce
\singlemuset{}, regardless the strategy adopted.
The same applies also to the \verbverification-based AllSAT circuit
enumeration of \cite{friedAllSATCombinationalCircuits2023}, see \cref{ex:enumeration-entail}.
\hfill$\diamond$
\end{example}



OBDDs \cite{bryant2} contain branches representing
partial assignments which {\em entail} the input formula, because if $\mu\entails\vi$ then
\applymuvi is
valid (property~\ref{prop:partial-entailment}(iii)), so that its corresponding 
sub-OBDD is reduced into the $\top$ node. (SDDs~\cite{darwicheSDDNewCanonical2011} behave similarly.)

%\input{figure.tex}
%\input{figure_long.tex}


%  
\begin{figure}[t]
  \begin{tabular}{lll}
    \scalebox{.8}{\input{tableau.pdf_t}} 
    &\ \hspace{.5cm} &
    \scalebox{.8}{\input{dpll.pdf_t}}       
  \end{tabular}
  \caption{\label{fig:search} $\vi\defas\mainwff{}$.
    \newline
    Enumeration by  analytic tableaux (left) and (non-CNF) DPLL (right).
%\\With both procedures the enumeration produces:\\\allmus{}
}
\ \\
  \begin{tabular}{lllll}
    \scalebox{.8}{\input{ddnnf.pdf_t}} 
    &\ \hspace{.2cm} &
    \scalebox{.8}{\input{obdd.pdf_t}} 
    &\ \hspace{.2cm} &
    \scalebox{.8}{\input{sdd.pdf_t}} 
  \end{tabular}
  \caption{\label{fig:compilers} $\vi\defas\mainwff{}$.
  \newline Compilation of $\vi$ into: d-DNNF (left), OBDD (center), SDD (right).
\\ }  
%
%\TODO{add example with dualiza/HALL}
%\TODO{Add example of enumeration of CNF-ized formula}
\end{figure} 



%
\begin{example}
\label{ex:compilation}
%\marg{d-DNNF, OBDD, SDD}
Consider $\vi$ as in \cref{ex:enumeration-basic}.
  Figure~\ref{fig:compilers} represents possible compilations of $\vi$
  into d-DNNF, OBDD and SDD respectively.~\footnote{The outcome may
    vary with the ordering by
  which variables and subformulas are analyzed.}
% \ignore{
% The d-DNNF compilers typically implement a top-down search, implicitly
% \RSTODO{Spostare fuori dall'esempio?}
% adopting \verbverification{} ($\applymuvi=\top$) 
% as partial-assignment satisfiability test. 
% The OBDD and SDD compilers instead typically build the encoding
% bottom-up, and they are able to encode 
% $\applymuvi$ into $\top$ as soon as $\applymuvi$ becomes valid.
% (That is, they implicitly use entailment a as partial-assignment satisfiability test.) 
% }
Notice that, unlike with OBDDs and SDDs which collapse equivalent
subformulas into one,  the two $\vee$-subformulas in the d-DNNF are not
recognized to be equivalent to the nodes $\Aone$ and $\nAthree$
respectively. 

Applying enumeration to the d-DNNF we obtain the total
assignments of \cref{ex:enumeration-basic}:\\\allmus{}.
By applying enumeration to the OBDD or to the SDD, we obtain
the single-assignment \singlemuset{}, so that $\singlemu\entails\vi$ but $\singlemu\not
\verifies\vi$.
% Notice that neither Analytic Tableaux nor DPLL can produce \singlemu{} alone.
\hfill$\diamond$
\end{example}




\subsection{Implementing entailment within enumeration procedures}
% \TODO{
%   Explain Dualization:\\
%   - basic ideas\\
%   - strategies\\
%   Explain HALL\\
% Implementations and results
% } 
%
Implementing efficiently entailment-based enumeration procedures can be
tricky. One possible approach is to
integrate AllSAT/AllSMT with OBDDs, exploiting the capability of OBDD
to implicitly perform entailment-based reductions \cite{cavada_fmcad07_predabs}. The main problem
with this approach is the fact that OBDDs quickly blow up in memory as
soon as the input formula increases in size.

\cite{FazekasSB16,mohleDualizingProjectedModel2018} proposed a formal
reasoning framework based on the idea of {\em dualized search}:
while the main enumerator produces partial assignments $\mu$ for the input
formula $\vi$, another ``dual'' SAT solver is incrementally called on
$\TseitinCNF(\neg\vi)\wedge\andmu$: if it is unsatisfiable
%(i.e. if $\mu\models\vi$)
then the main enumerator produces  $\mu$ and
backtracks. %, continues the search.
Based on the analysis in \cite{sebastianiAreYouSatisfied2020} and
noticing that the above dual check in
\cite{FazekasSB16,mohleDualizingProjectedModel2018} is an entailment
($\mu\entails\vi$) rather than a \verbverification{} ($\mu\verifies\vi$), in \cite{moehle20,moehle21} we
proposed enumeration and model counting frameworks and algorithms
based on dual search, enhanced with chronological backtracking. 
%
Unfortunately no
implementation efficient enough to compete with s.o.a. enumeration
procedures was produced.

\cite{friedAllSATCombinationalCircuits2023} presented {\sf HALL}, a sophisticate AllSAT
procedure for circuits which, among other techniques, exploited a form of
(\verbverification-based) {\em generalization} (aka minimization or reduction): as soon as a 
total truth assignment $\eta$ satisfying $\vi$ is produced,
the literals in $\eta$ are removed one by one and the resulting
partial assignment is tested to \verbverify{} $\vi$.
In \cite{friedEntailingGeneralizationBoosts2024}
we
 have enhanced {\sf HALL} generalization procedure by substituting
 \verbverification{} checks with entailment checks based on dualized
 search, boosting its performance in terms of both time efficiency and size of 
 partial-assignment sets.

%% EXAMPLE ENUMERATION WITH ENTAILMENT
\begin{example}
\label{ex:enumeration-entail}
Consider $\vi\defas\mainwff$\\ as in \cref{ex:enumeration-basic} and
assume some total assignment satisfying it is produced,
e.g. $\eta\defas \set{\Aone,\Atwo,\nAthree,\Afour}$.
Since there is no literal $l\in\eta$
s.t. $\eta\backslash\set{l}\verifies\vi$, no assignment
reduction based on verification can be successfully applied to $\eta$.
Consequently, even the sophisticate \verbverification{}-based circuit AllSAT procedure in
\cite{friedAllSATCombinationalCircuits2023} produces the set of four
un-reduced total assignments of \cref{ex:enumeration-basic}.

Instead, since $\eta\backslash\set{\Atwo,\Afour}\entails\vi$
whereas $\eta\backslash\set{\Aone}\not\entails\vi$ and
$\eta\backslash\set{\nAthree}\not\entails\vi$,
the entailment-based assignment-reduction technique of
\cite{friedEntailingGeneralizationBoosts2024}  shrinks $\eta$ into
$\singlemu$, so that the enumeration procedure returns $\singlemuset$.
\hfill$\diamond$
\end{example}


\ignore{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\TODO{Aggiunte da prima, piazzare da qualche parte:\\}
In many application domains, fundamental operations ---like {\em 
\RSTODO{rivedere questo paragrafo?}
  preimage computation} in symbolic model checking
(see e.g. \cite{burch1}) or {\em predicate abstraction} in SW verification
(see e.g. \cite{graf_predabs97,beyercgks09})---
require dealing with existentially-quantified formulas and with
the enumeration of partial assignments satisfying them.
(This applies implicitly also to a formula $\psi$ resulting from
Tseitin CNF-ization of some formula $\vi$, because
$\vi(\alla)\equiv\exists.\allb\psi(\alla,\allb)$ (see \sref{sec:background}).)
} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> arxiv-version/related.tex <==

  % \nocite{plaistedStructurepreservingClauseForm1986,friedEntailingGeneralizationBoosts2024,friedAllSATCombinationalCircuits2023,darwicheCompilerDeterministicDecomposable2002,spallittaDisjointPartialEnumeration2024,moehle21,moehle20,chisticov15,PhanM15,mohleDualizingProjectedModel2018,morettin_aij19,sebastianiAreYouSatisfied2020,lagniezLeveragingDecisionDNNFCompilation2024}
  
\paragraph{Related Work.}
%\subsection{Related Work}
\label{sec:related}
This paper is a revised version of a 2020  unpublished paper
\cite{sebastianiAreYouSatisfied2020}, which at that time was not published due to
lack of algorithmic support and empirical evidence.
%
These came afterwards. Based on the theoretical analysis in 
\cite{sebastianiAreYouSatisfied2020} in combination with the idea of dualized search
from \cite{FazekasSB16,mohleDualizingProjectedModel2018},
in~\cite{moehle20,moehle21}
we proposed novel enumeration and counting 
 procedures based on entailment. 
Unfortunately we were not able to produce any 
implementation efficient enough to compete with s.o.a. enumeration procedures based
on \verbverification.
%
Only very recently, in \cite{friedEntailingGeneralizationBoosts2024} we
 have enhanced the {\sf HALL} enumeration tool for circuits from
 \cite{friedAllSATCombinationalCircuits2023} by substituting
 \verbverification{} checks with entailment checks for
 partial-assignment reductions (``generalizations''
 in \cite{friedEntailingGeneralizationBoosts2024}),
boosting its performance in terms of both
time efficiency and size of partial-assignment sets.
% obtaining drastic
%  improvements in terms of both time efficiency and size of 
%  partial-assignment sets.

In \cite{masinaCNFConversionDisjoint2023} we addressed a problem which
is different although related to $(e)$, showing that adopting a form 
of CNF-ization different from
\cite{tseitin1,plaistedStructurepreservingClauseForm1986} improves the
efficiency and effectiveness of enumeration. Such
encoding, however, does not fix fact $(e)$ (see \sref{sec:partialsat-cnf}).


==> arxiv-version/rgb.tex <==

%% rgb.tex
%% this file defines the X11 rgb color names for use with pstricks
%% put \usepackage{pstricks, pstcol} in the preamble of your document
%% the put \input{rgb.tex} in the body of your document.
%% Color in pstricks works like a switch.  If you enter
%%    The text will become \color{red}red.
%% Then all text after the \color command will printed in red in the
%% postscript file.  You can restrict the range of the red text in this
%% manner
%%    One {\color{red}some text} will be red.
%% The color will NOT show up in the dvi file, only in the .ps file!
%%
%% this file was created by rgb2tex.pl
%% rgb2tex.pl is by Bruce Ravel <bruce.ravel@nist.gov>
%% --------------------------------------------------------------------------

\definecolor {snow}                {rgb}{1.00,0.98,0.98}
\definecolor {ghostwhite}          {rgb}{0.97,0.97,1.00}
\definecolor {whitesmoke}          {rgb}{0.96,0.96,0.96}
\definecolor {gainsboro}           {rgb}{0.86,0.86,0.86}
\definecolor {floralwhite}         {rgb}{1.00,0.98,0.94}
\definecolor {oldlace}             {rgb}{0.99,0.96,0.90}
\definecolor {linen}               {rgb}{0.98,0.94,0.90}
\definecolor {antiquewhite}        {rgb}{0.98,0.92,0.84}
\definecolor {papayawhip}          {rgb}{1.00,0.94,0.84}
\definecolor {blanchedalmond}      {rgb}{1.00,0.92,0.80}
\definecolor {bisque}              {rgb}{1.00,0.89,0.77}
\definecolor {peachpuff}           {rgb}{1.00,0.85,0.73}
\definecolor {navajowhite}         {rgb}{1.00,0.87,0.68}
\definecolor {moccasin}            {rgb}{1.00,0.89,0.71}
\definecolor {cornsilk}            {rgb}{1.00,0.97,0.86}
\definecolor {ivory}               {rgb}{1.00,1.00,0.94}
\definecolor {lemonchiffon}        {rgb}{1.00,0.98,0.80}
\definecolor {seashell}            {rgb}{1.00,0.96,0.93}
\definecolor {honeydew}            {rgb}{0.94,1.00,0.94}
\definecolor {mintcream}           {rgb}{0.96,1.00,0.98}
\definecolor {azure}               {rgb}{0.94,1.00,1.00}
\definecolor {aliceblue}           {rgb}{0.94,0.97,1.00}
\definecolor {lavender}            {rgb}{0.90,0.90,0.98}
\definecolor {lavenderblush}       {rgb}{1.00,0.94,0.96}
\definecolor {mistyrose}           {rgb}{1.00,0.89,0.88}
\definecolor {white}               {rgb}{1.00,1.00,1.00}
\definecolor {black}               {rgb}{0.00,0.00,0.00}
\definecolor {darkslategray}       {rgb}{0.18,0.31,0.31}
\definecolor {dimgray}             {rgb}{0.41,0.41,0.41}
\definecolor {slategray}           {rgb}{0.44,0.50,0.56}
\definecolor {lightslategray}      {rgb}{0.47,0.53,0.60}
\definecolor {gray}                {rgb}{0.75,0.75,0.75}
\definecolor {lightgrey}           {rgb}{0.83,0.83,0.83}
\definecolor {midnightblue}        {rgb}{0.10,0.10,0.44}
\definecolor {navy}                {rgb}{0.00,0.00,0.50}
\definecolor {cornflowerblue}      {rgb}{0.39,0.58,0.93}
\definecolor {darkslateblue}       {rgb}{0.28,0.24,0.55}
\definecolor {slateblue}           {rgb}{0.42,0.35,0.80}
\definecolor {mediumslateblue}     {rgb}{0.48,0.41,0.93}
\definecolor {lightslateblue}      {rgb}{0.52,0.44,1.00}
\definecolor {mediumblue}          {rgb}{0.00,0.00,0.80}
\definecolor {royalblue}           {rgb}{0.25,0.41,0.88}
\definecolor {blue}                {rgb}{0.00,0.00,1.00}
\definecolor {dodgerblue}          {rgb}{0.12,0.56,1.00}
\definecolor {deepskyblue}         {rgb}{0.00,0.75,1.00}
\definecolor {skyblue}             {rgb}{0.53,0.81,0.92}
\definecolor {lightskyblue}        {rgb}{0.53,0.81,0.98}
\definecolor {steelblue}           {rgb}{0.27,0.51,0.71}
\definecolor {lightsteelblue}      {rgb}{0.69,0.77,0.87}
\definecolor {lightblue}           {rgb}{0.68,0.85,0.90}
\definecolor {powderblue}          {rgb}{0.69,0.88,0.90}
\definecolor {paleturquoise}       {rgb}{0.69,0.93,0.93}
\definecolor {darkturquoise}       {rgb}{0.00,0.81,0.82}
\definecolor {mediumturquoise}     {rgb}{0.28,0.82,0.80}
\definecolor {turquoise}           {rgb}{0.25,0.88,0.82}
\definecolor {cyan}                {rgb}{0.00,1.00,1.00}
\definecolor {lightcyan}           {rgb}{0.88,1.00,1.00}
\definecolor {cadetblue}           {rgb}{0.37,0.62,0.63}
\definecolor {mediumaquamarine}    {rgb}{0.40,0.80,0.67}
\definecolor {aquamarine}          {rgb}{0.50,1.00,0.83}
\definecolor {darkgreen}           {rgb}{0.00,0.39,0.00}
\definecolor {darkolivegreen}      {rgb}{0.33,0.42,0.18}
\definecolor {darkseagreen}        {rgb}{0.56,0.74,0.56}
\definecolor {seagreen}            {rgb}{0.18,0.55,0.34}
\definecolor {mediumseagreen}      {rgb}{0.24,0.70,0.44}
\definecolor {lightseagreen}       {rgb}{0.13,0.70,0.67}
\definecolor {palegreen}           {rgb}{0.60,0.98,0.60}
\definecolor {springgreen}         {rgb}{0.00,1.00,0.50}
\definecolor {lawngreen}           {rgb}{0.49,0.99,0.00}
\definecolor {green}               {rgb}{0.00,1.00,0.00}
\definecolor {chartreuse}          {rgb}{0.50,1.00,0.00}
\definecolor {mediumspringgreen}   {rgb}{0.00,0.98,0.60}
\definecolor {greenyellow}         {rgb}{0.68,1.00,0.18}
\definecolor {limegreen}           {rgb}{0.20,0.80,0.20}
\definecolor {yellowgreen}         {rgb}{0.60,0.80,0.20}
\definecolor {forestgreen}         {rgb}{0.13,0.55,0.13}
\definecolor {olivedrab}           {rgb}{0.42,0.56,0.14}
\definecolor {darkkhaki}           {rgb}{0.74,0.72,0.42}
\definecolor {khaki}               {rgb}{0.94,0.90,0.55}
\definecolor {palegoldenrod}       {rgb}{0.93,0.91,0.67}
\definecolor {lightgoldenrodyellow} {rgb}{0.98,0.98,0.82}
\definecolor {lightyellow}         {rgb}{1.00,1.00,0.88}
\definecolor {yellow}              {rgb}{1.00,1.00,0.00}
\definecolor {gold}                {rgb}{1.00,0.84,0.00}
\definecolor {lightgoldenrod}      {rgb}{0.93,0.87,0.51}
\definecolor {goldenrod}           {rgb}{0.85,0.65,0.13}
\definecolor {darkgoldenrod}       {rgb}{0.72,0.53,0.04}
\definecolor {rosybrown}           {rgb}{0.74,0.56,0.56}
\definecolor {indianred}           {rgb}{0.80,0.36,0.36}
\definecolor {saddlebrown}         {rgb}{0.55,0.27,0.07}
\definecolor {sienna}              {rgb}{0.63,0.32,0.18}
\definecolor {peru}                {rgb}{0.80,0.52,0.25}
\definecolor {burlywood}           {rgb}{0.87,0.72,0.53}
\definecolor {beige}               {rgb}{0.96,0.96,0.86}
\definecolor {wheat}               {rgb}{0.96,0.87,0.70}
\definecolor {sandybrown}          {rgb}{0.96,0.64,0.38}
\definecolor {tan}                 {rgb}{0.82,0.71,0.55}
\definecolor {chocolate}           {rgb}{0.82,0.41,0.12}
\definecolor {firebrick}           {rgb}{0.70,0.13,0.13}
\definecolor {brown}               {rgb}{0.65,0.16,0.16}
\definecolor {darksalmon}          {rgb}{0.91,0.59,0.48}
\definecolor {salmon}              {rgb}{0.98,0.50,0.45}
\definecolor {lightsalmon}         {rgb}{1.00,0.63,0.48}
\definecolor {orange}              {rgb}{1.00,0.65,0.00}
\definecolor {darkorange}          {rgb}{1.00,0.55,0.00}
\definecolor {coral}               {rgb}{1.00,0.50,0.31}
\definecolor {lightcoral}          {rgb}{0.94,0.50,0.50}
\definecolor {tomato}              {rgb}{1.00,0.39,0.28}
\definecolor {orangered}           {rgb}{1.00,0.27,0.00}
\definecolor {red}                 {rgb}{1.00,0.00,0.00}
\definecolor {hotpink}             {rgb}{1.00,0.41,0.71}
\definecolor {deeppink}            {rgb}{1.00,0.08,0.58}
\definecolor {pink}                {rgb}{1.00,0.75,0.80}
\definecolor {lightpink}           {rgb}{1.00,0.71,0.76}
\definecolor {palevioletred}       {rgb}{0.86,0.44,0.58}
\definecolor {maroon}              {rgb}{0.69,0.19,0.38}
\definecolor {mediumvioletred}     {rgb}{0.78,0.08,0.52}
\definecolor {violetred}           {rgb}{0.82,0.13,0.56}
\definecolor {magenta}             {rgb}{1.00,0.00,1.00}
\definecolor {violet}              {rgb}{0.93,0.51,0.93}
\definecolor {plum}                {rgb}{0.87,0.63,0.87}
\definecolor {orchid}              {rgb}{0.85,0.44,0.84}
\definecolor {mediumorchid}        {rgb}{0.73,0.33,0.83}
\definecolor {darkorchid}          {rgb}{0.60,0.20,0.80}
\definecolor {darkviolet}          {rgb}{0.58,0.00,0.83}
\definecolor {blueviolet}          {rgb}{0.54,0.17,0.89}
\definecolor {purple}              {rgb}{0.63,0.13,0.94}
\definecolor {mediumpurple}        {rgb}{0.58,0.44,0.86}
\definecolor {thistle}             {rgb}{0.85,0.75,0.85}
\definecolor {snow2}               {rgb}{0.93,0.91,0.91}
\definecolor {snow3}               {rgb}{0.80,0.79,0.79}
\definecolor {snow4}               {rgb}{0.55,0.54,0.54}
\definecolor {seashell2}           {rgb}{0.93,0.90,0.87}
\definecolor {seashell3}           {rgb}{0.80,0.77,0.75}
\definecolor {seashell4}           {rgb}{0.55,0.53,0.51}
\definecolor {antiquewhite1}       {rgb}{1.00,0.94,0.86}
\definecolor {antiquewhite2}       {rgb}{0.93,0.87,0.80}
\definecolor {antiquewhite3}       {rgb}{0.80,0.75,0.69}
\definecolor {antiquewhite4}       {rgb}{0.55,0.51,0.47}
\definecolor {bisque2}             {rgb}{0.93,0.84,0.72}
\definecolor {bisque3}             {rgb}{0.80,0.72,0.62}
\definecolor {bisque4}             {rgb}{0.55,0.49,0.42}
\definecolor {peachpuff2}          {rgb}{0.93,0.80,0.68}
\definecolor {peachpuff3}          {rgb}{0.80,0.69,0.58}
\definecolor {peachpuff4}          {rgb}{0.55,0.47,0.40}
\definecolor {navajowhite2}        {rgb}{0.93,0.81,0.63}
\definecolor {navajowhite3}        {rgb}{0.80,0.70,0.55}
\definecolor {navajowhite4}        {rgb}{0.55,0.47,0.37}
\definecolor {lemonchiffon2}       {rgb}{0.93,0.91,0.75}
\definecolor {lemonchiffon3}       {rgb}{0.80,0.79,0.65}
\definecolor {lemonchiffon4}       {rgb}{0.55,0.54,0.44}
\definecolor {cornsilk2}           {rgb}{0.93,0.91,0.80}
\definecolor {cornsilk3}           {rgb}{0.80,0.78,0.69}
\definecolor {cornsilk4}           {rgb}{0.55,0.53,0.47}
\definecolor {ivory2}              {rgb}{0.93,0.93,0.88}
\definecolor {ivory3}              {rgb}{0.80,0.80,0.76}
\definecolor {ivory4}              {rgb}{0.55,0.55,0.51}
\definecolor {honeydew2}           {rgb}{0.88,0.93,0.88}
\definecolor {honeydew3}           {rgb}{0.76,0.80,0.76}
\definecolor {honeydew4}           {rgb}{0.51,0.55,0.51}
\definecolor {lavenderblush2}      {rgb}{0.93,0.88,0.90}
\definecolor {lavenderblush3}      {rgb}{0.80,0.76,0.77}
\definecolor {lavenderblush4}      {rgb}{0.55,0.51,0.53}
\definecolor {mistyrose2}          {rgb}{0.93,0.84,0.82}
\definecolor {mistyrose3}          {rgb}{0.80,0.72,0.71}
\definecolor {mistyrose4}          {rgb}{0.55,0.49,0.48}
\definecolor {azure2}              {rgb}{0.88,0.93,0.93}
\definecolor {azure3}              {rgb}{0.76,0.80,0.80}
\definecolor {azure4}              {rgb}{0.51,0.55,0.55}
\definecolor {slateblue1}          {rgb}{0.51,0.44,1.00}
\definecolor {slateblue2}          {rgb}{0.48,0.40,0.93}
\definecolor {slateblue3}          {rgb}{0.41,0.35,0.80}
\definecolor {slateblue4}          {rgb}{0.28,0.24,0.55}
\definecolor {royalblue1}          {rgb}{0.28,0.46,1.00}
\definecolor {royalblue2}          {rgb}{0.26,0.43,0.93}
\definecolor {royalblue3}          {rgb}{0.23,0.37,0.80}
\definecolor {royalblue4}          {rgb}{0.15,0.25,0.55}
\definecolor {blue2}               {rgb}{0.00,0.00,0.93}
\definecolor {blue4}               {rgb}{0.00,0.00,0.55}
\definecolor {dodgerblue2}         {rgb}{0.11,0.53,0.93}
\definecolor {dodgerblue3}         {rgb}{0.09,0.45,0.80}
\definecolor {dodgerblue4}         {rgb}{0.06,0.31,0.55}
\definecolor {steelblue1}          {rgb}{0.39,0.72,1.00}
\definecolor {steelblue2}          {rgb}{0.36,0.67,0.93}
\definecolor {steelblue3}          {rgb}{0.31,0.58,0.80}
\definecolor {steelblue4}          {rgb}{0.21,0.39,0.55}
\definecolor {deepskyblue2}        {rgb}{0.00,0.70,0.93}
\definecolor {deepskyblue3}        {rgb}{0.00,0.60,0.80}
\definecolor {deepskyblue4}        {rgb}{0.00,0.41,0.55}
\definecolor {skyblue1}            {rgb}{0.53,0.81,1.00}
\definecolor {skyblue2}            {rgb}{0.49,0.75,0.93}
\definecolor {skyblue3}            {rgb}{0.42,0.65,0.80}
\definecolor {skyblue4}            {rgb}{0.29,0.44,0.55}
\definecolor {lightskyblue1}       {rgb}{0.69,0.89,1.00}
\definecolor {lightskyblue2}       {rgb}{0.64,0.83,0.93}
\definecolor {lightskyblue3}       {rgb}{0.55,0.71,0.80}
\definecolor {lightskyblue4}       {rgb}{0.38,0.48,0.55}
\definecolor {slategray1}          {rgb}{0.78,0.89,1.00}
\definecolor {slategray2}          {rgb}{0.73,0.83,0.93}
\definecolor {slategray3}          {rgb}{0.62,0.71,0.80}
\definecolor {slategray4}          {rgb}{0.42,0.48,0.55}
\definecolor {lightsteelblue1}     {rgb}{0.79,0.88,1.00}
\definecolor {lightsteelblue2}     {rgb}{0.74,0.82,0.93}
\definecolor {lightsteelblue3}     {rgb}{0.64,0.71,0.80}
\definecolor {lightsteelblue4}     {rgb}{0.43,0.48,0.55}
\definecolor {lightblue1}          {rgb}{0.75,0.94,1.00}
\definecolor {lightblue2}          {rgb}{0.70,0.87,0.93}
\definecolor {lightblue3}          {rgb}{0.60,0.75,0.80}
\definecolor {lightblue4}          {rgb}{0.41,0.51,0.55}
\definecolor {lightcyan2}          {rgb}{0.82,0.93,0.93}
\definecolor {lightcyan3}          {rgb}{0.71,0.80,0.80}
\definecolor {lightcyan4}          {rgb}{0.48,0.55,0.55}
\definecolor {paleturquoise1}      {rgb}{0.73,1.00,1.00}
\definecolor {paleturquoise2}      {rgb}{0.68,0.93,0.93}
\definecolor {paleturquoise3}      {rgb}{0.59,0.80,0.80}
\definecolor {paleturquoise4}      {rgb}{0.40,0.55,0.55}
\definecolor {cadetblue1}          {rgb}{0.60,0.96,1.00}
\definecolor {cadetblue2}          {rgb}{0.56,0.90,0.93}
\definecolor {cadetblue3}          {rgb}{0.48,0.77,0.80}
\definecolor {cadetblue4}          {rgb}{0.33,0.53,0.55}
\definecolor {turquoise1}          {rgb}{0.00,0.96,1.00}
\definecolor {turquoise2}          {rgb}{0.00,0.90,0.93}
\definecolor {turquoise3}          {rgb}{0.00,0.77,0.80}
\definecolor {turquoise4}          {rgb}{0.00,0.53,0.55}
\definecolor {cyan2}               {rgb}{0.00,0.93,0.93}
\definecolor {cyan3}               {rgb}{0.00,0.80,0.80}
\definecolor {cyan4}               {rgb}{0.00,0.55,0.55}
\definecolor {darkslategray1}      {rgb}{0.59,1.00,1.00}
\definecolor {darkslategray2}      {rgb}{0.55,0.93,0.93}
\definecolor {darkslategray3}      {rgb}{0.47,0.80,0.80}
\definecolor {darkslategray4}      {rgb}{0.32,0.55,0.55}
\definecolor {aquamarine2}         {rgb}{0.46,0.93,0.78}
\definecolor {aquamarine4}         {rgb}{0.27,0.55,0.45}
\definecolor {darkseagreen1}       {rgb}{0.76,1.00,0.76}
\definecolor {darkseagreen2}       {rgb}{0.71,0.93,0.71}
\definecolor {darkseagreen3}       {rgb}{0.61,0.80,0.61}
\definecolor {darkseagreen4}       {rgb}{0.41,0.55,0.41}
\definecolor {seagreen1}           {rgb}{0.33,1.00,0.62}
\definecolor {seagreen2}           {rgb}{0.31,0.93,0.58}
\definecolor {seagreen3}           {rgb}{0.26,0.80,0.50}
\definecolor {palegreen1}          {rgb}{0.60,1.00,0.60}
\definecolor {palegreen2}          {rgb}{0.56,0.93,0.56}
\definecolor {palegreen3}          {rgb}{0.49,0.80,0.49}
\definecolor {palegreen4}          {rgb}{0.33,0.55,0.33}
\definecolor {springgreen2}        {rgb}{0.00,0.93,0.46}
\definecolor {springgreen3}        {rgb}{0.00,0.80,0.40}
\definecolor {springgreen4}        {rgb}{0.00,0.55,0.27}
\definecolor {green2}              {rgb}{0.00,0.93,0.00}
\definecolor {green3}              {rgb}{0.00,0.80,0.00}
\definecolor {green4}              {rgb}{0.00,0.55,0.00}
\definecolor {chartreuse2}         {rgb}{0.46,0.93,0.00}
\definecolor {chartreuse3}         {rgb}{0.40,0.80,0.00}
\definecolor {chartreuse4}         {rgb}{0.27,0.55,0.00}
\definecolor {olivedrab1}          {rgb}{0.75,1.00,0.24}
\definecolor {olivedrab2}          {rgb}{0.70,0.93,0.23}
\definecolor {olivedrab4}          {rgb}{0.41,0.55,0.13}
\definecolor {darkolivegreen1}     {rgb}{0.79,1.00,0.44}
\definecolor {darkolivegreen2}     {rgb}{0.74,0.93,0.41}
\definecolor {darkolivegreen3}     {rgb}{0.64,0.80,0.35}
\definecolor {darkolivegreen4}     {rgb}{0.43,0.55,0.24}
\definecolor {khaki1}              {rgb}{1.00,0.96,0.56}
\definecolor {khaki2}              {rgb}{0.93,0.90,0.52}
\definecolor {khaki3}              {rgb}{0.80,0.78,0.45}
\definecolor {khaki4}              {rgb}{0.55,0.53,0.31}
\definecolor {lightgoldenrod1}     {rgb}{1.00,0.93,0.55}
\definecolor {lightgoldenrod2}     {rgb}{0.93,0.86,0.51}
\definecolor {lightgoldenrod3}     {rgb}{0.80,0.75,0.44}
\definecolor {lightgoldenrod4}     {rgb}{0.55,0.51,0.30}
\definecolor {lightyellow2}        {rgb}{0.93,0.93,0.82}
\definecolor {lightyellow3}        {rgb}{0.80,0.80,0.71}
\definecolor {lightyellow4}        {rgb}{0.55,0.55,0.48}
\definecolor {yellow2}             {rgb}{0.93,0.93,0.00}
\definecolor {yellow3}             {rgb}{0.80,0.80,0.00}
\definecolor {yellow4}             {rgb}{0.55,0.55,0.00}
\definecolor {gold2}               {rgb}{0.93,0.79,0.00}
\definecolor {gold3}               {rgb}{0.80,0.68,0.00}
\definecolor {gold4}               {rgb}{0.55,0.46,0.00}
\definecolor {goldenrod1}          {rgb}{1.00,0.76,0.15}
\definecolor {goldenrod2}          {rgb}{0.93,0.71,0.13}
\definecolor {goldenrod3}          {rgb}{0.80,0.61,0.11}
\definecolor {goldenrod4}          {rgb}{0.55,0.41,0.08}
\definecolor {darkgoldenrod1}      {rgb}{1.00,0.73,0.06}
\definecolor {darkgoldenrod2}      {rgb}{0.93,0.68,0.05}
\definecolor {darkgoldenrod3}      {rgb}{0.80,0.58,0.05}
\definecolor {darkgoldenrod4}      {rgb}{0.55,0.40,0.03}
\definecolor {rosybrown1}          {rgb}{1.00,0.76,0.76}
\definecolor {rosybrown2}          {rgb}{0.93,0.71,0.71}
\definecolor {rosybrown3}          {rgb}{0.80,0.61,0.61}
\definecolor {rosybrown4}          {rgb}{0.55,0.41,0.41}
\definecolor {indianred1}          {rgb}{1.00,0.42,0.42}
\definecolor {indianred2}          {rgb}{0.93,0.39,0.39}
\definecolor {indianred3}          {rgb}{0.80,0.33,0.33}
\definecolor {indianred4}          {rgb}{0.55,0.23,0.23}
\definecolor {sienna1}             {rgb}{1.00,0.51,0.28}
\definecolor {sienna2}             {rgb}{0.93,0.47,0.26}
\definecolor {sienna3}             {rgb}{0.80,0.41,0.22}
\definecolor {sienna4}             {rgb}{0.55,0.28,0.15}
\definecolor {burlywood1}          {rgb}{1.00,0.83,0.61}
\definecolor {burlywood2}          {rgb}{0.93,0.77,0.57}
\definecolor {burlywood3}          {rgb}{0.80,0.67,0.49}
\definecolor {burlywood4}          {rgb}{0.55,0.45,0.33}
\definecolor {wheat1}              {rgb}{1.00,0.91,0.73}
\definecolor {wheat2}              {rgb}{0.93,0.85,0.68}
\definecolor {wheat3}              {rgb}{0.80,0.73,0.59}
\definecolor {wheat4}              {rgb}{0.55,0.49,0.40}
\definecolor {tan1}                {rgb}{1.00,0.65,0.31}
\definecolor {tan2}                {rgb}{0.93,0.60,0.29}
\definecolor {tan4}                {rgb}{0.55,0.35,0.17}
\definecolor {chocolate1}          {rgb}{1.00,0.50,0.14}
\definecolor {chocolate2}          {rgb}{0.93,0.46,0.13}
\definecolor {chocolate3}          {rgb}{0.80,0.40,0.11}
\definecolor {firebrick1}          {rgb}{1.00,0.19,0.19}
\definecolor {firebrick2}          {rgb}{0.93,0.17,0.17}
\definecolor {firebrick3}          {rgb}{0.80,0.15,0.15}
\definecolor {firebrick4}          {rgb}{0.55,0.10,0.10}
\definecolor {brown1}              {rgb}{1.00,0.25,0.25}
\definecolor {brown2}              {rgb}{0.93,0.23,0.23}
\definecolor {brown3}              {rgb}{0.80,0.20,0.20}
\definecolor {brown4}              {rgb}{0.55,0.14,0.14}
\definecolor {salmon1}             {rgb}{1.00,0.55,0.41}
\definecolor {salmon2}             {rgb}{0.93,0.51,0.38}
\definecolor {salmon3}             {rgb}{0.80,0.44,0.33}
\definecolor {salmon4}             {rgb}{0.55,0.30,0.22}
\definecolor {lightsalmon2}        {rgb}{0.93,0.58,0.45}
\definecolor {lightsalmon3}        {rgb}{0.80,0.51,0.38}
\definecolor {lightsalmon4}        {rgb}{0.55,0.34,0.26}
\definecolor {orange2}             {rgb}{0.93,0.60,0.00}
\definecolor {orange3}             {rgb}{0.80,0.52,0.00}
\definecolor {orange4}             {rgb}{0.55,0.35,0.00}
\definecolor {darkorange1}         {rgb}{1.00,0.50,0.00}
\definecolor {darkorange2}         {rgb}{0.93,0.46,0.00}
\definecolor {darkorange3}         {rgb}{0.80,0.40,0.00}
\definecolor {darkorange4}         {rgb}{0.55,0.27,0.00}
\definecolor {coral1}              {rgb}{1.00,0.45,0.34}
\definecolor {coral2}              {rgb}{0.93,0.42,0.31}
\definecolor {coral3}              {rgb}{0.80,0.36,0.27}
\definecolor {coral4}              {rgb}{0.55,0.24,0.18}
\definecolor {tomato2}             {rgb}{0.93,0.36,0.26}
\definecolor {tomato3}             {rgb}{0.80,0.31,0.22}
\definecolor {tomato4}             {rgb}{0.55,0.21,0.15}
\definecolor {orangered2}          {rgb}{0.93,0.25,0.00}
\definecolor {orangered3}          {rgb}{0.80,0.22,0.00}
\definecolor {orangered4}          {rgb}{0.55,0.15,0.00}
\definecolor {red2}                {rgb}{0.93,0.00,0.00}
\definecolor {red3}                {rgb}{0.80,0.00,0.00}
\definecolor {red4}                {rgb}{0.55,0.00,0.00}
\definecolor {deeppink2}           {rgb}{0.93,0.07,0.54}
\definecolor {deeppink3}           {rgb}{0.80,0.06,0.46}
\definecolor {deeppink4}           {rgb}{0.55,0.04,0.31}
\definecolor {hotpink1}            {rgb}{1.00,0.43,0.71}
\definecolor {hotpink2}            {rgb}{0.93,0.42,0.65}
\definecolor {hotpink3}            {rgb}{0.80,0.38,0.56}
\definecolor {hotpink4}            {rgb}{0.55,0.23,0.38}
\definecolor {pink1}               {rgb}{1.00,0.71,0.77}
\definecolor {pink2}               {rgb}{0.93,0.66,0.72}
\definecolor {pink3}               {rgb}{0.80,0.57,0.62}
\definecolor {pink4}               {rgb}{0.55,0.39,0.42}
\definecolor {lightpink1}          {rgb}{1.00,0.68,0.73}
\definecolor {lightpink2}          {rgb}{0.93,0.64,0.68}
\definecolor {lightpink3}          {rgb}{0.80,0.55,0.58}
\definecolor {lightpink4}          {rgb}{0.55,0.37,0.40}
\definecolor {palevioletred1}      {rgb}{1.00,0.51,0.67}
\definecolor {palevioletred2}      {rgb}{0.93,0.47,0.62}
\definecolor {palevioletred3}      {rgb}{0.80,0.41,0.54}
\definecolor {palevioletred4}      {rgb}{0.55,0.28,0.36}
\definecolor {maroon1}             {rgb}{1.00,0.20,0.70}
\definecolor {maroon2}             {rgb}{0.93,0.19,0.65}
\definecolor {maroon3}             {rgb}{0.80,0.16,0.56}
\definecolor {maroon4}             {rgb}{0.55,0.11,0.38}
\definecolor {violetred1}          {rgb}{1.00,0.24,0.59}
\definecolor {violetred2}          {rgb}{0.93,0.23,0.55}
\definecolor {violetred3}          {rgb}{0.80,0.20,0.47}
\definecolor {violetred4}          {rgb}{0.55,0.13,0.32}
\definecolor {magenta2}            {rgb}{0.93,0.00,0.93}
\definecolor {magenta3}            {rgb}{0.80,0.00,0.80}
\definecolor {magenta4}            {rgb}{0.55,0.00,0.55}
\definecolor {orchid1}             {rgb}{1.00,0.51,0.98}
\definecolor {orchid2}             {rgb}{0.93,0.48,0.91}
\definecolor {orchid3}             {rgb}{0.80,0.41,0.79}
\definecolor {orchid4}             {rgb}{0.55,0.28,0.54}
\definecolor {plum1}               {rgb}{1.00,0.73,1.00}
\definecolor {plum2}               {rgb}{0.93,0.68,0.93}
\definecolor {plum3}               {rgb}{0.80,0.59,0.80}
\definecolor {plum4}               {rgb}{0.55,0.40,0.55}
\definecolor {mediumorchid1}       {rgb}{0.88,0.40,1.00}
\definecolor {mediumorchid2}       {rgb}{0.82,0.37,0.93}
\definecolor {mediumorchid3}       {rgb}{0.71,0.32,0.80}
\definecolor {mediumorchid4}       {rgb}{0.48,0.22,0.55}
\definecolor {darkorchid1}         {rgb}{0.75,0.24,1.00}
\definecolor {darkorchid2}         {rgb}{0.70,0.23,0.93}
\definecolor {darkorchid3}         {rgb}{0.60,0.20,0.80}
\definecolor {darkorchid4}         {rgb}{0.41,0.13,0.55}
\definecolor {purple1}             {rgb}{0.61,0.19,1.00}
\definecolor {purple2}             {rgb}{0.57,0.17,0.93}
\definecolor {purple3}             {rgb}{0.49,0.15,0.80}
\definecolor {purple4}             {rgb}{0.33,0.10,0.55}
\definecolor {mediumpurple1}       {rgb}{0.67,0.51,1.00}
\definecolor {mediumpurple2}       {rgb}{0.62,0.47,0.93}
\definecolor {mediumpurple3}       {rgb}{0.54,0.41,0.80}
\definecolor {mediumpurple4}       {rgb}{0.36,0.28,0.55}
\definecolor {thistle1}            {rgb}{1.00,0.88,1.00}
\definecolor {thistle2}            {rgb}{0.93,0.82,0.93}
\definecolor {thistle3}            {rgb}{0.80,0.71,0.80}
\definecolor {thistle4}            {rgb}{0.55,0.48,0.55}
\definecolor {gray1}               {rgb}{0.01,0.01,0.01}
\definecolor {gray2}               {rgb}{0.02,0.02,0.02}
\definecolor {gray3}               {rgb}{0.03,0.03,0.03}
\definecolor {gray4}               {rgb}{0.04,0.04,0.04}
\definecolor {gray5}               {rgb}{0.05,0.05,0.05}
\definecolor {gray6}               {rgb}{0.06,0.06,0.06}
\definecolor {gray7}               {rgb}{0.07,0.07,0.07}
\definecolor {gray8}               {rgb}{0.08,0.08,0.08}
\definecolor {gray9}               {rgb}{0.09,0.09,0.09}
\definecolor {gray10}              {rgb}{0.10,0.10,0.10}
\definecolor {gray11}              {rgb}{0.11,0.11,0.11}
\definecolor {gray12}              {rgb}{0.12,0.12,0.12}
\definecolor {gray13}              {rgb}{0.13,0.13,0.13}
\definecolor {gray14}              {rgb}{0.14,0.14,0.14}
\definecolor {gray15}              {rgb}{0.15,0.15,0.15}
\definecolor {gray16}              {rgb}{0.16,0.16,0.16}
\definecolor {gray17}              {rgb}{0.17,0.17,0.17}
\definecolor {gray18}              {rgb}{0.18,0.18,0.18}
\definecolor {gray19}              {rgb}{0.19,0.19,0.19}
\definecolor {gray20}              {rgb}{0.20,0.20,0.20}
\definecolor {gray21}              {rgb}{0.21,0.21,0.21}
\definecolor {gray22}              {rgb}{0.22,0.22,0.22}
\definecolor {gray23}              {rgb}{0.23,0.23,0.23}
\definecolor {gray24}              {rgb}{0.24,0.24,0.24}
\definecolor {gray25}              {rgb}{0.25,0.25,0.25}
\definecolor {gray26}              {rgb}{0.26,0.26,0.26}
\definecolor {gray27}              {rgb}{0.27,0.27,0.27}
\definecolor {gray28}              {rgb}{0.28,0.28,0.28}
\definecolor {gray29}              {rgb}{0.29,0.29,0.29}
\definecolor {gray30}              {rgb}{0.30,0.30,0.30}
\definecolor {gray31}              {rgb}{0.31,0.31,0.31}
\definecolor {gray32}              {rgb}{0.32,0.32,0.32}
\definecolor {gray33}              {rgb}{0.33,0.33,0.33}
\definecolor {gray34}              {rgb}{0.34,0.34,0.34}
\definecolor {gray35}              {rgb}{0.35,0.35,0.35}
\definecolor {gray36}              {rgb}{0.36,0.36,0.36}
\definecolor {gray37}              {rgb}{0.37,0.37,0.37}
\definecolor {gray38}              {rgb}{0.38,0.38,0.38}
\definecolor {gray39}              {rgb}{0.39,0.39,0.39}
\definecolor {gray40}              {rgb}{0.40,0.40,0.40}
\definecolor {gray42}              {rgb}{0.42,0.42,0.42}
\definecolor {gray43}              {rgb}{0.43,0.43,0.43}
\definecolor {gray44}              {rgb}{0.44,0.44,0.44}
\definecolor {gray45}              {rgb}{0.45,0.45,0.45}
\definecolor {gray46}              {rgb}{0.46,0.46,0.46}
\definecolor {gray47}              {rgb}{0.47,0.47,0.47}
\definecolor {gray48}              {rgb}{0.48,0.48,0.48}
\definecolor {gray49}              {rgb}{0.49,0.49,0.49}
\definecolor {gray50}              {rgb}{0.50,0.50,0.50}
\definecolor {gray51}              {rgb}{0.51,0.51,0.51}
\definecolor {gray52}              {rgb}{0.52,0.52,0.52}
\definecolor {gray53}              {rgb}{0.53,0.53,0.53}
\definecolor {gray54}              {rgb}{0.54,0.54,0.54}
\definecolor {gray55}              {rgb}{0.55,0.55,0.55}
\definecolor {gray56}              {rgb}{0.56,0.56,0.56}
\definecolor {gray57}              {rgb}{0.57,0.57,0.57}
\definecolor {gray58}              {rgb}{0.58,0.58,0.58}
\definecolor {gray59}              {rgb}{0.59,0.59,0.59}
\definecolor {gray60}              {rgb}{0.60,0.60,0.60}
\definecolor {gray61}              {rgb}{0.61,0.61,0.61}
\definecolor {gray62}              {rgb}{0.62,0.62,0.62}
\definecolor {gray63}              {rgb}{0.63,0.63,0.63}
\definecolor {gray64}              {rgb}{0.64,0.64,0.64}
\definecolor {gray65}              {rgb}{0.65,0.65,0.65}
\definecolor {gray66}              {rgb}{0.66,0.66,0.66}
\definecolor {gray67}              {rgb}{0.67,0.67,0.67}
\definecolor {gray68}              {rgb}{0.68,0.68,0.68}
\definecolor {gray69}              {rgb}{0.69,0.69,0.69}
\definecolor {gray70}              {rgb}{0.70,0.70,0.70}
\definecolor {gray71}              {rgb}{0.71,0.71,0.71}
\definecolor {gray72}              {rgb}{0.72,0.72,0.72}
\definecolor {gray73}              {rgb}{0.73,0.73,0.73}
\definecolor {gray74}              {rgb}{0.74,0.74,0.74}
\definecolor {gray75}              {rgb}{0.75,0.75,0.75}
\definecolor {gray76}              {rgb}{0.76,0.76,0.76}
\definecolor {gray77}              {rgb}{0.77,0.77,0.77}
\definecolor {gray78}              {rgb}{0.78,0.78,0.78}
\definecolor {gray79}              {rgb}{0.79,0.79,0.79}
\definecolor {gray80}              {rgb}{0.80,0.80,0.80}
\definecolor {gray81}              {rgb}{0.81,0.81,0.81}
\definecolor {gray82}              {rgb}{0.82,0.82,0.82}
\definecolor {gray83}              {rgb}{0.83,0.83,0.83}
\definecolor {gray84}              {rgb}{0.84,0.84,0.84}
\definecolor {gray85}              {rgb}{0.85,0.85,0.85}
\definecolor {gray86}              {rgb}{0.86,0.86,0.86}
\definecolor {gray87}              {rgb}{0.87,0.87,0.87}
\definecolor {gray88}              {rgb}{0.88,0.88,0.88}
\definecolor {gray89}              {rgb}{0.89,0.89,0.89}
\definecolor {gray90}              {rgb}{0.90,0.90,0.90}
\definecolor {gray91}              {rgb}{0.91,0.91,0.91}
\definecolor {gray92}              {rgb}{0.92,0.92,0.92}
\definecolor {gray93}              {rgb}{0.93,0.93,0.93}
\definecolor {gray94}              {rgb}{0.94,0.94,0.94}
\definecolor {gray95}              {rgb}{0.95,0.95,0.95}
\definecolor {gray97}              {rgb}{0.97,0.97,0.97}
\definecolor {gray98}              {rgb}{0.98,0.98,0.98}
\definecolor {gray99}              {rgb}{0.99,0.99,0.99}
\definecolor {darkgrey}            {rgb}{0.66,0.66,0.66}


==> arxiv-version/rs_macros_colors.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% This file is an hard link, whose source is in   
%%%%%%% cipeciop.science.unitn.it:/home/rseba/latex/macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% cambiate in modo da gestire le animazioni
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\darkblue}[1]{\textcolor{blue}{#1}}
\newcommand{\lightblue}[1]{\textcolor{lightblue4}{#1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\green}[1]{\textcolor{darkgreen}{#1}}
\newcommand{\lightgreen}[1]{\textcolor{palegreen1}{#1}}
\newcommand{\violet}[1]{\textcolor{violet}{#1}}
\newcommand{\darkviolet}[1]{\textcolor{darkviolet}{#1}}
\newcommand{\darkgrey}[1]{\textcolor{darkgrey}{#1}}
\newcommand{\palegrey}[1]{\textcolor{lightgrey}{#1}}
\newcommand{\gray}[1]{\textcolor{gray}{#1}}
\newcommand{\white}[1]{\textcolor{white}{#1}}
\newcommand{\black}[1]{\textcolor{black}{#1}}
\newcommand{\orange}[1]{\textcolor{orange}{#1}}
\newcommand{\darkorange}[1]{\textcolor{darkorange3}{#1}}

% \newcommand<>{\blue}{\color#1{blue}}
% \newcommand<>{\darkblue}{\color#1{blue}}
% \newcommand<>{\lightblue}{\color#1{lightblue4}}
% \newcommand<>{\red}{\color#1{red}}
% \newcommand<>{\green}{\color#1{darkgreen}}
% \newcommand<>{\lightgreen}{\color#1{palegreen1}}
% \newcommand<>{\violet}{\color#1{violet}}
% \newcommand<>{\darkviolet}{\color#1{darkviolet}}
% \newcommand<>{\darkgrey}{\color#1{darkgrey}}
% \newcommand<>{\palegrey}{\color#1{lightgrey}}
% \newcommand<>{\gray}{\color#1{gray}}
% \newcommand<>{\white}{\color#1{white}}
% \newcommand<>{\black}{\color#1{black}}
% \newcommand<>{\orange}{\color#1{orange}}
% \newcommand<>{\darkorange}{\color#1{darkorange3}}


==> arxiv-version/rs_macros_dl.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% This file is an hard link, whose source is in   
%%%%%%% cipeciop.science.unitn.it:/home/rseba/latex/macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\en}[2]{{#1}e{#2}}
\newcommand{\den}[4]{\en{#1}{#2}/\en{#3}{#4}}

\newcommand{\mc}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\msf}[1]{\ensuremath{\mathsf{#1}}}

\newcommand{\snomed}{\textsc{Snomed-CT}\xspace}
\newcommand{\geneonto}{\textsc{GeneOntology}\xspace}
\newcommand{\nci}{\textsc{NCI}\xspace}
\newcommand{\galen}{\textsc{Galen}\xspace}

\newcommand{\shsnomed}{\textsc{Snomed09}\xspace} 
\newcommand{\shnci}{\textsc{NCI}\xspace} 
\newcommand{\shgalen}{\textsc{notGalen}\xspace}
\newcommand{\shfullgalen}{{\textsc{fullGalen}}\xspace}
\newcommand{\shgeneontology}{{\textsc{GeneOnt.}}\xspace}

\newcommand{\conj}{\sqcap}
\newcommand{\disj}{\sqcup}
\newcommand{\exr}[2]{{\exists}#1.#2}

\newcommand{\subs}{\sqsubseteq}
\newcommand{\sups}{\sqsupseteq}
\newcommand{\norm}{\triangleq}
\newcommand{\comp}{\circ}

\newcommand{\topt}{\ensuremath{\top}\xspace}
\newcommand{\bott}{\ensuremath{\bot}\xspace}
\newcommand{\conjt}[2]{\ensuremath{#1 \sqcap #2}\xspace}
\newcommand{\disjt}[2]{\ensuremath{#1 \sqcup #2}\xspace}
\newcommand{\exrt}[2]{\ensuremath{{\exists}#1.#2}\xspace}
\newcommand{\equivt}[2]{\ensuremath{#1 \equiv #2}\xspace}
\newcommand{\subst}[2]{\ensuremath{#1 \sqsubseteq #2}\xspace}
\newcommand{\supst}[2]{\ensuremath{#1 \sqsupseteq #2}\xspace}
%\newcommand{\eqdef}{\stackrel{def}{=}}
%\newcommand{\defas}{\ensuremath{\stackrel{\text{\tiny def}}{=}}\xspace}
 
\newcommand{\pr}[1]{\ensuremath{p_{#1}}\xspace}
\newcommand{\prc}[1]{\ensuremath{p_{[#1]}}\xspace}
\newcommand{\sel}[1]{\ensuremath{s_{#1}}\xspace}
\newcommand{\selc}[1]{\ensuremath{s_{[#1]}}\xspace}

\newcommand{\goal}{\ensuremath{C_i\subs_\T D_i}\xspace}
\newcommand{\goalsure}{\ensuremath{C_i~\subs_\T~D_i}\xspace}
\newcommand{\tgoal}[1]{\ensuremath{C_i\subs_{#1} D_i}\xspace}
\newcommand{\igoal}[1]{\ensuremath{{C_{#1} \subs_\T D_{#1}}}\xspace}
\newcommand{\sgoal}{\ensuremath{\selc{\goal}}\xspace}
\newcommand{\isgoal}[1]{\ensuremath{\selc{\igoal{#1}}}\xspace}
\newcommand{\nsgoal}{\ensuremath{\neg\selc{C_i\subs_\T D_i}}\xspace}

\newcommand{\assumptiongoal}{\ensuremath{\{\neg\prc{D_i},\prc{C_i}\}}\xspace}
\newcommand{\assumptionsgoal}{\ensuremath{\{\neg\sgoal\}}\xspace}

\newcommand{\aenc}[1]{\ensuremath{\elp2sat(#1)}\xspace}
\newcommand{\wffsubs}{\ensuremath{\phi_{\T{}}}\xspace}
\newcommand{\wffsubsnotrans}{\ensuremath{\phi_{\T{}}^{notrans}}\xspace}
\newcommand{\wffmina}{\ensuremath{\wffsubs^{one}}\xspace}
\newcommand{\wffminarule}{\ensuremath{\phi_{\T(po)}^{one}}\xspace}
\newcommand{\wffminaT}[1]{\ensuremath{\phi_{#1}^{one}}\xspace}
\newcommand{\wffminaTrule}[1]{\ensuremath{\phi_{#1}^{one}}\xspace}
\newcommand{\wffallmina}{\ensuremath{\wffsubs^{all}}\xspace}
\newcommand{\wffallminarule}{\ensuremath{\phi_{\T{}(po)}^{all}}\xspace}
\newcommand{\wffallminaT}[1]{\ensuremath{\phi_{#1}^{all}}\xspace}
\newcommand{\wffallminaTrule}[1]{\ensuremath{\phi_{#1 (po)}^{all}}\xspace}
\newcommand{\wffallminaO}{\ensuremath{\phi_{\T^*}^{all}}\xspace}
\newcommand{\wffallminaruleO}{\ensuremath{\phi_{\T^*(po)}^{all}}\xspace}

\newcommand{\pinpointingwff}{\ensuremath{\Phi^{\goal}}\xspace}
\newcommand{\pinpointingwffall}{\ensuremath{\Phi^{all}}\xspace}

\newcommand{\hatT}{\ensuremath{\hat{\T}}\xspace}
\newcommand{\Tp}{\ensuremath{\ensuremath{\mathcal{T'}}\xspace}}

\newcommand{\elsat}{{\elp{}\textsc{SAT}}\xspace}















\newcommand{\el}{\ensuremath{\mathcal{EL}}\xspace}
\newcommand{\elh}{\ensuremath{\mathcal{ELH}}\xspace}
\newcommand{\elp}{\ensuremath{\mathcal{EL^{+}}}\xspace}
\newcommand{\elpp}{\ensuremath{\mathcal{EL^{++}}}\xspace}
\newcommand{\eloh}{\ensuremath{\mathcal{ELOH}}\xspace}
\newcommand{\eqdef}{\stackrel{def}{=}}


% \newcommand{\sel}[1]{\ensuremath{s_{#1}}\xspace}
% \newcommand{\selc}[1]{\ensuremath{s_{[#1]}}\xspace}
% \newcommand{\sgoal}{\ensuremath{\selc{\goal}}\xspace}
% \newcommand{\isgoal}[1]{\ensuremath{\selc{\igoal{#1}}}\xspace}
% \newcommand{\nsgoal}{\ensuremath{\neg\selc{C_i\subs_\T D_i}}\xspace}
% \newcommand{\aenc}[1]{\ensuremath{\elp2sat(#1)}\xspace}
% \newcommand{\elsat}{{\elp{}\textsc{SAT}}\xspace}






 


==> arxiv-version/rs_macros_general.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% This file is an hard link, whose source is in   
%%%%%%% cipeciop.science.unitn.it:/home/rseba/latex/macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% general-use macros 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{rgb}

%%%%%%%%%%%%%% REDEFINITION OF COMMENTS IN "algorithmic" 
%\renewcommand{\algorithmiccomment}[1]{\ \ \ \ \ // #1}


%%% CONTROL MACROS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\RSHIGHLIGHT}[1]{\textcolor{blue}{{{#1}}}}


%\renewcommand{\emph}[1]{\darkorange{{\em #1}}}
%\newcommand{\new}[1]{\darkorange{#1}}
\newcommand{\new}[1]{{\blue #1}\/}
\newcommand{\ex}[1]{{\green #1}\/} 
%\newcommand{\ex}[1]{{#1}} 

\newcommand{\resp}[1]{[resp. #1]}
\newcommand{\done}{\textcolor{darkgreen}{\checkmark}}


%\newcommand{\TODO}[1]{{\bf \textcolor{blue}{{\fbox{TODO:} #1}}}}
\newcommand{\TODO}[1]{{}}
\newcommand{\ACTODO}[1]{{\bf \textcolor{red}{{\fbox{AC TODO:} #1}}}}
\newcommand{\RS}[1]{\textcolor{blue}{#1}}
\newcommand{\ignore}[1]{}
%\newcommand{\todo}[1] {\noindent \textcolor{blue}{\fbox{{\bf TO DO:}} #1 }}
%\newcommand{\todo}[1] {}
\newcommand{\RSCHANGE}[1]{\textcolor{darkgreen}{#1}}
\renewcommand{\RS}[1]{\textcolor{darkgreen}{#1}}
\newcommand{\PT}[1]{\textcolor{darkviolet}{#1}}
\newcommand{\RSTODO}[1]{{\bf \textcolor{darkgreen}{{\fbox{RS TODO:} #1}}}}
\renewcommand{\RSTODO}[1]{}
%\renewcommand{\RSCHANGE}[1]{#1}
\newcommand{\nota}[1] {\noindent \fbox{{\bf NOTA:}} #1 }
\newcommand{\marg}[1]{\marginpar{\ \\{\em #1\/}}}
\renewcommand{\marg}[1]{\marginpar{\ \\\textcolor{blue}{\ {\sf #1\/}}}}
%\renewcommand{\marg}[1]{}

\newenvironment{rschange}{\color{darkgreen}}{\normalcolor}
\newenvironment{rs}{\color{darkgreen}}{\normalcolor}
\newenvironment{pt}{\color{darkviolet}}{\normalcolor}

\newcommand{\RSNOTE}[1]{\marginpar{\textcolor{darkgreen}{\textbf{RS: }
      {\footnotesize #1}}}}
\renewcommand{\RSNOTE}[1]{\textcolor{darkgreen}{{\bf RS: #1}}}




%%% FOR SHORTER VERSION
 \newcommand{\ignoreinshort}[1]{}
 \newcommand{\ignoreinlong}[1]{{#1}}
 % \renewcommand{\ignoreinshort}[1]{\textcolor{blue}{#1}}
 % \renewcommand{\ignoreinlong}[1]{}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% FREQUENTLY-USED ENVIRONMENTS (from mrg/environments.tex)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\makenewenumerate#1#2{%
\newcounter{cnt#1}
\newenvironment{#1}%
{\begin{list}{\makebox[0pt][r]{#2}}%
{\setlength{\itemsep}{0pt}% 
 \setlength{\parsep}{.2em}%
 \setlength{\leftmargin}{1.5em}%
 \setlength{\labelwidth}{.4em}%
 \usecounter{cnt#1}}}
{\end{list}}}

\makenewenumerate{myenumerate}{\arabic{cntmyenumerate}.}

\makenewenumerate{renumerate}{\rm(\roman{cntrenumerate})}
\makenewenumerate{renumerateprime}{\rm(\roman{cntrenumerateprime}$'$)}
\makenewenumerate{renumeratesecond}{\rm(\roman{cntrenumeratesecond}$''$)}

\makenewenumerate{aenumerate}{({\it\alph{cntaenumerate}})}
\makenewenumerate{aenumerateprime}{({\it\alph{cntaenumerateprime}$'$})}
\makenewenumerate{aenumeratesecond}{({\it\alph{cntaenumeratesecond}$''$})}

\def\newplaintheorem#1#2{%
\newtheorem{#1plain}{#2}[section]%
\newenvironment{#1}{\begin{#1plain}\rm }{\end{#1plain}}}

% \newtheorem{definition}{Definition}[section]
% \newtheorem{intfact}{Intuitive Fact}[section]
\newtheorem{Property}{Property}%[section]
\newtheorem{Proposition}{Proposition}[section]
%\newtheorem{conjecture}{Conjecture}[section]
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{corollary}{Corollary}[section]
%\newtheorem{lemma}{Lemma}[section]
\newplaintheorem{notation}{Notation}
% \newplaintheorem{remark}{Remark}
% \newplaintheorem{example}{Example}
\newplaintheorem{cexample}{Counter-Example}
\newtheorem{strategy}{Strategy}
%\newenvironment{proof}{{\bf Proof }}{\mbox{\hspace{0cm}}\hfill Q.E.D.} 

%%% TRICK FOR SHORTENING
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\fakesubsubsection}[1]{\smallskip\noindent {\bf #1.}}


%%% FREQUENTLY-USED MACROS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\sref}[1]{\S{}\ref{#1}}
\newcommand{\noi}{\noindent}


%%% FREQUENTLY-USED logic macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\pair}[2]{\ensuremath{\langle{#1},{#2}\rangle}\xspace}
\newcommand{\triple}[3]{\ensuremath{\langle{#1},{#2},{#3}\rangle}\xspace}
\newcommand{\tuple}[1]{\ensuremath{\langle{#1}\rangle}\xspace}
\newcommand{\set}[1]{\ensuremath{\{{#1}\}}\xspace}
\newcommand{\imp}{\ensuremath{\rightarrow}\xspace}
\newcommand{\limp}{\ensuremath{\leftarrow}\xspace}
\renewcommand{\iff}{\ensuremath{\leftrightarrow}\xspace}
\newcommand{\defas}{\ensuremath{\stackrel{\text{\tiny def}}{=}}\xspace}
\newcommand{\thus}{\ensuremath{\Longrightarrow}\xspace}

\newcommand{\pos}{\phantom{\neg}}



%%% FREQUENTLY-USED symbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% CALYGRAPHIC LETTERS
\newcommand\cala{\ensuremath{\mathcal{A}}\xspace}
\newcommand\calb{\ensuremath{\mathcal{B}}\xspace}
\newcommand\calc{\ensuremath{\mathcal{C}}\xspace}
\newcommand\cald{\ensuremath{\mathcal{D}}\xspace}
\newcommand\cale{\ensuremath{\mathcal{E}}\xspace}
\newcommand\calf{\ensuremath{\mathcal{F}}\xspace}
\newcommand\calg{\ensuremath{\mathcal{G}}\xspace}
\newcommand\calh{\ensuremath{\mathcal{H}}\xspace}
\newcommand\cali{\ensuremath{\mathcal{I}}\xspace}
\newcommand\calj{\ensuremath{\mathcal{J}}\xspace}
\newcommand\calk{\ensuremath{\mathcal{K}}\xspace}
\newcommand\call{\ensuremath{\mathcal{L}}\xspace}
\newcommand\calm{\ensuremath{\mathcal{M}}\xspace}
\newcommand\caln{\ensuremath{\mathcal{N}}\xspace}
\newcommand\calo{\ensuremath{\mathcal{O}}\xspace}
\newcommand\calp{\ensuremath{\mathcal{P}}\xspace}
\newcommand\calq{\ensuremath{\mathcal{Q}}\xspace}
\newcommand\calr{\ensuremath{\mathcal{R}}\xspace}
\newcommand\cals{\ensuremath{\mathcal{S}}\xspace}
\newcommand\calt{\ensuremath{\mathcal{T}}\xspace}
\newcommand\calu{\ensuremath{\mathcal{U}}\xspace}
\newcommand\calv{\ensuremath{\mathcal{V}}\xspace}
\newcommand\calw{\ensuremath{\mathcal{W}}\xspace}
\newcommand\calx{\ensuremath{\mathcal{X}}\xspace}
\newcommand\caly{\ensuremath{\mathcal{Y}}\xspace}
\newcommand\calz{\ensuremath{\mathcal{Z}}\xspace}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% macros for handling modification due to reviems
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\rone}{\marginnote{\ \textcolor{red}{\ {\sf R1\/}}}}
\newcommand{\rtwo}{\marginnote{\ \textcolor{red}{\ {\sf R2\/}}}}
\newcommand{\rthree}{\marginnote{\ \textcolor{red}{\ {\sf R3\/}}}}
\newcommand{\ronetwo}{\marginnote{\ \textcolor{red}{\ {\sf R1\/}, {\sf R2\/}}}}
\newcommand{\ronethree}{\marginnote{\ \textcolor{red}{\ {\sf R1\/}, {\sf R3\/}}}}

\newcommand{\ronefour}{\marginnote{\ \textcolor{red}{\ {\sf R1\/}, {\sf R4\/}}}}
\newcommand{\rtwothree}{\marginnote{\ \textcolor{red}{\ {\sf R2\/}, {\sf R3\/}}}}
\newcommand{\rtwofour}{\marginnote{\ \textcolor{red}{\ {\sf R2\/}, {\sf R4\/}}}}

\newcommand{\ronetwothree}{\marginnote{\ \textcolor{red}{\ {\sf
R1\/}, {\sf R2\/} {\sf R3\/}}}}
\newcommand{\ronethreefour}{\marginnote{\ \textcolor{red}{\ {\sf
R1\/}, {\sf R3\/} {\sf R4\/}}}}
\newcommand{\rtwothreefour}{\marginnote{\ \textcolor{red}{\ {\sf
R2\/}, {\sf R3\/} {\sf R4\/}}}}
 
\newcommand{\ronetwothreefour}{\marginnote{\ \textcolor{red}{\ {\sf
R1\/}, {\sf R2\/}, {\sf R3\/}  {\sf R4\/}}}}


\renewcommand{\RSCHANGE}[1]{\textcolor{darkgreen}{{#1}}}
%\renewcommand{\RSCHANGE}[1]{#1}
\newcommand{\RSCHANGEONE}[1]{\rone{}~\textcolor{blue}{{#1}}}
\newcommand{\RSCHANGETWO}[1]{\rtwo{}~\textcolor{blue}{{#1}}}
\newcommand{\RSCHANGETHREE}[1]{\rthree{}~\textcolor{blue}{{#1}}}
\newcommand{\RSCHANGEONETHREE}[1]{\ronethree{}~\textcolor{blue}{{#1}}}
\newcommand{\RSCHANGEONETWO}[1]{\ronetwo{}~\textcolor{blue}{{#1}}}
\newcommand{\RSCHANGETWOTHREE}[1]{\rtwothree{}~\textcolor{blue}{{#1}}}

\newcommand{\RSCHANGEFOUR}[1]{\rfour{}~\textcolor{blue}{{#1}}}
\newcommand{\RSCHANGEONEFOUR}[1]{\ronefour{}~\textcolor{blue}{{#1}}}
\newcommand{\RSCHANGETWOFOUR}[1]{\rtwofour{}~\textcolor{blue}{{#1}}}
\newcommand{\RSCHANGETHREEFOUR}[1]{\rtwothreefour{}~\textcolor{blue}{{#1}}}
\newcommand{\RSCHANGEONETHREEFOUR}[1]{\ronethreefour{}~\textcolor{blue}{{#1}}}



==> arxiv-version/rs_macros_mc.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% This file is an hard link, whose source is in   
%%%%%%% cipeciop.science.unitn.it:/home/rseba/latex/macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\nusmv}{{\sc NuSMV}}
\newcommand{\PROMELA}{{\sc PROMELA}}
\newcommand{\smv}{{\sc SMV}}

\newcommand{\bdds}{\text{BDD}s\xspace}
\newcommand{\bdd}{\textrm{BDD}\xspace}
%\newcommand{\imp}{\rightarrow}
\newcommand{\dis}{\vee}
\newcommand{\con}{\wedge}
\newcommand{\liff}{\leftrightarrow}
\newcommand{\true}{\top}
\newcommand{\false}{\bot}
\newcommand{\CTL}{\textsc{CTL}\xspace}
\newcommand{\LTL}{\textsc{LTL}\xspace}




%%% MACROS BMC
\newcommand{\E}{{\bf E\/}}
\newcommand{\A}{{\bf A\/}}
\newcommand{\G}{{\bf G\/}}
\newcommand{\F}{{\bf F\/}}
\newcommand{\U}{{\bf U\/}}
\newcommand{\R}{{\bf R\/}}
\newcommand{\X}{{\bf X\/}}
\newcommand{\AG}{{\bf AG\/}}
\newcommand{\AF}{{\bf AF\/}}
\newcommand{\AU}{{\bf AU\/}}
\newcommand{\AR}{{\bf AR\/}}
\newcommand{\AX}{{\bf AX\/}}
\newcommand{\EG}{{\bf EG\/}}
\newcommand{\EF}{{\bf EF\/}}
\newcommand{\EU}{{\bf EU\/}}
\newcommand{\ER}{{\bf ER\/}}
\newcommand{\EX}{{\bf EX\/}}

\newcommand{\n}[2]{[[#1]]_{#2}}
\newcommand{\kil}[3]{\ _{#3}[[#1]]_{k}^{#2}}
\newcommand{\ki}[2]{\kil{#1}{#2}{}}
\renewcommand{\k}[1]{\kil{#1}{}{}}
\newcommand{\kl}[2]{\kil{#1}{}{#2}}

\newcommand{\fkil}[2]{\kil{f}{#1}{#2}}
\newcommand{\fki}[1]{\kil{f}{#1}{}}
\newcommand{\fk}{\kil{f}{}{}}
\newcommand{\fkl}[1]{\kil{f}{}{#1}}

\newcommand{\gkil}[2]{\kil{g}{#1}{#2}}
\newcommand{\gki}[1]{\kil{g}{#1}{}}
\newcommand{\gk}{\kil{g}{}{}}
\newcommand{\gkl}[1]{\kil{g}{}{#1}}

\newcommand{\Lkl}[1]{\ _{#1}{L}_{k}}
\newcommand{\Lkkll}[2]{\ _{#2}{L}_{#1}}
\newcommand{\Lkll}[1]{{L}_{k|#1}}
\newcommand{\Lk}{{L}_{k}}

\newcommand{\Mkil}[3]{\kil{M}{#1}{#2}{#3}}
\newcommand{\Mki}[2]{\kil{M}{#1}{#2}{}}
\newcommand{\Mk}[1]{\kil{M}{#1}{}{}}
\newcommand{\Mkl}[2]{\kil{M}{#1}{}{#2}}


==> arxiv-version/rs_macros_optsmt.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% This file is an hard link, whose source is in   
%%%%%%% cipeciop.science.unitn.it:/home/rseba/latex/macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% 
%%%               MACROS SPECIFIC FOR SMT WITH COSTS
%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 

%%% FUNCTIONS

\newcommand{\omtproblem}{\triple{\vi}{\costfs}{\bounds}\xspace}
\newcommand{\omt}{\ensuremath{\text{OMT}}\xspace}
\newcommand{\bomt}{\ensuremath{\text{BOMT}}\xspace}
\newcommand{\omtt}{\ensuremath{\text{OMT}({\T})}\xspace}
\newcommand{\bomtt}{\ensuremath{\text{BOMT}({\T})}\xspace}

\newcommand{\omtplus}[1]{\ensuremath{\text{OMT}({#1})}\xspace}
\newcommand{\omlarat}{\ensuremath{\text{OMT}(\larat)}\xspace}
\newcommand{\omlaint}{\ensuremath{\text{OMT}(\laint)}\xspace}
\newcommand{\omla}{\ensuremath{\text{OMT}(\la)}\xspace}
\newcommand{\omlaintplus}{\ensuremath{\text{OMT}(\laint\cup\T)}\xspace}
\newcommand{\omlaratplus}{\ensuremath{\text{OMT}(\larat\cup\T)}\xspace}
\newcommand{\omlaplus}{\ensuremath{\text{OMT}(\la\cup\T)}\xspace}

\newcommand{\smtlaratplus}{\smttt{\larat\cup\T}\xspace}
\newcommand{\laratplus}{\ensuremath{\larat\cup\T}\xspace}


%cost function symbols
\newcommand{\costfs}{\ensuremath{\underline{costs}}\xspace}
\newcommand{\costfgen}[1]{\ensuremath{{cost}^{#1}}\xspace}
\newcommand{\costfi}{\costfgen{i}}
\newcommand{\costfone}{\costfgen{1}}
\newcommand{\costfM}{\costfgen{M}}

%cost variable symbols
\newcommand{\costs}{\ensuremath{\underline{c}}\xspace}
\newcommand{\costgen}[1]{\ensuremath{{c}^{#1}}\xspace}
\newcommand{\costi}{\costgen{i}}
\newcommand{\costone}{\costgen{1}}
\newcommand{\costM}{\costgen{M}}

%generic values symbols
\newcommand{\vvgen}[2]{\ensuremath{{\sf v}^{#1}_{#2}}\xspace}
\newcommand{\vvi}[1]{\vvgen{i}{#1}}
\newcommand{\wvgen}[2]{\ensuremath{{\sf w}^{#1}_{#2}}\xspace}
\newcommand{\wvi}[1]{\wvgen{i}{#1}}
\newcommand{\xvgen}[2]{\ensuremath{{\sf x}^{#1}_{#2}}\xspace}
\newcommand{\xvi}[1]{\xvgen{i}{#1}}
\newcommand{\yvgen}[2]{\ensuremath{{\sf y}^{#1}_{#2}}\xspace}
\newcommand{\yvi}[1]{\yvgen{i}{#1}}


%bounds symbols
\newcommand{\lbgen}[2]{\ensuremath{{\sf lb}^{#1}_{#2}}\xspace}
\newcommand{\ubgen}[2]{\ensuremath{{\sf ub}^{#1}_{#2}}\xspace}
\newcommand{\lb}{\lbgen{}{}}
\newcommand{\ub}{\ubgen{}{}}
\newcommand{\lbi}{\lbgen{i}{}}
\newcommand{\ubi}{\ubgen{i}{}}
\newcommand{\lbone}{\lbgen{1}{}}
\newcommand{\ubone}{\ubgen{1}{}}
\newcommand{\lbM}{\lbgen{M}{}}
\newcommand{\ubM}{\ubgen{M}{}}
\newcommand{\lbigen}[1]{\lbgen{i}{(#1)}}
\newcommand{\ubigen}[1]{\ubgen{i}{(#1)}}
\newcommand{\lbimax}{\lbgen{i}{max}}
\newcommand{\ubimin}{\ubgen{i}{min}}
\newcommand{\lbonemax}{\lbgen{1}{max}}
\newcommand{\ubonemin}{\ubgen{1}{min}}

\newcommand{\pivot}{\ensuremath{\mathsf{pivot}}\xspace}
\newcommand{\trueval}{{\ensuremath{\mathsf{true}}}}
\newcommand{\falseval}{{\ensuremath{\mathsf{false}}}}
%preds symbols
\newcommand{\tpredgen}[2]{{\ensuremath{\psi^{#1}_{#2}}}\xspace}
\newcommand{\tpredigen}[1]{\tpredgen{i}{#1}}
\newcommand{\tpredij}{\tpredigen{j}}
\newcommand{\predgen}[2]{{\ensuremath{A^{#1}_{#2}}}\xspace}
\newcommand{\predigen}[1]{\predgen{i}{#1}}
\newcommand{\predij}{\predigen{j}}
\newcommand{\predonej}{\predgen{1}{j}}

% symbols for PB section (to be coherent wrt. teh rest of the paper)
\newcommand{\Agen}[1]{\ensuremath{A_{#1}}\xspace}
\newcommand{\Aj}{\Agen{j}}
\newcommand{\aij}{\ensuremath{{\sf a}_{ij}}\xspace}
\newcommand{\bi}{\ensuremath{{\sf b}_{i}}\xspace}
\newcommand{\cj}{\ensuremath{{\sf c}_{j}}\xspace}
\newcommand{\ddj}{\ensuremath{{\sf d}_{j}}\xspace}
\newcommand{\lj}{\ensuremath{{l}_{j}}\xspace}

%cost values symbols
\newcommand{\cgen}[3]{{\ensuremath{{\sf c}^{#1}_{#2#3}}}\xspace}
\newcommand{\cigen}[2]{{\ensuremath{{\sf c}^{i}_{#1#2}}}\xspace}
\newcommand{\cijgen}[1]{{\ensuremath{{\sf c}^{i}_{j#1}}}\xspace}
\newcommand{\cijone}{{\ensuremath{{\sf c}^{i}_{j1}}}\xspace}
\newcommand{\cijtwo}{{\ensuremath{{\sf c}^{i}_{j2}}}\xspace}
\newcommand{\cij}{{\ensuremath{{\sf c}^{i}_{j}}}\xspace}
\newcommand{\conej}{{\ensuremath{{\sf c}^{1}_{j}}}\xspace}

\newcommand{\cc}{{\ensuremath{{\sf c}}}\xspace}


\newcommand{\bounds}{\ensuremath{\underline{\sf bounds}}\xspace}
\newcommand{\boundi}{\ensuremath{\langle\lbi,\ubi\rangle}\xspace}

\newcommand{\icost}{\ensuremath{{\sf IC}}\xspace}
\newcommand{\icostgen}[3]{\ensuremath{\icost(#3,#2,#1)}\xspace}
%\newcommand{\icostgen}[3]{\ensuremath{\icost_{#1#2}(#3,#1)}\xspace}
\newcommand{\icosti}[1]{\icostgen{\cigen{#1}{}}{#1}{\costgen{i}}}
\newcommand{\icostij}{\icostgen{\cij}{j}{\costgen{i}}}
\newcommand{\icostonej}{\icostgen{\cgen{1}{j}{}}{j}{\costgen{1}}}

\newcommand{\bcost}{\ensuremath{{\sf BC}}\xspace}
\newcommand{\cost}{\ensuremath{{cost}}\xspace}
\renewcommand{\costs}{\ensuremath{{costs}}\xspace}
\newcommand{\mincost}{\ensuremath{{mincost}}\xspace}
\newcommand{\bound}{\ensuremath{{bound}}\xspace}
\newcommand{\guess}{\ensuremath{{guess}}\xspace}
\newcommand{\oldguess}{\ensuremath{{oldguess}}\xspace}
\newcommand{\oldbound}{\ensuremath{{oldbound}}\xspace}
\newcommand{\maxboundi}{\ensuremath{{\sf bound}^{i}_{max}}\xspace}
\newcommand{\maxboundone}{\ensuremath{{\sf bound}^{1}_{max}}\xspace}
\newcommand{\nextsmallerbound}{\ensuremath{{\sf bound}_{next}}\xspace}
\newcommand{\noroom}{\ensuremath{{\sf NR}}\xspace}
\newcommand{\mustbe}{\ensuremath{{\sf MB}}\xspace}
\newcommand{\bleft}{\ensuremath{{lower}}\xspace}
\newcommand{\bright}{\ensuremath{{upper}}\xspace}
\newcommand{\pending}{\ensuremath{{\sf pending}}\xspace}

\newcommand{\tite}{\ensuremath{{ite}}\xspace}
\newcommand{\ite}{\ensuremath{{ITE}}\xspace}

\newcommand{\costof}[2]{\ensuremath{{\sf CostOf_{#1}}(#2)}\xspace}
\newcommand{\costiof}[1]{\costof{i}{#1}}
\newcommand{\mcostof}[2]{\ensuremath{{\sf MCostOf_{#1}}(#2)}\xspace}
\newcommand{\mcostiof}[1]{\mcostof{i}{#1}}

%%% THEORY OF COSTS

\newcommand{\C}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\Clemma}{\C-lemma\xspace}
\newcommand{\Csolver}{\TsolverGen{\C}}



%\newcommand{\TC}{\ensuremath{\mathcal{T}\cup\mathcal{C}}\xspace}
%\newcommand{\TC}{\ensuremath{(\mathcal{T}+\mathcal{C})}\xspace}
\newcommand{\incsmttc}{\ensuremath{\text{IncrementalSMT}_{\TC}}\xspace}
\newcommand{\smttcost}{\ensuremath{\text{SMT}(\T)+cost}\xspace}
\newcommand{\smttc}{\ensuremath{\text{SMT}({\TC})}\xspace}
\newcommand{\smtc}{\ensuremath{\text{SMT}({\C})}\xspace}
\newcommand{\Tlaint}{\ensuremath{\T\cup\laint}\xspace}
\newcommand{\smttlaint}{\ensuremath{\text{SMT}(\T\cup\laint)}\xspace}


\newcommand{\optsmttc}{\ensuremath{\text{OptSMT}_{\TC}}\xspace}

\newcommand{\decproblem}{\ensuremath{\triple{\vi}{\cost}{\bound}}\xspace}
\newcommand{\optproblem}{\ensuremath{\pair{\vi}{\cost}}\xspace}

%%% formulas
\newcommand{\vic}{\ensuremath{\vi_{\C}}\xspace}

%%% interface equalities
\newcommand{\eqij}{\ensuremath{(x_i=x_j)}\xspace}
\newcommand{\neqij}{\ensuremath{\neg(x_i=x_j)}\xspace}
\newcommand{\dij}{\ensuremath{(x_i<x_j)}\xspace}
\newcommand{\dji}{\ensuremath{(x_i>x_j)}\xspace}


%%% assignments
\newcommand{\muc}{\ensuremath{\mu_{\C}}\xspace}
\newcommand{\mucgen}[1]{\ensuremath{\mu^{#1}_{\C}}\xspace}
\newcommand{\muci}{\mucgen{i}}
\newcommand{\mut}{\ensuremath{\mu_{\T}}\xspace}
\newcommand{\mub}{\ensuremath{\mu_{\calb}}\xspace}

\newcommand{\mularat}{\ensuremath{\mu_{\larat}}\xspace}
\newcommand{\mubool}{\ensuremath{\mu_{\mathbb{B}}}\xspace}

\newcommand{\mue}{\ensuremath{\mu_{e}}\xspace}
\newcommand{\mud}{\ensuremath{\mu_{d}}\xspace}
\newcommand{\mui}{\ensuremath{\mu_{i}}\xspace}
\newcommand{\mued}{\ensuremath{\mu_{ed}}\xspace}
\newcommand{\muei}{\ensuremath{\mu_{ei}}\xspace}
\newcommand{\mueid}{\ensuremath{\mu_{eid}}\xspace}

\newcommand{\murelaxed}{\ensuremath{\mu_{rel}}\xspace}




%%% index sets
\newcommand{\Jplus}{\ensuremath{J^{i+}}\xspace}
\newcommand{\Jminus}{\ensuremath{J^{i-}}\xspace}
\newcommand{\Kplus}{\ensuremath{K^{i+}}\xspace}
\newcommand{\Kminus}{\ensuremath{K^{i-}}\xspace}
\newcommand{\Kplusone}{\ensuremath{K^{1+}}\xspace}
\newcommand{\Kminusone}{\ensuremath{K^{1-}}\xspace}


%%% interpretations
\newcommand{\Ilaint}{\ensuremath{\cali_{\laint}}\xspace}
\newcommand{\IT}{\ensuremath{\cali_{\T}}\xspace}
\newcommand{\I}{\ensuremath{\cali}\xspace}

%%% names of tools
\newcommand{\mathsatC}{\mathsat}
\newcommand{\scip}{{\sc Scip}\xspace}
\newcommand{\bsolo}{{\sc Bsolo}\xspace}
\newcommand{\satforj}{{\sc Sat4j}\xspace}
\newcommand{\pbclasp}{{\sc PBClasp}\xspace}

%%% VARIOUS
\newcommand{\bl}{\phantom{0}}



%\definecolor{mygray}{rgb}{0.99,0.99,0.99}
%% \definecolor{mygray}{rgb}{0.85,0.85,0.85}
\newcommand\mysout{\bgroup \markoverwith{{-}}\ULon}
\newcommand\nosout{\bgroup \markoverwith{{ }}\ULon}
\definecolor{mygray}{rgb}{0.90,0.90,0.90}
\definecolor{mywhite}{rgb}{1.00,1.00,1.00}
\def \gbox #1{\colorbox{mygray}{{#1}}}
\newcommand{\fal}[1]{\colorbox{mygray}{$\red{#1}$}}
\newcommand{\tru}[1]{\blue{#1}}

\newcommand{\mycite}[1]{{\footnotesize \textcolor{darkviolet}{#1}}}
\newcommand{\mcite}[1]{{\footnotesize \textcolor{darkviolet}{[#1]}}}
%\newcommand{\mycite}[1]{}

\newcommand{\mueuf}{\ensuremath{\mu_{\euf}}\xspace}
\newcommand{\mulaint}{\ensuremath{\mu_{\laint}}\xspace}
\newcommand{\infrule}[3]{\ensuremath{\displaystyle\frac{#2}{#3}}}
\newcommand{\hyp}{\textsc{Hyp}\xspace}
\newcommand{\comb}{\textsc{Comb}\xspace}

\newcommand{\fakeinfrule}[3]{\ensuremath{\displaystyle\begin{array}{l}\phantom{#2}}\\{#3}\end{array}}


%%% NUOVE DA PAPER TOCL

\newcommand{\currlb}{\ensuremath{\mathsf{l}}\xspace}
\newcommand{\currub}{\ensuremath{\mathsf{u}}\xspace}
\newcommand{\range}{\ensuremath{[\lb,\ub[}\xspace}
\newcommand{\currrange}{\ensuremath{[\currlb,\currub[}\xspace}
\newcommand{\lpivotrange}{\ensuremath{[\currlb,\pivot[}\xspace}
\newcommand{\rpivotrange}{\ensuremath{[\pivot,\currub[}\xspace}
\newcommand{\computepivot}{\ensuremath{{\sf ComputePivot}}\xspace}
%\newcommand{\dopivoting}{\ensuremath{{\sf DoPivoting()}}\xspace}
\newcommand{\dopivoting}{\ensuremath{{\sf BinSearchMode()}}\xspace}

\newcommand{\ubliti}[1]{\ensuremath{(\cost < #1)}\xspace}
\newcommand{\lbliti}[1]{\ensuremath{\neg(\cost < #1)}\xspace}
\newcommand{\pivotatom}{\ensuremath{\mathsf{PIV}}\xspace}
\newcommand{\currlblit}{\ensuremath{\neg(\cost < \currlb)}\xspace}
\newcommand{\currublit}{\ensuremath{(\cost < \currub)}\xspace}
\newcommand{\currubliti}[1]{\ensuremath{(\cost < \currub_{#1})}\xspace}
\newcommand{\negcurrubliti}[1]{\ensuremath{\neg(\cost < \currub_{#1})}\xspace}

\newcommand{\minvalue}{\ensuremath{\mathsf{min}}\xspace}
\newcommand{\maxvalue}{\ensuremath{\mathsf{max}}\xspace}
\newcommand{\mvalue}{\ensuremath{\mathsf{m}}\xspace}
\renewcommand{\mincost}{\ensuremath{\mathsf{min}_\cost}\xspace}

\newcommand{\minimize}{\ensuremath{\mathsf{Minimize}}\xspace}
\newcommand{\isminimum}{\ensuremath{\mathsf{IsMinimum}}\xspace}
%\newcommand{\incrementalsmt}{\ensuremath{\mathsf{IncrementalSMT}}\xspace}
\newcommand{\incrementalsmt}{\ensuremath{\mathsf{SMT.IncrementalSolve}}\xspace}
\newcommand{\smtcoreextract}{\ensuremath{\mathsf{SMT.ExtractUnsatCore}}\xspace}
\newcommand{\incrementalsmtcore}{\ensuremath{\mathsf{SMT.IncrementalSolve\&ExtractCore}}\xspace}
\newcommand{\laqliterals}{\larat\ensuremath{\mathsf{LiteralsOf}}\xspace}
 

\newcommand{\optimathsat}{\textsc{OptiMathSAT}\xspace}
\newcommand{\optmathsat}{\textsc{OptiMathSAT}\xspace}
\newcommand{\symba}{\textsc{Symba}\xspace}
\newcommand{\nuz}{\textsc{$\nu Z$}\xspace}
\newcommand{\bclt}{\textsc{bclt}\xspace}


==> arxiv-version/rs_macros_sat.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% This file is an hard link, whose source is in   
%%%%%%% cipeciop.science.unitn.it:/home/rseba/latex/macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% 
%%%               MACROS FOR SAT
%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\dpll}{\textsc{DPLL}\xspace}

%% SAT TOOLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\zchaff}    {\textsc{Zchaff}\xspace}
\newcommand{\satelite}  {\textsc{SAT-Elite}\xspace}
\newcommand{\siege}     {\textsc{Siege}\xspace}
\newcommand{\berkmin}   {\textsc{BerkMin}\xspace}
\newcommand{\minisat}   {\textsc{MiniSat}\xspace}
\newcommand{\minisattwo}{\textsc{MiniSat2}\xspace}



%% DPLL FUNCTIONS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\pickassign}{\ensuremath{\sf{pick\_assignment}}\xspace}
\newcommand{\picknewassign}{\ensuremath{\sf{pick\_new\_total\_assignment}}\xspace}
\newcommand{\picktotalassign}{\ensuremath{\sf{pick\_total\_assign}}\xspace}
\newcommand{\decidebranch}{\ensuremath{\sf{decide\_new\_branch}}\xspace}
\newcommand{\decide}{\ensuremath{\sf{decide}}\xspace}
\newcommand{\blevel}{\ensuremath{\sf{blevel}}\xspace}
\newcommand{\analyzeconflict}{\ensuremath{\sf{analyze\_conflict}}\xspace}
\newcommand{\analyzededuction}{\ensuremath{\sf{analyze\_deduction}}\xspace}
\newcommand{\backtrack}{\ensuremath{\sf{backtrack}}\xspace}
\newcommand{\bcp}{\ensuremath{\sf{boolean\_constraint\_propagation}}\xspace}

%% RETURN VALUES
\newcommand{\satres}{\textsc{sat}\xspace}
\newcommand{\unsatres}{\textsc{unsat}\xspace}
\newcommand{\unknownres}{\textsc{unknown}\xspace}
\newcommand{\conflres}{\ensuremath{\mathsf{conflict}}\xspace}

%%% WALKSAT/WALKSMT
\newcommand{\walksat}{WalkSAT\xspace}
\newcommand{\basicwalksmt}{\textsc{Basic-WalkSMT}\xspace}
\newcommand{\walksmt}{\textsc{WalkSMT}\xspace}

\newcommand{\tpreprocess}{\T{}{\sc -preprocess}\xspace}
\newcommand{\initialtruthassignment}{{\sc InitialTruthAssignment}\xspace}
\newcommand{\chooseunsatisfiedclause}{{\sc ChooseUnsatisfiedClause}\xspace}
\newcommand{\nexttruthassignment}{{\sc NextTruthAssignment}\xspace}


==> arxiv-version/rs_macros_smt.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% This file is an hard link, whose source is in   
%%%%%%% cipeciop.science.unitn.it:/home/rseba/latex/macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% 
%%%               MACROS FOR SMT 
%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%% USEFUL MACROS
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\proptofol}{\ensuremath{{\cal B}2{\cal T}}\xspace}
\newcommand{\foltoprop}{\ensuremath{{\cal T}2{\cal B}}\xspace}
\newcommand{\btot}{\proptofol}
\newcommand{\ttob}{\foltoprop}
% \newcommand{\satres}{\ensuremath{\mathsf{sat}}\xspace}
% \newcommand{\unsatres}{\ensuremath{\mathsf{unsat}}\xspace}
%\newcommand{\conflres}{\ensuremath{\mathsf{conflict}}\xspace}


%%% FREQUENTLY-USED symbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\vi}{\ensuremath{\varphi}\xspace}
\newcommand{\vip}{\ensuremath{\varphi^p}\xspace}
\newcommand{\mup}{\ensuremath{\mu^p}\xspace}
\newcommand{\muone}{\ensuremath{\mu_1}\xspace}
\newcommand{\mutwo}{\ensuremath{\mu_2}\xspace}
\newcommand{\muonetwo}{\ensuremath{\mu_1 \cup \mu_2}\xspace}
\newcommand{\taup}{\ensuremath{\tau^p}\xspace}
\newcommand{\etap}{\ensuremath{\eta^p}\xspace}
\newcommand{\cp}{\ensuremath{c^p}\xspace}

\newcommand{\atoms}[1]{\ensuremath{Atoms(#1)}\xspace}


%% THEORIES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\B}{\ensuremath{\mathcal{B}}\xspace}
\newcommand{\T}{\ensuremath{\mathcal{T}}\xspace}
\newcommand{\Tone}{\ensuremath{\T_1}\xspace}
\newcommand{\Ttwo}{\ensuremath{\T_2}\xspace}
\newcommand{\Tonetwo}{\ensuremath{\Tone\cup \Ttwo}\xspace}
\newcommand{\smt}{SMT\xspace}
\newcommand{\smtt}{\ensuremath{\text{SMT}(\T)}\xspace}
\newcommand{\smttt}[1]{\ensuremath{\text{SMT}(#1)}\xspace}
\newcommand{\smttonettwo}{\ensuremath{\text{SMT}(\tonetwo)}\xspace}
\newcommand{\Ti}{\ensuremath{\T_i}\xspace}
\newcommand{\tmany}{\ensuremath{\bigcup_i \T_i}\xspace}
\newcommand{\smtmany}{\ensuremath{\mathit{SMT}(\bigcup_i \T_i)}\xspace}

\newcommand{\utvpi}{\ensuremath{\mathcal{UTVPI}}\xspace}
\newcommand{\utvpiint}{\ensuremath{\mathcal{UTVPI(\mathbb{Z})}}\xspace}
\newcommand{\utvpirat}{\ensuremath{\mathcal{UTVPI(\mathbb{Q})}}\xspace}
\newcommand{\bool}{\ensuremath{\mathcal{BOOL}}\xspace}
\newcommand{\euf}{\ensuremath{\mathcal{EUF}}\xspace}
\newcommand{\eq}{\ensuremath{\mathcal{E}}\xspace}
\newcommand{\dl}{\ensuremath{\mathcal{DL}}\xspace}
\newcommand{\dlrat}{\ensuremath{\mathcal{DL(\mathbb{Q})}}\xspace}
\newcommand{\dlint}{\ensuremath{\mathcal{DL(\mathbb{Z})}}\xspace}
\newcommand{\la}{\ensuremath{\mathcal{LA}}\xspace}
\newcommand{\larat}{\ensuremath{\mathcal{LA}(\mathbb{Q})}\xspace}
\newcommand{\laint}{\ensuremath{\mathcal{LA}(\mathbb{Z})}\xspace}
\newcommand{\laratint}{\ensuremath{\mathcal{LA}(\mathbb{Q}\mathbb{Z})}\xspace}
%%%%%%%%%%%%% RISCRITTE
\renewcommand{\la}{\ensuremath{\mathcal{LA}}\xspace}
\renewcommand{\larat}{\ensuremath{\mathcal{LRA}}\xspace}
\renewcommand{\laint}{\ensuremath{\mathcal{LIA}}\xspace}
\renewcommand{\laratint}{\ensuremath{\mathcal{LA}}\xspace}


\newcommand{\fl}{\ensuremath{\mathcal{FP}}\xspace}
\newcommand{\nla}{\ensuremath{\mathcal{NLA}}\xspace}
\newcommand{\nlarat}{\ensuremath{\mathcal{NLA}(\mathbb{R})}\xspace}
\newcommand{\nlaint}{\ensuremath{\mathcal{NLA}(\mathbb{Z})}\xspace}
\newcommand{\bv}{\ensuremath{\mathcal{BV}}\xspace}
\newcommand{\mem}{\ensuremath{\mathcal{AR}}\xspace}
\newcommand{\lists}{\ensuremath{\mathcal{LI}}\xspace}
\newcommand{\tonetwo}{\ensuremath{\T_1\cup\T_2}\xspace}

\newcommand{\smteuf}{\smttt{\euf}}
\newcommand{\smtdl}{\smttt{\dl}}
\newcommand{\smtdlrat}{\smttt{\dlrat}}
\newcommand{\smtdlint}{\smttt{\dlint}}
\newcommand{\smtutvpi}{\smttt{\utvpi}}
\newcommand{\smtutvpirat}{\smttt{\utvpirat}}
\newcommand{\smtutvpiint}{\smttt{\utvpiint}}
\newcommand{\smtla}{\smttt{\la}}
\newcommand{\smtlarat}{\smttt{\larat}}
\newcommand{\smtlaint}{\smttt{\laint}}
\newcommand{\smtbv}{\smttt{\bv}}
\newcommand{\smtmem}{\smttt{\mem}}


\newcommand{\genmodels}[1]{\models_{#1}}
\newcommand{\Tmodels}{\models_{\T}}
\newcommand{\laratmodels}{\models_{\larat}}
\newcommand{\laintmodels}{\models_{\laint}}
\newcommand{\lamodels}{\models_{\la}}
\newcommand{\dlmodels}{\models_{\dl}}
\newcommand{\dlintmodels}{\models_{\dlint}}
\newcommand{\dlratmodels}{\models_{\dlrat}}
\newcommand{\pmodels}{\models_p}

%% T-solvers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\TsolverGen}[1]{\ensuremath{{#1}\textit{-solver}}\xspace}
\newcommand{\TsolversGen}[1]{\ensuremath{{#1}\textit{-solvers}}\xspace}
\newcommand{\Tsolver}{\TsolverGen{\T}}
\newcommand{\Tsolvers}{\TsolversGen{\T}}
\newcommand{\Psolver}{\TsolverGen{\mathsf{Bool}}}
\newcommand{\TTsolver}[1]{\TsolverGen{\ensuremath{#1}}}
\newcommand{\Tonesolver}{\TsolverGen{\ensuremath{\Tone}}}
\newcommand{\Ttwosolver}{\TsolverGen{\ensuremath{\Ttwo}}}
\newcommand{\Tonetwosolver}{\TsolverGen{\ensuremath{\Tone\cup \Ttwo}}}
\newcommand{\Tisolver}{\TsolverGen{\ensuremath{\Ti}}}
\newcommand{\Tisolvers}{\TsolversGen{\ensuremath{\Ti}}}
\newcommand{\TdeduceGen}[1]{\ensuremath{{#1}\textit{-deduce}}\xspace}
\newcommand{\Tonededuce}{\TdeduceGen{\ensuremath{\Tone}}}
\newcommand{\Ttwodeduce}{\TdeduceGen{\ensuremath{\Ttwo}}}

\newcommand{\Tlemma}{\T-lemma\xspace}
\newcommand{\Tlemmas}{\T-lemmas\xspace}
\newcommand{\Tilemma}{\Ti-lemma\xspace}
\newcommand{\Tilemmas}{\Ti-lemmas\xspace}

\newcommand{\laratsolver}{\larat-\ensuremath{\mathsf{Solver}}}
\newcommand{\laratsolvers}{\larat-\ensuremath{\mathsf{Solvers}}}
\newcommand{\laintsolver}{\laint-\ensuremath{\mathsf{Solver}}}
\newcommand{\laintsolvers}{\laint-\ensuremath{\mathsf{Solvers}}}
\newcommand{\lasolver}{\la-\ensuremath{\mathsf{Solver}}}
\newcommand{\lasolvers}{\la-\ensuremath{\mathsf{Solvers}}}

%% SMT TOOLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\argolib}{\textsc{ArgoLib}\xspace}
\newcommand{\barcelogic}{\textsc{Barcelogic}\xspace}
\newcommand{\blast}{\textsc{Blast}\xspace}
\newcommand{\clp}{\textsc{clp-prover}\xspace}
\newcommand{\csisat}{\textsc{CSIsat}\xspace}
\newcommand{\cvcthree}{\textsc{CVC3}\xspace}
\newcommand{\foci}{\textsc{Foci}\xspace}
\newcommand{\haRVey}{\textsc{haRVey}\xspace}
\newcommand{\intjain}{\textsc{INT2}\xspace}
\newcommand{\lifter}{\textsc{Lifter}\xspace}
\newcommand{\mathsat}{\textsc{MathSAT}\xspace}
\newcommand{\verifun} {\textsc{Verifun}\xspace}
\newcommand{\yices}{\textsc{Yices}\xspace}
\newcommand{\zapato}  {\textsc{Zapato}\xspace}
\newcommand{\zap}{\textsc{Zap}\xspace}
\newcommand{\zthree}{\textsc{Z3}\xspace}

\newcommand{\microformal}{\textsc{MicroFormal}\xspace}

\newcommand{\mathsatfour}{\textsc{MathSAT4}\xspace}
\newcommand{\mathsatfive}{\textsc{MathSAT5}\xspace}
\newcommand{\mathsatfivePrep}{\textsc{MathSAT5}$_{\textsc{preprocessing}}$\xspace}
\newcommand{\mathsatfiveCleaneling}{\textsc{MathSAT5}$_{\cleaneling}$\xspace}
\newcommand{\mathsatfiveMinisat}{\textsc{MathSAT5}$_{\minisat}$\xspace}

%% THEORY COMBINATION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\myeij}{\ensuremath{e_{ij}}\xspace}
\newcommand{\myeijs}{\ensuremath{e_{ij}}s\xspace}
\newcommand{\mynegeij}{\ensuremath{\neg e_{ij}}\xspace}
\newcommand{\eij}{\ensuremath{v_i=v_j}\xspace}
\newcommand{\eik}{\ensuremath{v_i=v_k}\xspace}
\newcommand{\ejk}{\ensuremath{v_j=v_k}\xspace}
\newcommand{\diseij}{\ensuremath{\vee(\eij)}\xspace}

\newcommand{\NO}{\ensuremath{\mathsf{no}(T_1,T_2)}\xspace}
\newcommand{\Bool}{\ensuremath{\mathsf{Bool}}\xspace}
\newcommand{\BoolGen}[1]{\ensuremath{\mathsf{Bool+}{#1}}\xspace}
\newcommand{\BoolT}{\BoolGen{T}}
\newcommand{\BoolTonetwo}{\BoolGen{T_1+T_2}}
\newcommand{\BoolTi}{\BoolGen{{T_i}}}
\newcommand{\BoolNO}{\BoolGen{\NO}}
\newcommand{\DelBoolNO}{\ensuremath{{\mathsf{Bool+}}T_1{\mathsf{+}}T_2}\xspace}
 
\newcommand{\TsatisfiableGen}[1]{\ensuremath{{#1}\textit{-satisfiable}}\xspace}
\newcommand{\TsatGen}[1]{\ensuremath{{#1}\textit{-sat}}\xspace}
\newcommand{\TunsatGen}[1]{\ensuremath{{#1}\textit{-unsat}}\xspace}
\newcommand{\Tonesat}{\TsatGen{\ensuremath{T_1}}}
\newcommand{\Ttwosat}{\TsatGen{\ensuremath{T_2}}}
\newcommand{\Toneunsat}{\TunsatGen{\ensuremath{T_1}}}
\newcommand{\Ttwounsat}{\TunsatGen{\ensuremath{T_2}}}
\newcommand{\Tsatisfiable}{\TsatisfiableGen{T}}
\newcommand{\Psatisfiable}{\TsatisfiableGen{\mathsf{Bool}}}
\newcommand{\Tonesatisfiable}{\TsatisfiableGen{\ensuremath{T_1}}}
\newcommand{\Ttwosatisfiable}{\TsatisfiableGen{\ensuremath{T_2}}}
\newcommand{\Tisatisfiable}{\TsatisfiableGen{\ensuremath{T_i}}}
 


==> arxiv-version/rs_macros_specific.tex <==

\renewcommand{\new}[1]{{\em #1}}
%\renewcommand{\thus}{{\ensuremath \Rightarrow}}
\renewcommand{\RSTODO}[1]{{\bf \textcolor{darkgreen}{{\fbox{RS TODO:} #1}}}}
\renewcommand{\paragraph}[1]{\smallskip\noindent{\emph{#1}}}


\newcommand{\alla}{\ensuremath{{\mathbf{A}}}\xspace}
\newcommand{\allb}{\ensuremath{{\mathbf{B}}}\xspace}
\renewcommand{\vi}{\ensuremath{\varphi_{[\alla]}}\xspace}
\newcommand{\vione}{\ensuremath{\varphi'_{[\alla]}}\xspace}
\newcommand{\vitwo}{\ensuremath{\varphi''_{[\alla]}}\xspace}
\renewcommand{\vi}{\ensuremath{\varphi}\xspace}
\renewcommand{\vione}{\ensuremath{\varphi_{1}}\xspace}
\renewcommand{\vitwo}{\ensuremath{\varphi_{2}}\xspace}
\newcommand{\ps}{\ensuremath{\psi_{[\alla,\allb]}}\xspace}

\renewcommand{\trueval}{\ensuremath{\mbox{{\sf T}}\xspace}}
\renewcommand{\falseval}{\ensuremath{\mbox{{\sf F}}\xspace}}
\newcommand{\unknown}{\ensuremath{\mbox{{\sf ?}}\xspace}}

\newcommand{\tval}{\trueval}
\newcommand{\fval}{\falseval}
\newcommand{\uval}{\unknown}
% \newcommand{\tval}{{\mathsf T}\xspace}
% \newcommand{\fval}{{\mathsf F}\xspace}
% \newcommand{\uval}{\ensuremath{{\mathsf ?}\xspace}}

\newcommand{\andmu}{\ensuremath{\bigwedge\!\mu}\xspace}
\newcommand{\andeta}{\ensuremath{\bigwedge\!\eta}\xspace}


\newcommand{\apply}[2]{\ensuremath{#1|_{#2}}\xspace}
\newcommand{\applymuvi}{\apply{\vi}{\mu}\xspace}
\newcommand{\applyetavi}{\apply{\vi}{\eta}\xspace}

\newcommand{\muof}[1]{\ensuremath{\mu(#1)}}
\newcommand{\etaof}[1]{\ensuremath{\eta(#1)}}

\newcommand{\oksym}{{\Large \ensuremath{\textcolor{darkgreen}{\checkmark}}}\xspace}
\newcommand{\noksym}{{\LARGE \ensuremath{\textcolor{red}{\mathbf{\times}}}}\xspace}

\newcommand{\shannon}[2]{\ensuremath{#1|_{\exists#2}}\xspace}
\renewcommand{\shannon}[2]{\ensuremath{{\sf SE}[{\exists#2}.#1}]\xspace}
\newcommand{\shannonpsib}{\shannon{\psi}{\allb}}

\newcommand{\predabsphi}{\ensuremath{{\sf PredAbs}(\phi,\set{\phi_i}_{i=1}^N)}}
\renewcommand{\predabsphi}{\ensuremath{{\sf PredAbs}(\phi,{\mathbf \Phi})}}

\newcommand{\genericentails}{\mid\!\simeq}
\newcommand{\entails}{\ensuremath{\models}}
\newcommand{\verifies}{\vdash}
\renewcommand{\verifies}{\Vdash}
\renewcommand{\verifies}{\ensuremath{\mid\!\approx}}

\newcommand{\verbverify}{validate}
\newcommand{\verbverified}{validated}
\newcommand{\verbverifies}{validates}
\newcommand{\verbverifying}{validating}
\newcommand{\verbverification}{verification}
\newcommand{\Verbverification}{Verification}

\renewcommand{\verbverify}{evaluate to true}
\renewcommand{\verbverified}{evaluated to true}
\renewcommand{\verbverifies}{evaluates to true}
\renewcommand{\verbverifying}{evaluating to true}
\renewcommand{\verbverification}{evaluation to true}
\renewcommand{\Verbverification}{Evaluation to true}

\renewcommand{\verbverify}{verify}
\renewcommand{\verbverified}{verified}
\renewcommand{\verbverifies}{verifies}
\renewcommand{\verbverifying}{verifying}
\renewcommand{\verbverification}{verification}
\renewcommand{\Verbverification}{Verification}

\newcommand{\verbfalsifies}{falsifies}



\renewcommand{\RSTODO}[1]{\todo[size=\tiny,color=green!40]{{\small{#1}}}}

\newcommand{\cnfnamed}[1]{\ensuremath{\mathsf{CNF_{#1}}}}
\newcommand{\DeMorganCNF}{\cnfnamed{DM}}
\newcommand{\TseitinCNF}{\cnfnamed{Ts}}
\newcommand{\PlaistedCNF}{\cnfnamed{PG}}
\newcommand{\NNF}[1]{\ensuremath{\mathsf{NNF}(#1)}}
\newcommand{\NNFna}[1]{\ensuremath{\mathsf{NNF}}}

%%%% figures
\newcommand{\mainwffone}{\ensuremath{(A_1\wedge  A_2)\vee(A_1\wedge \neg A_2)}}
\newcommand{\mainwfftwo}{\ensuremath{(\neg A_3\wedge  A_4)\vee(\neg A_3\wedge \neg A_4)}}
\newcommand{\mainwff}{\ensuremath{(\mainwffone)\wedge(\mainwfftwo)}}
\newcommand{\mainwffstacked}{\ensuremath{
    \begin{array}{c}
      \mainwffone \\
      \mainwfftwo
    \end{array}}}
\newcommand{\wffl}{\ensuremath{(A_1\wedge  A_2)}}
\newcommand{\wffr}{\ensuremath{(A_1\wedge \neg A_2)}}
\newcommand{\wffltwo}{\ensuremath{(\neg A_3\wedge  A_4)}}
\newcommand{\wffrtwo}{\ensuremath{(\neg A_3\wedge \neg A_4)}} 
\newcommand{\Aone}{\ensuremath{A_1}}
\newcommand{\nAone}{\ensuremath{\neg A_1}}
\newcommand{\Atwo}{\ensuremath{A_2}}
\newcommand{\nAtwo}{\ensuremath{\neg A_2}}  
\newcommand{\Athree}{\ensuremath{A_3}}
\newcommand{\nAthree}{\ensuremath{\neg A_3}}
\newcommand{\Afour}{\ensuremath{A_4}}
\newcommand{\nAfour}{\ensuremath{\neg A_4}} 
\newcommand{\singlemu}{\set{A_1,\neg A_3}}
\newcommand{\singlemuset}{\set{\set{A_1,\neg A_3}}}
\newcommand{\allmus}{
  \set{
    \set{A_1,A_2,\neg A_3,A_4},
    \set{A_1,A_2,\neg A_3,\neg A_4},
    \set{A_1,\neg A_2,\neg A_3,A_4},
    \set{A_1,\neg A_2,\neg A_3,\neg A_4}}}


==> arxiv-version/thanks.tex <==
\section*{Acknowledgements} 

The analysis described in this paper has
strongly benefitted from interesting discussions, either in person or via
email, with (in alphabetic order):
Armin Biere,
Alessandro Cimatti,
Dror Fried,
Allen van Gelder,
Gabriele Masina,
David Mitchell,
Sibylle M\"ohle,
Paolo Morettin,
Andrea Passerini,
Alexander Nadel,
Yogev Shalmon,
Laurent Simon,
Giuseppe Spallitta,
Armando Tacchella,
Stefano Tonetta,
and
Moshe Vardi,
whom are all warmly thanked.



==> arxiv-version/todo.tex <==
\newpage
\section*{TODO}
\begin{itemize}
\item Everywhere
  \begin{itemize}
  \item 
  \item 
  \item
  \end{itemize}

\item INTRO
  \begin{itemize}
  \item add mention to poll
  \item add content
  \end{itemize}
\item background: 
  \begin{itemize}
  \item 
  \item 
  \end{itemize}
\item satisfiability
  \begin{itemize}
  \item 
  \item 
\item 
  \item 
  \end{itemize}
\item existential satisfiability
  \begin{itemize}
  \item 
  \item 
  \end{itemize}
\item POLL
  \begin{itemize}
  \item 
  \item 
  \end{itemize}
\end{itemize}




==> figure.tex <==
\newcommand{\mainwff}{\ensuremath{(A_1\wedge  A_2)\vee(A_1\wedge \neg A_2)}}
\newcommand{\wffl}{\ensuremath{(A_1\wedge  A_2)}}
\newcommand{\wffr}{\ensuremath{(A_1\wedge \neg A_2)}}
\newcommand{\Aone}{\ensuremath{A_1}}
\newcommand{\nAone}{\ensuremath{\neg A_1}}
\newcommand{\Atwo}{\ensuremath{A_2}}
\newcommand{\nAtwo}{\ensuremath{\neg A_2}}  
\newcommand{\singlemu}{\set{A_1}}
\newcommand{\allmus}{\set{\set{A_1,A_2},\set{A_1,\neg A_2}}}
% 
\begin{figure}[t]  
  \centering   
\scalebox{.8}{\input{comparison.pdf_t}} 
\caption{Left: OBDD for $\vi\defas\mainwff{}$. \newline
Center and right: Assignment enumeration for  $\vi$ via Analytic
Tableaux and (non-CNF) DPLL.
\label{fig:comparison}} 
\end{figure} 


==> figure_long.tex <==
\newcommand{\mainwffone}{\ensuremath{(A_1\wedge  A_2)\vee(A_1\wedge \neg A_2)}}
\newcommand{\mainwfftwo}{\ensuremath{(\neg A_3\wedge  A_4)\vee(\neg A_3\wedge \neg A_4)}}
\newcommand{\mainwff}{\ensuremath{(\mainwffone)\wedge(\mainwfftwo)}}
\newcommand{\mainwffstacked}{\ensuremath{
    \begin{array}{c}
      \mainwffone \\
      \mainwfftwo
    \end{array}}}
\newcommand{\wffl}{\ensuremath{(A_1\wedge  A_2)}}
\newcommand{\wffr}{\ensuremath{(A_1\wedge \neg A_2)}}
\newcommand{\wffltwo}{\ensuremath{(\neg A_3\wedge  A_4)}}
\newcommand{\wffrtwo}{\ensuremath{(\neg A_3\wedge \neg A_4)}} 
\newcommand{\Aone}{\ensuremath{A_1}}
\newcommand{\nAone}{\ensuremath{\neg A_1}}
\newcommand{\Atwo}{\ensuremath{A_2}}
\newcommand{\nAtwo}{\ensuremath{\neg A_2}}  
\newcommand{\Athree}{\ensuremath{A_3}}
\newcommand{\nAthree}{\ensuremath{\neg A_3}}
\newcommand{\Afour}{\ensuremath{A_4}}
\newcommand{\nAfour}{\ensuremath{\neg A_4}} 
\newcommand{\singlemu}{\set{A_1,\neg A_3}}
\newcommand{\allmus}{
  \set{
    \set{A_1,A_2,\neg A_3,A_4},
    \set{A_1,A_2,\neg A_3,\neg A_4},
    \set{A_1,\neg A_2,\neg A_3,A_4},
    \set{A_1,\neg A_2,\neg A_3,\neg A_4}}}
%  
\begin{figure}[t]  
  \centering 
\scalebox{.8}{\input{comparison_long.pdf_t}} 
\caption{$\vi\defas\mainwff{}$.
%\TODO{Split into two figures}  
  \TODO{Add example of d-DNNFs and SDDs}
  \TODO{add example with dualiza/HALL}
\TODO{Add example of enumeration of CNF-ized formula}
Left and center: Assignment enumeration for $\vi$  via Analytic
Tableaux and (non-CNF) DPLL. 
Right: OBDD for $\vi$.
\label{fig:comparison}} 
\end{figure} 


==> intro.tex.1 <==
% Although  CDCL 
% \cite{MSLM09HBSAT} 
% and SLS \cite{Maj09HBSAT} SAT solvers return  {\em total} truth assignments
% satisfying the input formula, other SAT procedures 
Many procedures for for SAT and SAT-related problems
(e.g. OBDDs
\cite{bryant2}, Analytic Tableaux \cite{smullyan1}, DPLL
\cite{davis7}) rely their efficiency
on the detection of {\em partial} assignments satisfying an input
formula.
In particular,
when it comes to SAT-based problems requiring
the complete enumeration of satisfying assignments (e.g. \#SAT
\cite{GSS09HBSAT}, Lazy SMT \cite{BSST09HBSAT}, AllSAT and AllSMT
\cite{allsmt}, satisfiability of modal and description logics
\cite{ST09HBSAT}), the capability of enumerating  {\em
partial}  satisfying assignments which are as small as possible is often essential, because 
detecting that a partial assignment satisfies the input formula 
may avoid the enumeration of the whole subtree
of total assignments extending it, whose size is exponential in the
number of unassigned propositions.

% a satisfying partial
% assignment can be generated instead of the whole subtree
% of total assignments extending it, whose size is exponential in the
% number of unassigned propositions.

% When we deal with (tautology-free) CNF formulas, the notion of
% partial-assignment satisfiablity is clear SPIEGA E CITA. BOTH PROPERTIES

In this paper we analyze in deep the notion of partial-assignment
satisfiability. 
First we raise a flag on the fact that by
``{\em a partial truth assignment $\mu$ satisfies a formula $\vi$}'',
we may mean either that $\mu$ {\em entails} $\vi$
(i.e. that all total assignments extending $\mu$
satisfy $\vi$) or that $\mu$ {\em validates} $\vi$
 (i.e. that applying $\mu$ to $\vi$ makes $\vi$ true).
%
Typically most authors in the SAT community
leave this definition
implicit, or provide a definition only for (tautology-free) CNF
formulas (e.g. \cite{KBK09HBSAT}).
% where we notice that
% entailment and validation concide. 
%
We notice that, whereas for (tautology-free) CNF formulas entailment 
and validation are equivalent, for non-CNF formulas --and for
existentially-quantified formulas, even CNF ones--
{\em validation is strictly stronger than entailment}, and they have
complementary properties. 

We also notice that 
 (Tseitin-style) CNF-ization does not solve this
issue, because 
%with Tseitin CNF-ization 
it may lose 
information regarding partial-assignment entailment or validation.
%\ignoreinshort{\RSTODO{Mention Kripke \& C e Stefano Tonetta?}}
%We stress the fact that the 

We stress the fact that the distinction between entailment and validation
is not just an issue of terminology; rather, it 
has important consequences at
algorithmic level. 
%
We notice, e.g., that
OBDDs \cite{bryant2} implicitly enumerate partial assignment {\em entailing}
the input formulas, whereas Analytic Tableaux \cite{smullyan1} and
(non-CNF) DPLL \cite{davis7} implicitly enumerate partial assignment
{\em validating} it. 
%
Also, e.g., techniques like {\em pure-literal
filtering} 
%and {\em ghost-literal filtering} 
\cite{sebastiani07,BSST09HBSAT} in lazy
SMT 
implicitly aim at reducing a
total assignment to a partial one {\em validating} the input formula. 
%
On the one hand, checking entailment is computationally
much harder than checking
validation. On the other hand, since partial assignments entailing
$\vi$ are in general subsets of those validating $\vi$, being able
to produce  partial assignments
{\em entailing} the input formula rather than {\em validating} it
 allows for producing smaller partial assignments,
and hence possibly drastically reducing their number. 
This may drive the development of more effective assignment-enumeration algorithms.
%
% When it comes to enumerating, in order to maximizing efficiency
% we would like to produce  partial assignments
% entailing the input formula, although most 
% algorithms give us only partial assignments
% validating it.

%\RSTODO{Aggiungi riferimento a poll.\\}
\ignore{
\paragraph{A poll.}
In order to support the analysis, I've set up an email
poll among some current or past SAT PC and some SMT PC members, asking
for the truth/falsehood of five statements on the
notion of partial-assignment satisfiability.
The result are available at \cite{poll} %
%\footnote{\url{http://disi.unitn.it/rseba/partialsat_poll_2019.03.11.pdf}}
 and as an appendix submitted with this paper. 
Although only 20 out of 65 people replied, 
the result 
reveals the lack of general agreement among the repliers on the notion of
partial-assignment satisfiability and on its consequences: e.g.,
% since 
the repliers split evenly into supporters 
of entailment, of validation, and people considering them equivalent.
}


\paragraph{Personal note.} The analysis presented in this paper was
triggered
by the effort of conceiving more efficient procedures for predicate
abstraction in SMT for improving Weighted Model Integration
\cite{MorPasSeb17,morettin_aij19},
which forced me to elaborate on the distinction between entailment
and validation. Before then, I personally used to see
partial-assignment satisfiability as {entailment}
 (see \cite{gs-infocomp2000}) without paying attention to the distinction.

{\paragraph{Content.} The rest of the paper is organized as follows.
\sref{sec:background} provides the necessary notation, terminology
and concepts used in the paper.
\sref{sec:partialsat} introduces entailment and
validation for generic propositional formulas and discusses their
relative properties and use.
\sref{sec:partialsat-exist} lifts the discussion to
existentially-quantified formulas.
\sref{sec:concl} provides some conclusions and future-work suggestions.
}



==> intro_v1.tex <==
% Although  CDCL 
% \cite{MSLM09HBSAT} 
% and SLS \cite{Maj09HBSAT} SAT solvers return  {\em total} truth assignments
% satisfying the input formula, other SAT procedures 
Many procedures for for SAT and SAT-related problems
(e.g. OBDDs
\cite{bryant2}, Analytic Tableaux \cite{smullyan1}, DPLL
\cite{davis7}) rely their efficiency
on the detection of {\em partial} assignments satisfying an input
formula.
In particular,
when it comes to SAT-based problems requiring
the complete enumeration of satisfying assignments (e.g. \#SAT
\cite{GomesSS21}, Lazy SMT \cite{BarrettSST21}, AllSAT and AllSMT
\cite{allsmt}, satisfiability of modal and description logics
\cite{SebastianiT21}), the capability of enumerating  {\em
partial}  satisfying assignments which are as small as possible is often essential, because 
detecting that a partial assignment satisfies the input formula 
may avoid the enumeration of the whole subtree
of total assignments extending it, whose size is exponential in the
number of unassigned propositions.

% a satisfying partial
% assignment can be generated instead of the whole subtree
% of total assignments extending it, whose size is exponential in the
% number of unassigned propositions.

% When we deal with (tautology-free) CNF formulas, the notion of
% partial-assignment satisfiablity is clear SPIEGA E CITA. BOTH PROPERTIES

In this paper we analyze in deep the notion of partial-assignment
satisfiability. 
First we raise a flag on the fact that by
``{\em a partial truth assignment $\mu$ satisfies a formula $\vi$}'',
we may mean either that $\mu$ {\em entails} $\vi$
(i.e. that all total assignments extending $\mu$
satisfy $\vi$) or that $\mu$ {\em verifies} $\vi$
 (i.e. that applying $\mu$ to $\vi$ makes $\vi$ true).
%
Typically most authors in the SAT community
leave this definition
implicit, or provide a definition only for (tautology-free) CNF
formulas (e.g. \cite{BuningK21}).
% where we notice that
% entailment and verification concide. 
%
We notice that, whereas for (tautology-free) CNF formulas entailment 
and verification are equivalent, for non-CNF formulas --and for
existentially-quantified formulas, even CNF ones--
{\em verification is strictly stronger than entailment}, and they have
complementary properties. 

We also notice that 
 (Tseitin-style) CNF-ization does not solve this
issue, because 
%with Tseitin CNF-ization 
it may lose 
information regarding partial-assignment entailment or verification.
%\ignoreinshort{\RSTODO{Mention Kripke \& C e Stefano Tonetta?}}
%We stress the fact that the 

We stress the fact that the distinction between entailment and verification
is not just an issue of terminology; rather, it 
has important consequences at
algorithmic level. 
%
We notice, e.g., that
OBDDs \cite{bryant2} implicitly enumerate partial assignment {\em entailing}
the input formulas, whereas Analytic Tableaux \cite{smullyan1} and
(non-CNF) DPLL \cite{davis7} implicitly enumerate partial assignment
{\em verifying} it. 
%
Also, e.g., techniques like {\em pure-literal
filtering} 
%and {\em ghost-literal filtering} 
\cite{sebastiani07,BarrettSST21} in lazy
SMT 
implicitly aim at reducing a
total assignment to a partial one {\em verifying} the input formula. 
%
On the one hand, checking entailment is computationally
much harder than checking
verification. On the other hand, since partial assignments entailing
$\vi$ are in general subsets of those verifying $\vi$, being able
to produce  partial assignments
{\em entailing} the input formula rather than {\em verifying} it
 allows for producing smaller partial assignments,
and hence possibly drastically reducing their number. 
This may drive the development of more effective assignment-enumeration algorithms.
%
% When it comes to enumerating, in order to maximizing efficiency
% we would like to produce  partial assignments
% entailing the input formula, although most 
% algorithms give us only partial assignments
% verifying it.

%\RSTODO{Aggiungi riferimento a poll.\\}
\ignore{
\paragraph{A poll.}
In order to support the analysis, I've set up an email
poll among some current or past SAT PC and some SMT PC members, asking
for the truth/falsehood of five statements on the
notion of partial-assignment satisfiability.
The result are available at \cite{poll} %
%\footnote{\url{http://disi.unitn.it/rseba/partialsat_poll_2019.03.11.pdf}}
 and as an appendix submitted with this paper. 
Although only 20 out of 65 people replied, 
the result 
reveals the lack of general agreement among the repliers on the notion of
partial-assignment satisfiability and on its consequences: e.g.,
% since 
the repliers split evenly into supporters 
of entailment, of verification, and people considering them equivalent.
}


\paragraph{Personal note.} The analysis presented in this paper was
triggered
by the effort of conceiving more efficient procedures for predicate
abstraction in SMT for improving Weighted Model Integration
\cite{MorPasSeb17,morettin_aij19},
which forced me to elaborate on the distinction between entailment
and verification. Before then, I personally used to see
partial-assignment satisfiability as {entailment}
 (see \cite{gs-infocomp2000}) without paying attention to the distinction.

{\paragraph{Content.} The rest of the paper is organized as follows.
\sref{sec:background} provides the necessary notation, terminology
and concepts used in the paper.
\sref{sec:partialsat} introduces entailment and
verification for generic propositional formulas and discusses their
relative properties and use.
\sref{sec:partialsat-exist} lifts the discussion to
existentially-quantified formulas.
\sref{sec:concl} provides some conclusions and future-work suggestions.
}



==> intro_v2.tex <==
% Although  CDCL 
% \cite{MSLM09HBSAT} 
% and SLS \cite{Maj09HBSAT} SAT solvers return  {\em total} truth assignments
% satisfying the input formula, other SAT procedures 

\TODO{Cambiare la narrazione:
\\- we wish... however...
\\- Proporre da
qualche parte ``satisfy'' as ``entailment''.
\\- far notare come
tipicamente evaluation to true.
}

 \newpage
\marg{need for PAS}
Many procedures for SAT and SAT-related problems
(e.g. OBDDs
\cite{bryant2}, Analytic Tableaux \cite{smullyan1}, DPLL
\cite{davis7}) rely their efficiency
on the detection of {\em partial} truth assignments $\mu$  satisfying an input
 propositional formula $\vi$, which allows to
state that (i) $\vi$ is satisfiable and (ii) all total 
assignments extending $\mu$ satisfy \vi. 
% state not only that $\vi$ is satisfiable, but also that all total 
% assignments extending $\mu$ satisfy \vi. 
In particular,
when it comes to SAT-based problems requiring
the {\em complete enumeration} of satisfying assignments (e.g. \#SAT
\cite{GomesSS21}, Lazy SMT \cite{BarrettSST21}, AllSAT and AllSMT
\cite{allsmt}, satisfiability of modal and description logics
\cite{SebastianiT21}, Weighted Model Integration \cite{MorPasSeb17}),
%
the ability of enumerating satisfying {partial} assignments which are
as small as possible is essential, because
%detecting that a partial assignment satisfies the input formula 
each of them
avoids the enumeration of the whole subtree
of total assignments extending it, whose size is exponential in the
number of unassigned propositions.

\marg{no definition}
Surprisingly,
% despite its widespread (implicit) usage of
% partial-assignment satisfiablity
% in algorithms and
%apart from the case of (tautology-free) CNF formulas,
there seems to be no general and universally-agreed definition of
partial-assignment satisfaction:
most authors do not
define partial-assignment satisfaction explicitly, or define it only when dealing with
(tautology-free) CNF formulas (e.g.  \cite{BuningK21});
%
\marg{algos diff notions}
also, different algorithms implictly implement different notions of
partial-assignment satisfaction (see below).
%
% In order to be useful, such a definition should at least guarantee
% that, if a partial assignment $\mu$ satisfies a formula \vi, then (i)
% \vi is satisfiable and (ii) all total truth assignments extending it
% satisfy \vi.~%\footnote{

%\begin{remark}
We stress the fact that this is not simply an issue of
the meaning of the word ``satisfy'': whichever ``verb'' one
might  use for it (e.g. ``satisfy'', ``entail'', ``imply'', ``evaluate to
true'',...), we would like a universally-agreed criterion
to extablishing that, if a partial truth-assignment ``verbs'' a formula
$\vi$, then (i) $\vi$ is satisfiable and (ii) all total truth
 assignments extending it satisfy $\vi$. 
\ignore{
we need a universally-agreed criterion
 complying with the two conditions (i) and (ii)
above.
} 
%\end{remark}
%}
% a criterion the sentence
% ``a partial truth assignment $\mu$ [verb] a formula $\vi$'' should
% imply that (i) \vi is satisfiable and (ii) that all total truth
% assignments extending it satisfy \vi. 

% a satisfying partial
% assignment can be generated instead of the whole subtree
% of total assignments extending it, whose size is exponential in the
% number of unassigned propositions.

% When we deal with (tautology-free) CNF formulas, the notion of
% partial-assignment satisfiablity is clear SPIEGA E CITA. BOTH PROPERTIES

\ignore{In this paper 
analyze in deep the notion of partial-assignment
satisfiability,
raising  a flag about the ambiguities and subtleties
of this concept,
and highlighting their practical consequences.

In this paper we
raise  a flag about the ambiguities and subtleties
of partial-assignment
satisfiability, in particular for  non-CNF or
existentially-quantified formulas, 
and investigate their practical consequences.
}
%\TODO{We wish to fill this gap...}

\RSTODO{move up?}
In this paper we want to address this issue explicitly. We
analyze the notion of partial-assignment
satisfiability,
raising  a flag about the ambiguities and subtleties
of this concept  --in particular when dealing with  non-CNF and
existentially-quantified formulas-- 
and we investigate their practical consequences.

\marg{$\entails$ vs. $\verifies$}
We start by noticing the following fact:
whereas for (tautology-free) CNF formulas
``{\em a partial truth assignment $\mu$ satisfies a formula $\vi$}''
may be indifferently be interpreted either as 
``$\mu$ {\em entails} $\vi$''
(i.e. ``all total assignments extending $\mu$
satisfy $\vi$'') or as ``$\mu$ {\em \verbverifies{}} $\vi$''
 (i.e. ``applying $\mu$ to $\vi$ makes $\vi$ true'') because in this
 case the two  concepts are equivalent,
 %
 for non-CNF formulas instead --and for
existentially-quantified formulas, even CNF ones--
{\em \verbverification{} is strictly stronger than entailment}, and they have
complementary properties. 
%
\ignore{
First we raise a flag on the fact that by
``{\em a partial truth assignment $\mu$ satisfies a formula $\vi$}'',
we may mean either that $\mu$ {\em entails} $\vi$
(i.e. that all total assignments extending $\mu$
satisfy $\vi$) or that $\mu$ {\em \verbverifies{}} $\vi$
 (i.e. that applying $\mu$ to $\vi$ makes $\vi$ true).
%
Typically most authors in the SAT community
leave this definition
implicit, or provide a definition only for (tautology-free) CNF
formulas (e.g. \cite{BuningK21}).
% where we notice that
% entailment and \verbverification{} concide. 
%
We notice that, whereas for (tautology-free) CNF formulas entailment 
and \verbverification{} are equivalent, for non-CNF formulas --and for
existentially-quantified formulas, even CNF ones--
{\em \verbverification{} is strictly stronger than entailment}, and they have
complementary properties. 
}
We also notice that standard
 (Tseitin-style) CNF-ization does not solve this
issue, because 
%with Tseitin CNF-ization 
it may lose 
information regarding partial-assignment entailment or \verbverification{}.
%\ignoreinshort{\TODO{Mention Kripke \& C e Stefano Tonetta?}}
%We stress the fact that the 

We also stress the fact that the distinction between entailment and \verbverification{}
is not only an issue of providing an universally-agreed definition of
partial-assignment satisfiability, but it also 
has important practical consequences. 
%
\RSTODO{Aggiungere $\verifies$ vs. equivalence}
\RSTODO{Although...}
On the one hand, checking entailment is computationally
much harder than checking
\verbverification{}. On the other hand, since partial assignments entailing
$\vi$ are in general subsets of those \verbverifying{} $\vi$, being able
to produce  partial assignments
{entailing} the input formula rather than {\verbverifying{}} it
 allows for producing smaller partial assignments,
and hence possibly drastically reducing their number. 
This may drive the development of more effective assignment-enumeration algorithms.
%
% When it comes to enumerating, in order to maximizing efficiency
% we would like to produce  partial assignments
% entailing the input formula, although most 
% algorithms give us only partial assignments
% \verbverifying{} it.

\marg{algos different notions of PAS}
To this extent we notice, e.g., that, when applied to non-CNF
formulas, 
OBDDs \cite{bryant2} implicitly enumerate partial assignment {entailing}
the input formulas,  whereas other procedures like Analytic Tableaux \cite{smullyan1} and
(non-CNF) DPLL \cite{davis7} implicitly enumerate partial assignment
{\verbverifying{}} them. 
%
Also, e.g., techniques like {\em pure-literal
filtering} 
%and {\em ghost-literal filtering} 
\cite{sebastiani07,BarrettSST21} in lazy
SMT 
implicitly aim at reducing a
total assignment to a partial one {\verbverifying{}} the input formula. 


%\TODO{Aggiungi riferimento a poll.\\}
\ignore{
\paragraph{A poll.}
In order to support the analysis, I've set up an email
poll among some current or past SAT PC and some SMT PC members, asking
for the truth/falsehood of five statements on the
notion of partial-assignment satisfiability.
The result are available at \cite{poll} %
%\footnote{\url{http://disi.unitn.it/rseba/partialsat_poll_2019.03.11.pdf}}
 and as an appendix submitted with this paper. 
Although only 20 out of 65 people replied, 
the result 
reveals the lack of general agreement among the repliers on the notion of
partial-assignment satisfiability and on its consequences: e.g.,
% since 
the repliers split evenly into supporters 
of entailment, of \verbverification{}, and people considering them equivalent.
}


\paragraph{Motivation.} The analysis presented in this paper was
triggered
by the effort of conceiving more efficient procedures for predicate
abstraction in SMT for improving Weighted Model Integration
\cite{MorPasSeb17,morettin_aij19},
which forced me to elaborate on the distinction between entailment
and \verbverification{}. Before then, I personally used to see
partial-assignment satisfiability as {entailment}
 (see \cite{gs-infocomp2000}) without paying attention to the distinction.

{\paragraph{Content.} The rest of the paper is organized as follows.
\sref{sec:background} provides the necessary notation, terminology
and concepts used in the paper.
\sref{sec:partialsat} introduces entailment and
\verbverification{} for generic propositional formulas and discusses their
relative properties and use.
\sref{sec:partialsat-exist} lifts the discussion to
existentially-quantified formulas.
\sref{sec:concl} provides some conclusions and future-work suggestions.
}



==> partialsat.tex.1 <==
%\input{fig_threevalues}
% 
{What do we mean by ``a \emph{partial} assignment $\mu$ satisfies $\vi$"?}
We wish to provide a satisfactory definition of partial-assignment
satisfiability for a generic propositional formula ---i.e., non
necessarily (tautology-free) CNF. 
%

\paragraph{\Verbvalidation{} vs. Entailment.}
Ideally, a suitable definition of partial-assignment satisfiability
should verify all statements in Property~\ref{prop:total-properties},
in particular (ii) and (iv). 
%
In practice, unfortunately, at least for generic (non-CNF) formulas, we see
 this is not the case. 

 One first possibility is to see partial-assignment satisfiability as
{\em \verbvalidation}. 
%
\begin{definition}
\label{def:validation}
We say that a {\em partial} truth assignment $\mu$  {\bf \verbvalidates{}} $\varphi$ 
iff $\muof{\vi}=\tval$ (or, equivalently by
Property~\ref{prop:eval-simplifies}, iff $\apply{\mu}{\vi}=\top$).
%
We denote this fact with ``$\mu\validates\varphi$''.
\end{definition}
%
One second possibility is to see partial-assignment satisfiability as
{\em entailment}. 

\begin{definition}
\label{def:entailment}
  We say that a {\em partial} truth assignment $\mu$  {\bf entails} $\varphi$
if and only if, for every total truth assignments $\eta$
s.t.$\mu\subseteq\eta$, 
$\eta$ satisfies $\varphi$. 
%
We denote this fact with ``$\mu\entails\varphi$''.
\end{definition}

\noindent
%\noindent
In substance,
Definition~\ref{def:validation} extends to partial assignments 
Property~\ref{prop:total-properties}(iii),
whereas 
Definition~\ref{def:entailment} extends to partial
assignments Property~\ref{prop:total-properties}(i).
%
Notice that both \verbvalidation{} and entailment are {\em semantic}
definitions.
Due to Property~\ref{prop:eval-simplifies}, \verbvalidation{}
has also an easy-to-check
syntactic characterization as ``$\apply{\mu}{\vi}=\top$''. 
% by Property~\ref{prop:eval-simplifies}, $\mu$ \verbvalidates{} $\varphi$ 
% if and only if the result of applying $\mu$ to $\varphi$ is $\top$.



When the formula $\vi$ is in CNF and does not contain
valid clauses --which however are easy to eliminate by preprocessing-- 
then Definitions~\ref{def:validation} and
\ref{def:entailment}  are equivalent: 
$\mu\validates\varphi$ iff $\mu\entails\varphi$.
%\footnote{ 
In fact, if $\mu\validates\vi$ then,  for every $\eta$ s.t.
$\eta\supseteq\mu$, $\eta\validates\vi$ and thus $\eta\models\vi$, hence
$\mu\entails\vi$;
also, if $\mu\entails\vi$ then $\applymuvi$ is a valid
  CNF formula which does not contain valid clauses, so that $\applymuvi$
  must be $\top$, hence $\mu\validates\vi$.
%}
% We guess this equivalence is the reason why these two concepts are rarely
% distinguished in the literature.


Unfortunately, when dealing with generic (non-CNF) formulas, 
we notice that \emph{Definitions~\ref{def:validation} and
\ref{def:entailment}  are not equivalent, the former being
strictly stronger than the latter}. 
%\noindent
In fact, as above, if $\mu\validates\vi$ then obviously
% ,  for every $\eta$ s.t.
% $\eta\supseteq\mu$, $\eta\validates\vi$ and thus $\eta\models\vi$, hence
$\mu\entails\vi$, whereas {\em the converse is not true}: e.g.,
if $\vi\defas(A_1\wedge A_2)\vee (A_1\wedge \neg A_2)$ and 
$\mu\defas\set{A_1}$, 
then 
$\mu\entails\vi$ but $\mu\not\validates\vi$.
%
This leads to the following statement.

\begin{proposition}
\label{prop:stronger}
If a partial truth assignment $\mu$ {\verbvalidates{}}
$\varphi$, then it also {entails} $\varphi$, but the converse does
not hold.
% : 
% $\mu\validates\vi \thus \mu\entails\vi$ but 
% $\mu\entails\vi \not\thus \mu\validates\vi$.
\end{proposition}
%
\begin{IGNOREINSHORT}
\begin{example}
%~\footnote{%
Let
$\mu\defas\set{A_1,..,A_M}$ s.t. $M<N$ and
$\vi\defas\bigvee_i (A_i\wedge cube_i)$ s.t. each $cube_i$ is a cube and $\bigvee_i cube_i$ is
valid and does not contain occurrences of the atoms $A_1,..,A_M$. Then 
$\mu\entails\vi$ but \applymuvi{} is the valid formula $\bigvee_i
cube_i$, so that $\mu\not\validates\vi$. \hfill $\diamond$
%}  
\end{example}  
\end{IGNOREINSHORT}


We try to build a counterpart of Property~\ref{prop:total-properties}
for Definitions~\ref{def:validation} and
\ref{def:entailment} respectively, but in both cases we fail to
achieve all points (i)-(iv) in Property~\ref{prop:total-properties},
resulting into complementary situations.
%

%\subsubsection{Pros and cons of partial-assignment satisfiability as validation.}
%%% Validation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
From Definition~\ref{def:validation}
we easily derive the following facts. 
(Here ``\oksym{}'' \resp{``\noksym{}''} denotes facts from
Property~\ref{prop:total-properties} which are \resp{are not} preserved.)

\begin{property}
\label{prop:partial-validation}
Let $\mu$ be a partial truth assignment on \alla{} and
$\vi,\vione,\vitwo$ be formulas on \alla. 
\begin{renumerate}
\item \noksym{}
If $\mu\validates\varphi$ then $\andmu\entails\varphi$, {but not vice versa}.
\item \noksym{}
If $\vione$ and $\vitwo$ are  equivalent, this {does not} imply
that $\mu\validates\vione$ iff $\mu\validates\vitwo$.
\item \oksym{}
  $\mu\validates\varphi$ iff \applymuvi{} is $\top$
     (also, iff $\muof{\vi}= \tval$ by Property~\ref{prop:eval-simplifies}). 

\item \oksym{}
Checking
$\mu\validates\vi$  requires at most a polynomial amount of steps.
\end{renumerate}  
\end{property}

%\subsubsection{Pros and cons of partial-assignment satisfiability as entailment.}
%%% Entailment
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
From Definition~\ref{def:entailment}
we easily derive the following. 

\begin{property}
\label{prop:partial-entailment}
Let $\mu$ be a partial truth assignment on \alla{} and
$\vi,\vione,\vitwo$ be formulas on \alla. 
\begin{renumerate}
\item \oksym{}
$\mu\models\varphi$ iff $\andmu\entails\varphi$.
\item \oksym{}
If $\vione$ and $\vitwo$ are  equivalent, then 
$\mu\models\vione$ iff $\mu\models\vitwo$.
\item \noksym{}
  $\mu\models\varphi$ iff \applymuvi{} is a valid formula, not
  necessarily $\top$
   (also, in general $\muof{\vi} \neq \tval$). 
\item \noksym{}
Checking
$\mu\entails\vi$ is \emph{co-NP-complete}.
\footnote{In fact, checking the validity of \vi{}
translates into verifying that the empty assignment
entails it.}
\end{renumerate}  
\end{property}
\noindent

For instance we notice that, when applied to satisfiable formulas,
%
OBDDs \cite{bryant2} produce branches representing
partial assignments which {\em entail} the input formula
(Definition~\ref{def:entailment}), because if $\mu\entails\vi$ then
\applymuvi is
valid (Property~\ref{prop:partial-entailment}(iii)), so that its corresponding 
sub-OBDD is reduced into the $\top$ node.
%
Instead SAT/AllSAT algorithms like \new{Analytic Tableaux} 
\footnote{Notice that Analytic Tableaux may generate duplicated
 or subsumed  assignments (see \cite{dagostino1,gs-infocomp2000})}
\cite{smullyan1} 
or ``classic'' \new{DPLL}~%
\footnote{Classic DPLL procedure \cite{davis7} was
  designed to work for CNF  
  formulas. Nevertheless it is easy to produce non-CNF a version of this
procedure (see e.g. \cite{armando5}).} 
%
\cite{davis7} produce branches representing
partial assignments which {\em \verbvalidate} the input formula
(Definition~\ref{def:validation}) because, unlike with OBDDs,
as soon as it is produced (a branch corresponding to) an assignment
$\mu$ s.t. 
$\mu\entails\vi$ but $\mu\not\validates\vi$, they do not realize it and
proceed the search until they extend it to some $\mu'\supset\mu$ s.t. 
$\mu'\validates\vi$, extending the search tree of up to
$2^{||\mu'||-||\mu||}$ branches.  
%
%\RSTODO{espandi un po' e spiaga perche'. example?}

%\input{figure.tex}
\input{figure_long.tex}
%
\begin{example}
%  \RSTODO{estendere a formula con 2 congiunti simili. Aggiungere XDDs? }
Consider $\vi\defas\mainwff$. 
  Figure~\ref{fig:comparison} 
represents the OBDD for $\vi$ and 
the search trees corresponding to 
All-SAT executions of Analytic
Tableaux and 
(non-CNF) DPLL on $\vi$. 
\begin{IGNOREINSHORT}
\footnote{Here in DPLL the pure-literal rule \cite{davis7} is not used because 
 in All-SAT it may hinder the enumeration of
 some relevant models (see, e.g., \cite{sebastiani_frocos07}).}  
\end{IGNOREINSHORT}
The former produces the single assignment
\singlemu{}. Notice that $\singlemu\entails\vi$ but $\singlemu\not
\validates\vi$.  The latter two produce the assignments \allmus{}.

Notice that neither Analytic Tableaux nor DPLL can produce \singlemu{} alone.
\hfill $\diamond$
\end{example}

\TODO{Riscrivi prossimo paragrafo}
\marg{\Verbvalidation{} vs. Entailment.}
The advantage of adopting \verbvalidation{} for checking
% as a definition of
partial-assignment satisfiability is that it matches the intuition
and practical need that the process of checking it should be fast (Property~\ref{prop:partial-validation}(iv)).  
%
The main drawback is that 
that equivalent although syntactically different 
formulas may be satisfied by different sets of partial
assignments  (Property~\ref{prop:partial-validation}(ii)), 
which looks theoretically awkward. 
%even partial (Property~\ref{prop:partial-entailment}(ii)). 
\ignoreinshort{%
We believe this would be an embarrassing fact
if we adopted \verbvalidation{} as the definition of  partial-assignment
satisfiability for non-CNF formulas.
}

%\TODO{We believe this is quite embarassing...}

On the one hand, 
the advantage of adopting entailment
%as a definition of
%Definition~\ref{def:entailment} as
for checking
partial-assignment satisfiability is that it matches the intuition 
and theoretical requirement
that equivalent formulas should be satisfied by the same assignments,
even partial ones (Property~\ref{prop:partial-entailment}(ii)). 
%
On the other hand, the price to pay is that the resulting problem 
is co-NP-complete  (Property~\ref{prop:partial-entailment}(iv)),
because it is equivalent to checking the validity of the residual \applymuvi.


\smallskip
Due to Proposition~\ref{prop:stronger}, every
 partial assignments entailing the input formula is  a \emph{subset}
 of some other(s) \verbvalidating{} it.
Therefore, for an assignment-enumeration algorithm,
 being able to enumerate partial 
assignments entailing the input formula rather than simply \verbvalidating{}
it  may (even drastically) reduce the number of the satisfying assignment
enumerated. 
%



%\NOTE{Spiegare. }
\begin{IGNOREINSHORT}  
\paragraph{Other possible partial-satisfaction relations.}
Given the above facts, we wonder if we could use other notions
of partial-assignment satisfiability (e.g., we could enrich
$\validates$ with some form of formula simplification).
In particular, we wonder if there exists some suitable notion of
partial-assignment satisfaction which is strictly stronger than
entailment and fixes the ``embarassing issue'' of
Property~\ref{prop:partial-validation}(ii).
The following theorem states this is not the case.
\begin{theorem}
\label{uniqueness:teo}
Let $\genericentails$ denote some generical relation between a (possibly partial)
truth assignment  and a Boolean formula, such that
% \RSTODO{sostituire (a) con ``if $\eta$ total for $\vi$, then
%   $\eta\genericentails\vi$ iff
%   $\eta\models\vi$? Da questo deriva anche (b)?}
\begin{aenumerate}
\item  if $\eta$ is total for $\vi$, then
  $\eta\genericentails\vi$ iff
  $\eta\models\vi$;
\item for every $\mu$, $\vi_1$ and $\vi_2$, if $\mu\genericentails\vi_1\wedge\vi_2$, then $\mu\genericentails\vi_1$ and
  $\mu\genericentails\vi_2$;
\item there exist $\mu$ and $\vi$ s.t. $\mu\entails\vi$ and $\mu\not\genericentails\vi$ .
\end{aenumerate}
Then there exist $\mu'$, $\psi_1$ and $\psi_2$ s.t. $\psi_1\equiv\psi_2$, 
$\mu'\genericentails\psi_1$ and $\mu'\not\genericentails\psi_2$.
\end{theorem}
\begin{proof}
%% PROOF VERIFICATA
  Consider $\mu$ and $\vi$ as in point {\em (c)}.
  Let $\mu'\defas\mu$,
  $\psi_1\defas\andmu$ and $\psi_2\defas\andmu\wedge\varphi$.
  Then $\psi_1\equiv\psi_2$ because $\mu\entails\vi$ and because of
  Property~\ref{prop:partial-entailment}(i); also, $\mu'\genericentails\psi_1$
  by point {\em (a)} and $\mu'\not\genericentails\psi_2$ by point {\em
    (b)}.
  \hfill $\diamond$
\end{proof}
Theorem \ref{uniqueness:teo} says that entailment is
the only relation
which extends to partial assignments the standard notion of
total-assignment satisfaction
(point $(a)$), maintains the standard semantics of
$\wedge$ (point $(b)$) and verifies
Property~\ref{prop:partial-entailment}(ii).
Any relation $\genericentails$ which is strictly stronger than $\models$ suffers for
the same ``embarassing issue'' of
Property~\ref{prop:partial-validation}(ii) (point $(c)$).
% Theorem \ref{uniqueness:teo} says that if a relation $\genericentails$
% extends to partial assignments the standard notion of satisfaction
% (point $(a)$), maintains the standard semantics of
% $\wedge$ (point $(b)$) and
% is strictly stronger than entailment (point $(c)$), than it does not verify
% Property~\ref{prop:partial-entailment}(ii), that is, it suffers for
% the same ``embarassing issue'' of
% Property~\ref{prop:partial-validation}(ii).
\end{IGNOREINSHORT}

\paragraph{Dealing with CNF-ized formulas.}
One may argue that in SAT/AllSAT the distinction between $\validates$ and
$\entails$ is not much relevant in practice, because we can
CNF-ize upfront the input formulas ---typically by
variants of Tseitin CNF-ization--- removing tautological clauses, and this
distinction does not hold for (tautology-free) CNF
formulas.
%
However, we notice that with Tseitin CNF-ization we may loose
information regarding entailment or \verbvalidation{}. In fact, if
$\psi$ on $\alla\cup\allb$ is the result of Tseitin CNF-izing $\vi$,
then:
\begin{itemize}
% \item 
% If $\mu\cup\gamma\validates\phi$ for some total truth assignment
%   $\gamma$, then $\mu\validates\vi$.
% \item 
% If $\mu\cup\gamma\entails\phi$ for some total truth assignment
%   $\gamma$, then $\mu\entails\vi$.
\item 
$\mu\validates\vi$ \emph{does not imply} that there exists a total assignment
  $\delta$ on \allb s.t. $\mu\cup\delta\validates\psi$;
\item 
$\mu\entails\vi$ \emph{does not imply} that there exists a total assignment
  $\delta$ on \allb s.t. $\mu\cup\delta\entails\psi$.
\end{itemize}

\begin{example}
Consider $\vi\defas A_1 \vee (A_2\wedge A_3)$ 
and its Tseitin CNF-ized version:\\
$
\begin{array}{lll}
\psi\defas & (A_1\vee  B_1)\ \wedge \\
& (\neg B_1 \vee  A_2) \wedge
(\neg B_1 \vee  A_3) \wedge 
(B_1\vee \neg A_2 \vee \neg A_3) & \ \ \ //\ B_1 \iff (A_2\wedge A_3). \\
\end{array}
$\\
On the one hand, $\mu\defas \set{A_1}$ is such that $\mu\validates\vi$. 
On the other hand, there is no total truth assignment $\delta$ on
\set{B_1} s.t. $\mu\cup\delta\validates\psi$. In fact, neither 
$\set{A_1,B_1}\validates\psi$ nor $\set{A_1,\neg B_1}\validates\psi$.

Consider $\vi\defas
(A_1\wedge \pos A_2)\vee (A_1\wedge\neg A_2) 
$ 
and its Tseitin CNF-ized version:\\
$
\begin{array}{lll}
\psi\defas  
& (B_1\vee B_2)\ \wedge & \\
& (\neg B_1 \vee \pos A_1) \wedge
(\neg B_1 \vee \pos A_2) \wedge
(B_1\vee \neg A_1 \vee \neg A_2)\ \wedge\ & \ \ \ //\ B_1 \iff (A_1\wedge \pos A_2) \\
& (\neg B_2 \vee \pos A_1) \wedge
(\neg B_2 \vee \neg A_2) \wedge
(B_2\vee \neg A_1 \vee \pos A_2).\ & \ \ \ //\ B_2 \iff (A_1\wedge \neg A_2) 
\end{array}
%
% \psi\defas
% (B_1\vee B_2) \wedge
% (\neg B_1 \vee A_1) \wedge
% (\neg B_1 \vee A_2) \wedge
% (B_1\vee \neg A_1 \vee \neg A_2) \wedge
% (\neg B_2 \vee \neg A_1) \wedge
% (\neg B_2 \vee \neg A_2) \wedge
% (B_2\vee \neg A_1 \vee A_2)   
$\\
Although $\mu\defas \set{A_1}$ is such that $\mu\entails\vi$,
%On the other hand,
 there is no total truth assignment $\delta$ on
\set{B_1,B_2} s.t. $\mu\cup\delta\entails\psi$:
$\set{A_1,B_1,\neg B_2}\not\entails \psi$ since
$\set{A_1,\neg A_2,B_1,\neg B_2}\not\entails \psi$;
$\set{A_1,\neg B_1,B_2}\not\entails \psi$
since $\set{A_1,A_2,\neg B_1,B_2}\not\entails \psi$;
$\set{A_1,B_1,B_2}$ and $\set{A_1,\neg B_1,\neg B_2}$ are both inconsistent
with $\psi$.
\hfill $\diamond$
\end{example}

\ignore{%%%%%%%%%%
\begin{proposition}
 \RSTODO{PROVA e scrivi controesempi. Scrivi in background l'equivalente controparte per $\eta \models\vi$\\}
Let $\vi$ be a generic (non-CNF)
formula on \alla and let $\psi$ on $\alla\cup\allb$ be the result of
CNF-izing \vi by applying standard Tseitin CNF-ization 
\cite{tseitin1} and removing valid clauses from $\psi$ if any, \allb
being the set of fresh propositions introduced in the process. Then:
\begin{itemize}
\item 
If $\mu\cup\gamma\validates\psi$ for some total truth assignment
  $\gamma$, then $\mu\validates\vi$.
\item 
If $\mu\cup\gamma\entails\psi$ for some total truth assignment
  $\gamma$, then $\mu\entails\vi$.
\item 
$\mu\validates\vi$ \emph{does not imply} that there exists a total assignment
  $\delta$ on \allb s.t. $\mu\cup\delta\validates\vi$
\item 
$\mu\entails\vi$ \emph{does not imply} that there exists a total assignment
  $\delta$ on \allb s.t. $\mu\cup\delta\entails\vi$
\end{itemize}

%Then $\mu\validates\vi$, but
%$\mu\entails\vi$
\end{proposition}
}


==> partialsat.tex.2 <==
%\input{fig_threevalues}
% 
{What do we mean by ``a \emph{partial} assignment $\mu$ satisfies $\vi$"?}
We wish to provide a satisfactory definition of partial-assignment
satisfiability for a generic propositional formula ---i.e., non
necessarily (tautology-free) CNF. 
%

\paragraph{\Verbvalidation{} vs. Entailment.}
Ideally, a suitable definition of partial-assignment satisfiability
should verify all statements in Property~\ref{prop:total-properties},
in particular (ii) and (iv). 
%
In practice, unfortunately, at least for generic (non-CNF) formulas, we see
 this is not the case. 

 One first possibility is to see partial-assignment satisfiability as
{\em \verbvalidation}. 
%
\begin{definition}
\label{def:validation}
We say that a {\em partial} truth assignment $\mu$  {\bf \verbvalidates{}} $\varphi$ 
iff $\muof{\vi}=\tval$ (or, equivalently by
Property~\ref{prop:eval-simplifies}, iff $\apply{\mu}{\vi}=\top$).
%
We denote this fact with ``$\mu\validates\varphi$''.
\end{definition}
%
One second possibility is to see partial-assignment satisfiability as
{\em entailment}. 

\begin{definition}
\label{def:entailment}
  We say that a {\em partial} truth assignment $\mu$  {\bf entails} $\varphi$
if and only if, for every total truth assignments $\eta$
s.t.$\mu\subseteq\eta$, 
$\eta$ satisfies $\varphi$. 
%
We denote this fact with ``$\mu\entails\varphi$''.
\end{definition}

\noindent
%\noindent
In substance,
Definition~\ref{def:validation} extends to partial assignments 
Property~\ref{prop:total-properties}(iii),
whereas 
Definition~\ref{def:entailment} extends to partial
assignments Property~\ref{prop:total-properties}(i).
%
Notice that both \verbvalidation{} and entailment are {\em semantic}
definitions.
Due to Property~\ref{prop:eval-simplifies}, \verbvalidation{}
has also an easy-to-check
syntactic characterization as ``$\apply{\mu}{\vi}=\top$''. 
% by Property~\ref{prop:eval-simplifies}, $\mu$ \verbvalidates{} $\varphi$ 
% if and only if the result of applying $\mu$ to $\varphi$ is $\top$.



When the formula $\vi$ is in CNF and does not contain
valid clauses --which however are easy to eliminate by preprocessing-- 
then Definitions~\ref{def:validation} and
\ref{def:entailment}  are equivalent: 
$\mu\validates\varphi$ iff $\mu\entails\varphi$.
%\footnote{ 
In fact, if $\mu\validates\vi$ then,  for every $\eta$ s.t.
$\eta\supseteq\mu$, $\eta\validates\vi$ and thus $\eta\models\vi$, hence
$\mu\entails\vi$;
also, if $\mu\entails\vi$ then $\applymuvi$ is a valid
  CNF formula which does not contain valid clauses, so that $\applymuvi$
  must be $\top$, hence $\mu\validates\vi$.
%}
% We guess this equivalence is the reason why these two concepts are rarely
% distinguished in the literature.


Unfortunately, when dealing with generic (non-CNF) formulas, 
we notice that \emph{Definitions~\ref{def:validation} and
\ref{def:entailment}  are not equivalent, the former being
strictly stronger than the latter}. 
%\noindent
In fact, as above, if $\mu\validates\vi$ then obviously
% ,  for every $\eta$ s.t.
% $\eta\supseteq\mu$, $\eta\validates\vi$ and thus $\eta\models\vi$, hence
$\mu\entails\vi$, whereas {\em the converse is not true}: e.g.,
if $\vi\defas(A_1\wedge A_2)\vee (A_1\wedge \neg A_2)$ and 
$\mu\defas\set{A_1}$, 
then 
$\mu\entails\vi$ but $\mu\not\validates\vi$.
%
This leads to the following statement.

\begin{proposition}
\label{prop:stronger}
If a partial truth assignment $\mu$ {\verbvalidates{}}
$\varphi$, then it also {entails} $\varphi$, but the converse does
not hold.
% : 
% $\mu\validates\vi \thus \mu\entails\vi$ but 
% $\mu\entails\vi \not\thus \mu\validates\vi$.
\end{proposition}
%
\begin{IGNOREINSHORT}
\begin{example}
%~\footnote{%
Let
$\mu\defas\set{A_1,..,A_M}$ s.t. $M<N$ and
$\vi\defas\bigvee_i (A_i\wedge cube_i)$ s.t. each $cube_i$ is a cube and $\bigvee_i cube_i$ is
valid and does not contain occurrences of the atoms $A_1,..,A_M$. Then 
$\mu\entails\vi$ but \applymuvi{} is the valid formula $\bigvee_i
cube_i$, so that $\mu\not\validates\vi$. \hfill $\diamond$
%}  
\end{example}  
\end{IGNOREINSHORT}


We try to build a counterpart of Property~\ref{prop:total-properties}
for Definitions~\ref{def:validation} and
\ref{def:entailment} respectively, but in both cases we fail to
achieve all points (i)-(iv) in Property~\ref{prop:total-properties},
resulting into complementary situations.
%

%\subsubsection{Pros and cons of partial-assignment satisfiability as validation.}
%%% Validation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
From Definition~\ref{def:validation}
we easily derive the following facts. 
(Here ``\oksym{}'' \resp{``\noksym{}''} denotes facts from
Property~\ref{prop:total-properties} which are \resp{are not} preserved.)

\begin{property}
\label{prop:partial-validation}
Let $\mu$ be a partial truth assignment on \alla{} and
$\vi,\vione,\vitwo$ be formulas on \alla. 
\begin{renumerate}
\item \noksym{}
If $\mu\validates\varphi$ then $\andmu\entails\varphi$, {but not vice versa}.
\item \noksym{}
If $\vione$ and $\vitwo$ are  equivalent, this {does not} imply
that $\mu\validates\vione$ iff $\mu\validates\vitwo$.
\item \oksym{}
  $\mu\validates\varphi$ iff \applymuvi{} is $\top$
     (also, iff $\muof{\vi}= \tval$ by Property~\ref{prop:eval-simplifies}). 

\item \oksym{}
Checking
$\mu\validates\vi$  requires at most a polynomial amount of steps.
\end{renumerate}  
\end{property}

%\subsubsection{Pros and cons of partial-assignment satisfiability as entailment.}
%%% Entailment
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
From Definition~\ref{def:entailment}
we easily derive the following. 

\begin{property}
\label{prop:partial-entailment}
Let $\mu$ be a partial truth assignment on \alla{} and
$\vi,\vione,\vitwo$ be formulas on \alla. 
\begin{renumerate}
\item \oksym{}
$\mu\models\varphi$ iff $\andmu\entails\varphi$.
\item \oksym{}
If $\vione$ and $\vitwo$ are  equivalent, then 
$\mu\models\vione$ iff $\mu\models\vitwo$.
\item \noksym{}
  $\mu\models\varphi$ iff \applymuvi{} is a valid formula, not
  necessarily $\top$
   (also, in general $\muof{\vi} \neq \tval$). 
\item \noksym{}
Checking
$\mu\entails\vi$ is \emph{co-NP-complete}.
\footnote{In fact, checking the validity of \vi{}
translates into verifying that the empty assignment
entails it.}
\end{renumerate}  
\end{property}
\noindent


\TODO{Riscrivi prossimo paragrafo}
\marg{\Verbvalidation{} vs. Entailment.}
The advantage of adopting \verbvalidation{} for checking
% as a definition of
partial-assignment satisfiability is that it matches the intuition
and practical need that the process of checking it should be fast (Property~\ref{prop:partial-validation}(iv)).  
%
The main drawback is that 
that equivalent although syntactically different 
formulas may be satisfied by different sets of partial
assignments  (Property~\ref{prop:partial-validation}(ii)), 
which looks theoretically awkward. 
%even partial (Property~\ref{prop:partial-entailment}(ii)). 
\ignoreinshort{%
We believe this would be an embarrassing fact
if we adopted \verbvalidation{} as the definition of  partial-assignment
satisfiability for non-CNF formulas.
}

%\TODO{We believe this is quite embarassing...}

On the one hand, 
the advantage of adopting entailment
%as a definition of
%Definition~\ref{def:entailment} as
for checking
partial-assignment satisfiability is that it matches the intuition 
and theoretical requirement
that equivalent formulas should be satisfied by the same assignments,
even partial ones (Property~\ref{prop:partial-entailment}(ii)). 
%
On the other hand, the price to pay is that the resulting problem 
is co-NP-complete  (Property~\ref{prop:partial-entailment}(iv)),
because it is equivalent to checking the validity of the residual \applymuvi.


\smallskip
Due to Proposition~\ref{prop:stronger}, every
 partial assignments entailing the input formula is  a \emph{subset}
 of some other(s) \verbvalidating{} it.
Therefore, for an assignment-enumeration algorithm,
 being able to enumerate partial 
assignments entailing the input formula rather than simply \verbvalidating{}
it  may (even drastically) reduce the number of the satisfying assignment
enumerated. 
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Procedures using \verbvalidation and entailment.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Procedures using \verbvalidation{} and entailment.}
We notice that, when applied to satisfiable formulas,
algorithms like \new{Analytic Tableaux}~\footnote{Notice that Analytic Tableaux may generate duplicated
 or subsumed  assignments (see \cite{dagostino1,gs-infocomp2000})}
\cite{smullyan1} 
or ``classic'' \new{DPLL}~%
\footnote{Classic DPLL procedure \cite{davis7} was
  designed to work for CNF  
  formulas. Nevertheless it is easy to produce non-CNF a version of this
procedure (see e.g. \cite{armando5}).} 
%
\cite{davis7} produce branches representing
partial assignments which {\em \verbvalidate} the input formula
(Definition~\ref{def:validation}). Consequently, 
as soon as these procedures produce (a branch corresponding to) an assignment
$\mu$ s.t. 
$\mu\entails\vi$ but $\mu\not\validates\vi$, they cannot realize this
fact and
proceed the search until they extend it to some $\mu'\supset\mu$ s.t. 
$\mu'\validates\vi$. This causes an extension of the search tree of up to
$2^{||\mu'||-||\mu||}$ branches.  
%
OBDDs instead \cite{bryant2} produce branches representing
partial assignments which {\em entail} the input formula
(Definition~\ref{def:entailment}), because if $\mu\entails\vi$ then
\applymuvi is
valid (Property~\ref{prop:partial-entailment}(iii)), so that its corresponding 
sub-OBDD is reduced into the $\top$ node.
%\input{figure.tex}
\input{figure_long.tex}
%
\begin{example}
Consider $\vi\defas\mainwff$. 
  Figure~\ref{fig:comparison} 
represents 
the search trees corresponding to 
All-SAT executions of Analytic
Tableaux and 
(non-CNF) DPLL on $\vi$,%
\footnote{Here in DPLL the pure-literal rule \cite{davis7} is not used because 
 in All-SAT it may hinder the enumeration of
 some relevant models (see, e.g., \cite{sebastiani_frocos07}).}  
and the OBDD for $\vi$.
The former two produce the assignments \allmus{}.
The latter produces the single assignment
\singlemu{}, s.t. $\singlemu\entails\vi$ but $\singlemu\not
\validates\vi$.
% Notice that neither Analytic Tableaux nor DPLL can produce \singlemu{} alone.
\hfill$\diamond$
\end{example}
\TODO{Aggiungere XDDs? }


%\NOTE{Spiegare. }
%\begin{IGNOREINSHORT}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Other possible partial-satisfaction relations.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Other possible partial-satisfaction relations.}
Given the above facts, we wonder if we could use other notions
of partial-assignment satisfiability (e.g., we could enrich
$\validates$ with some form of formula simplification).
In particular, we wonder if there exists some suitable notion of
partial-assignment satisfaction which is strictly stronger than
entailment and fixes the ``embarassing issue'' of
Property~\ref{prop:partial-validation}(ii).
The following theorem states this is not the case.
\begin{theorem}
\label{uniqueness:teo}
Let $\genericentails$ denote some generical relation between a (possibly partial)
truth assignment  and a Boolean formula, such that
% \RSTODO{sostituire (a) con ``if $\eta$ total for $\vi$, then
%   $\eta\genericentails\vi$ iff
%   $\eta\models\vi$? Da questo deriva anche (b)?}
\begin{aenumerate}
\item  if $\eta$ is total for $\vi$, then
  $\eta\genericentails\vi$ iff
  $\eta\models\vi$;
\item for every $\mu$, $\vi_1$ and $\vi_2$, if $\mu\genericentails\vi_1\wedge\vi_2$, then $\mu\genericentails\vi_1$ and
  $\mu\genericentails\vi_2$;
\item there exist $\mu$ and $\vi$ s.t. $\mu\entails\vi$ and $\mu\not\genericentails\vi$ .
\end{aenumerate}
Then there exist $\mu'$, $\psi_1$ and $\psi_2$ s.t. $\psi_1\equiv\psi_2$, 
$\mu'\genericentails\psi_1$ and $\mu'\not\genericentails\psi_2$.
\end{theorem}
\begin{proof}
%% PROOF VERIFICATA
  Consider $\mu$ and $\vi$ as in point {\em (c)}.
  Let $\mu'\defas\mu$,
  $\psi_1\defas\andmu$ and $\psi_2\defas\andmu\wedge\varphi$.
  Then $\psi_1\equiv\psi_2$ because $\mu\entails\vi$ and because of
  Property~\ref{prop:partial-entailment}(i); also, $\mu'\genericentails\psi_1$
  by point {\em (a)} and $\mu'\not\genericentails\psi_2$ by point {\em
    (b)}.
  \hfill $\diamond$
\end{proof}
Theorem \ref{uniqueness:teo} says that entailment is
the only relation
which extends to partial assignments the standard notion of
total-assignment satisfaction
(point $(a)$), maintains the standard semantics of
$\wedge$ (point $(b)$) and verifies
Property~\ref{prop:partial-entailment}(ii).
Any relation $\genericentails$ which is strictly stronger than $\models$ suffers for
the same ``embarassing issue'' of
Property~\ref{prop:partial-validation}(ii) (point $(c)$).
% Theorem \ref{uniqueness:teo} says that if a relation $\genericentails$
% extends to partial assignments the standard notion of satisfaction
% (point $(a)$), maintains the standard semantics of
% $\wedge$ (point $(b)$) and
% is strictly stronger than entailment (point $(c)$), than it does not verify
% Property~\ref{prop:partial-entailment}(ii), that is, it suffers for
% the same ``embarassing issue'' of
% Property~\ref{prop:partial-validation}(ii).
%\end{IGNOREINSHORT}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Dealing with CNF-ized formulas.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Dealing with CNF-ized formulas.}
One may argue that in SAT/AllSAT the distinction between $\validates$ and
$\entails$ is not much relevant in practice, because we can
CNF-ize upfront the input formulas ---typically by
variants of Tseitin CNF-ization--- removing tautological clauses, and this
distinction does not hold for (tautology-free) CNF
formulas.
%
However, we notice that with Tseitin CNF-ization we may loose
information regarding entailment or \verbvalidation{}. In fact, if
$\psi$ on $\alla\cup\allb$ is the result of Tseitin CNF-izing $\vi$,
then:
\begin{itemize}
% \item 
% If $\mu\cup\gamma\validates\phi$ for some total truth assignment
%   $\gamma$, then $\mu\validates\vi$.
% \item 
% If $\mu\cup\gamma\entails\phi$ for some total truth assignment
%   $\gamma$, then $\mu\entails\vi$.
\item 
$\mu\validates\vi$ \emph{does not imply} that there exists a total assignment
  $\delta$ on \allb s.t. $\mu\cup\delta\validates\psi$;
\item 
$\mu\entails\vi$ \emph{does not imply} that there exists a total assignment
  $\delta$ on \allb s.t. $\mu\cup\delta\entails\psi$.
\end{itemize}

\begin{example}
Consider $\vi\defas A_1 \vee (A_2\wedge A_3)$ 
and its Tseitin CNF-ized version:\\
$
\begin{array}{lll}
\psi\defas & (A_1\vee  B_1)\ \wedge \\
& (\neg B_1 \vee  A_2) \wedge
(\neg B_1 \vee  A_3) \wedge 
(B_1\vee \neg A_2 \vee \neg A_3) & \ \ \ //\ B_1 \iff (A_2\wedge A_3). \\
\end{array}
$\\
On the one hand, $\mu\defas \set{A_1}$ is such that $\mu\validates\vi$. 
On the other hand, there is no total truth assignment $\delta$ on
\set{B_1} s.t. $\mu\cup\delta\validates\psi$. In fact, neither 
$\set{A_1,B_1}\validates\psi$ nor $\set{A_1,\neg B_1}\validates\psi$.

Consider $\vi\defas
(A_1\wedge \pos A_2)\vee (A_1\wedge\neg A_2) 
$ 
and its Tseitin CNF-ized version:\\
$
\begin{array}{lll}
\psi\defas  
& (B_1\vee B_2)\ \wedge & \\
& (\neg B_1 \vee \pos A_1) \wedge
(\neg B_1 \vee \pos A_2) \wedge
(B_1\vee \neg A_1 \vee \neg A_2)\ \wedge\ & \ \ \ //\ B_1 \iff (A_1\wedge \pos A_2) \\
& (\neg B_2 \vee \pos A_1) \wedge
(\neg B_2 \vee \neg A_2) \wedge
(B_2\vee \neg A_1 \vee \pos A_2).\ & \ \ \ //\ B_2 \iff (A_1\wedge \neg A_2) 
\end{array}
%
% \psi\defas
% (B_1\vee B_2) \wedge
% (\neg B_1 \vee A_1) \wedge
% (\neg B_1 \vee A_2) \wedge
% (B_1\vee \neg A_1 \vee \neg A_2) \wedge
% (\neg B_2 \vee \neg A_1) \wedge
% (\neg B_2 \vee \neg A_2) \wedge
% (B_2\vee \neg A_1 \vee A_2)   
$\\
Although $\mu\defas \set{A_1}$ is such that $\mu\entails\vi$,
%On the other hand,
 there is no total truth assignment $\delta$ on
\set{B_1,B_2} s.t. $\mu\cup\delta\entails\psi$:
$\set{A_1,B_1,\neg B_2}\not\entails \psi$ since
$\set{A_1,\neg A_2,B_1,\neg B_2}\not\entails \psi$;
$\set{A_1,\neg B_1,B_2}\not\entails \psi$
since $\set{A_1,A_2,\neg B_1,B_2}\not\entails \psi$;
$\set{A_1,B_1,B_2}$ and $\set{A_1,\neg B_1,\neg B_2}$ are both inconsistent
with $\psi$.
\hfill $\diamond$
\end{example}

\ignore{%%%%%%%%%%
\begin{proposition}
 \RSTODO{PROVA e scrivi controesempi. Scrivi in background l'equivalente controparte per $\eta \models\vi$\\}
Let $\vi$ be a generic (non-CNF)
formula on \alla and let $\psi$ on $\alla\cup\allb$ be the result of
CNF-izing \vi by applying standard Tseitin CNF-ization 
\cite{tseitin1} and removing valid clauses from $\psi$ if any, \allb
being the set of fresh propositions introduced in the process. Then:
\begin{itemize}
\item 
If $\mu\cup\gamma\validates\psi$ for some total truth assignment
  $\gamma$, then $\mu\validates\vi$.
\item 
If $\mu\cup\gamma\entails\psi$ for some total truth assignment
  $\gamma$, then $\mu\entails\vi$.
\item 
$\mu\validates\vi$ \emph{does not imply} that there exists a total assignment
  $\delta$ on \allb s.t. $\mu\cup\delta\validates\vi$
\item 
$\mu\entails\vi$ \emph{does not imply} that there exists a total assignment
  $\delta$ on \allb s.t. $\mu\cup\delta\entails\vi$
\end{itemize}

%Then $\mu\validates\vi$, but
%$\mu\entails\vi$
\end{proposition}
}

